Logicbreaks: A Framework for Understanding Subversion of Rule-based Inference

We study how to subvert large language models (LLMs) from following prompt-specified rules. We first formalize rule-following as inference in propositional Horn logic, a mathematical system in which rules have the form "if $P$ and $Q$, then $R$" for some propositions $P$, $Q$, and $R$. Next, we prove that although small transformers can faithfully follow such rules, maliciously crafted prompts can still mislead both theoretical constructions and models learned from data. Furthermore, we demonstrate that popular attack algorithms on LLMs find adversarial prompts and induce attention patterns that align with our theory. Our novel logic-based framework provides a foundation for studying LLMs in rule-based settings, enabling a formal analysis of tasks like logical reasoning and jailbreak attacks.

==> contents/iclr_statements.tex <==

\myparagraph{Ethics Statement}
Our work seeks to understand the principles behind how jailbreak attacks subvert prompt-specified rules.
This work is useful for LLM developers who aim to improve model safeguards, and it is insightful for researchers seeking to better understand the mechanics of LLM reasoning.
However, because our work studies attacks, a malicious user may leverage our findings to improve adversarial attacks.


\myparagraph{Reproducibility Statement}
% {\color{editblue}
All code and experiments from this paper are available and open-sourced at~\url{https://github.com/AntonXue/tf_logic}
% \texttt{{https://anonymous.4open.science/r/tf\_logic-4DE6}}.
% }

==> figures/exp_qb2_llama_attentions_example.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=1.0\linewidth]{images/llama_supression.png}

\caption{
Llama-7B also exhibits a similar attention pattern mechanism when attacked to disobey context rules.
}

\label{fig:exp_qb2_llama_attentions_example}
\end{figure}

==> figures/exp_qb2_minecraft_attacks_analysis.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=1.0\linewidth]{images/minecraft_suppression.png}

\caption{
The attention values on the suppressed rule are lower when the adversarial suffix is present.
}

\label{fig:exp_qb2_attn}
\end{figure}

==> figures/exp_qb2_minecraft_attacks_attn_tradeoff.tex <==
\begin{figure}[t]
\centering

\begin{minipage}{0.48\textwidth}    
    \includegraphics[width=1.0\linewidth]{images/attn_plot_have_1.png}
\end{minipage}%
\begin{minipage}{0.48\textwidth}
    \includegraphics[width=1.0\linewidth]{images/attn_plot_have_1.png}
\end{minipage}%

% \begin{minipage}{0.48\textwidth}    
%     \includegraphics[width=1.0\linewidth]{images/exp2_suppress_rule_acc.png}
% \end{minipage}%
% \begin{minipage}{0.48\textwidth}    
%     \includegraphics[width=1.0\linewidth]{images/exp2_suppress_rule_attn.png}
% \end{minipage}%

% \begin{minipage}{0.48\textwidth}
%     \includegraphics[width=1.0\linewidth]{images/exp2_knowledge_amnesia_acc.png}
% \end{minipage}%
% \begin{minipage}{0.48\textwidth}    
%     \includegraphics[width=1.0\linewidth]{images/exp2_knowledge_amnesia_attn.png}
% \end{minipage}%

\caption{
Attention on the antecedents of the target rule is suppressed with the adversarial suffix. 
}
\label{fig:exp_qb2_attn_tradeoff}
\end{figure}

==> figures/one_inference_step.tex <==
\begin{figure*}[t]
\centering

\begin{center}
\begin{tikzcd}[column sep=large]
    (\Gamma, \Phi) \arrow[r, ""]
        \arrow[rd, "\msf{Enc}", swap]
        & \{A\} \arrow[r, "\msf{Apply}{[}\Gamma{]}"]
        & \{A,B,C\} \arrow[r, "\msf{Apply}{[}\Gamma{]}"]
        & \{A,B,C,E\} \arrow[r, "\msf{Apply}{[}\Gamma{]}"]
        & \{A,B,C,E,F\} \\
    & X_0 \arrow[r, "{\mcal{R},\,\msf{Dec},\,\msf{concat}}", swap]
            \arrow[u, "\msf{Dec}", swap]
    & X_1 \arrow[r, "{\mcal{R},\,\msf{Dec},\,\msf{concat}}", swap]
        \arrow[u, "\msf{Dec}", swap]
    & X_2 \arrow[r, "{\mcal{R},\,\msf{Dec},\,\msf{concat}}", swap]
        \arrow[u, "\msf{Dec}", swap]
    & X_3
        \arrow[u, "\msf{Dec}", swap]
\end{tikzcd}
\end{center}

\caption{
The ideal relation between the proof states generated by the forward chaining algorithm and those generated by chain-of-thought iterations with a reasoner \(\mcal{R}\).
Using rules \(\Gamma\) and facts \(\Phi\) from the running example~\eqref{eqn:forward_chaining}: the proof states \(s_0, s_1, s_2, s_3\) from forward chaining should match those generated by \(\mcal{R}\) on \(X_0 = \msf{Enc}(\Gamma, \Phi)\), provided that \(\mcal{R}\) has correctly learned logical inference.
}
\label{fig:one_inference_step}
\end{figure*}



==> mains/neurips_checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All claims made in our paper are supported by theoretical proofs or rigorous empirical evaluations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss some limitations in the Discussion and also in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our main paper has some informal theorem statements for ease of readability, however, we give formal versions of all the statements with full proofs in \cref{app:theory}. We also make sure to clarify the assumptions under which our results hold.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix~\ref{sec:experiment_details} contains all necessary information for reproducing the experimental results. This includes details of the datasets and the dataset creation process (~\ref{sec:mc_dataset_and_finetuning},~\ref{sec:llama_details}), model fine-tuning (~\ref{sec:mc_ft_details}), attack setup and implementation (\ref{sec:mc_attack_setup_appendix},~\ref{sec:gcg_details}) and attack evaluation (~\ref{sec:suppression_details},~\ref{sec:coercion_amnesia_details}). We also provide scripts to reproduce the experimental results as artifacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We release code used for all experiments in the paper along with a README file with instructions on reproducing the results. We use two datasets for evaluation: the first can be generated using steps described in Appendix~\ref{sec:mc_dataset_and_finetuning} and the second has 15 examples which are all listed in Table~\ref{tab:llama_dataset}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We present the main setting details in Section~\ref{sec:experiments}. We additionally provide training and testing details in Appendix~\ref{sec:experiment_details}: hyperparameters associated with GPT-2 finetuning are presented in ~\ref{sec:mc_ft_details} and the GCG algorithm setup in ~\ref{sec:gcg_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report the mean and standard deviation over multiple runs for all metrics with elements of randomness. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The compute details for the GPT-2 finetuning and GCG attacks are presented in Appendix~\ref{sec:mc_ft_details} and Appendix~\ref{sec:gcg_details} respectively.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We read the code of ethics in its entirety and strongly believe that our research abides by the stated code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss both the positive and negative broader impacts in the Discussion as well as the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not train new large language models, but use them in our experiments. We therefore warn the user about the potential risks of using LLMs in the code documentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assets are appropriately credited. The implementation code is available in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include the source code for our experiments and datasets in the supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not use crowd-sourced data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not use participant studies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> old/abstract_1.tex <==
\begin{abstract}

We study how to subvert language models from following the rules.
We model rule-following as inference over propositional Horn logic, a mathematical system in which rules have the form \textit{``if $P$ and $Q$, then $R$''} for some propositions $P$, $Q$, and $R$.
We prove that although transformers can faithfully abide by such rules, maliciously crafted prompts can nevertheless mislead even theoretically constructed models.
Empirically, we find that attacks on our theoretical models mirror popular attacks on large language models.
Our work suggests that studying smaller theoretical models can help understand the behavior of large language models in rule-based settings like logical reasoning and jailbreak attacks.


% We study how to attack the logical reasoning of language models.
% We focus on \emph{propositional Horn logic}, a simple mathematical logic wherein rules have the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\), and \(R\).
% We show that although even small transformers can exactly encode propositional reasoning, such ``theoretically exact'' reasoners can nevertheless output logical fallacies when given maliciously crafted prompts.
% Interestingly, we find that reasoning attacks against large language models induce similar attention patterns as those investigated in our theory of small models.
% This suggests that successful reasoning attacks on both small and large models may share common strategies.
% In particular, if the attention mechanism is easily manipulated, then logical fallacies are easily generated.


% We study how to jailbreak the logical reasoning of language models.
% We focus on \emph{propositional Horn logic}, a simple mathematical logic wherein rules have the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\), and \(R\).
% Although even small transformers have the capacity to encode propositional reasoning, we show that even these ``exact reasoners'' can deduce logical fallacies via carefully constructed attacks.
% Interestingly, we find that jailbreaks against large language models induce similar attention patterns as those investigated in our theory of small models.
% This suggests that successful reasoning jailbreaks on both small and large models may share common strategies.
% In particular, if the attention mechanism is easily manipulated, then logical fallacies are easily generated.



% We study the reasoning power of transformer-based language models over \emph{propositional Horn logic},
% a mathematical logic wherein rules take the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\), and \(R\).
% We prove that transformers with chain-of-thought reasoning can encode propositional inference using only one layer, one self-attention head, and an embedding dimension linear in the number of propositions.
% Empirically, we find that the performance trend of learned reasoners matches our theoretical predictions.
% Furthermore, we show that neither our theoretical nor learned models are robust reasoners: even highly accurate models can be tricked into logical fallacies and fail to generalize out of distribution.


% We study the reasoning power of transformer-based language models over \emph{propositional Horn logic},
% a mathematical logic wherein rules take the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\), and \(R\).
% We prove that transformers with chain-of-thought reasoning can encode propositional inference using only one layer, one attention head, and an embedding dimension linear in the number of propositions.
% Empirically, we find that the performance trend of learned reasoners matches our theoretical predictions.
% Furthermore, we show that neither our theoretical nor learned models are robust reasoners: even seemingly perfect reasoners can be tricked into logical fallacies.




% Empirically, we find that one-layer, one-head transformers can learn to reason with \(99\%+\) accuracy, and that this performance is linear in the embedding dimension.


% Furthermore, we probe the weaknesses and failure modes of models that learn to reason: we find that in both theory and practice, it is easy to attack even highly accurate models.


% Chain-of-thought prompting is a technique for improving the reasoning performance of large language models (LLMs).
% Despite much recent progress, the reasoning power and limitations of Large Language Models (LLMs) remain poorly understood.

% Our investigation of LLM reasoning over this simple yet foundational fragment establishes the groundwork for future investigations into more complex logics.


% Moreover, we investigate the robustness of our theoretical and learned constructions and show that both are susceptible to adversarial attacks.




% This document provides a basic paper template and submission guidelines.
% Abstracts must be a single paragraph, ideally between 4--6 sentences long.
% Gross violations will trigger corrections at the camera-ready phase.
\end{abstract}

==> old/autoreg_example.tex <==
\begin{figure*}[ht]
\centering


\includegraphics[width=0.8\linewidth]{images/autoreg.png}

\caption{
\red{Text about the autoregressive loop}
}
\label{fig:autoreg_example}
\end{figure*}



==> old/background_1.tex <==


\section{Background}
\label{sec:background}

In Section~\ref{sec:background_logical_inference}, we first give the necessary background on propositional Horn logic.
Then, in Section~\ref{sec:background_llm}, we present the mathematical formalization of LLMs in~\eqref{eqn:llm}, with a focus on the transformer module in~\eqref{eqn:tf}.
Finally, in Section~\ref{sec:background_autoreg}, we give an implementation of chain-of-thought reasoning as an autoregressive evaluation loop in~\eqref{eqn:autoreg}.
% Finally, in Section~\ref{sec:background_logical_inference}, we state the task of logical inference in propositional Horn logic in Problem~\ref{prob:propositional_inference}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reasoning in Propositional Horn Logic}
\label{sec:background_logical_inference}

We formulate the task of logical reasoning as follows.

\begin{problem}[Logical Reasoning]
\label{prob:reasoning}
    Consider some rules \(\Gamma\), facts \(\Phi\), and query \(\tau\).
    Is \(\tau\) logically entailed by \(\Gamma\) and \(\Phi\)?
\end{problem}

We make the above concrete in the remainder of this Section, and for now, give an example in Figure~\ref{fig:inference_example} that considers the following set of rules:
\begin{align} \label{eqn:gamma_example}
    \Gamma =
        \{A \rightarrow B, \enskip
        B \rightarrow C, \enskip
        A \land C \rightarrow D\}
\end{align}
with propositions \(A, B, C, D\).
Propositions are mathematical objects like \(\msf{Rainy}\) or \(\msf{Cloudy}\) that represent assertions of truth and are the building blocks of propositional logic.
For instance, the third rule reads: \emph{if \(A\) and \(C\) hold, then \(D\) holds}.
Suppose we are now given the facts \(\Phi = \{A\}\), can we derive the query \(\tau = D\)?
That is, if we know proposition \(A\) holds, we must decide whether \(D\) must also hold.
Figure~\ref{fig:inference_example} presents a basic reasoning mechanism: one tracks what propositions are proven so far and iteratively applies the rules to derive new ones until either the query is subsumed or the possible actions are exhausted.



Propositional Horn logic is so called because the rules \(\gamma \in \Gamma\) take the form:
\begin{align} \label{eqn:horn_rule}
    \gamma = (A_1 \land \ldots \land A_k
    \enskip \to \enskip B_1 \land \ldots \land B_m)
\end{align}
for some propositions \(A_1, \ldots, A_k\) that constitute the \emph{antecedent} and some propositions \(B_1, \ldots, B_m\) that make up the \emph{consequent}.
The facts \(\Phi\) are also given as propositions \(\Phi = \{F_1, \ldots, F_p\}\), and the query is a conjunction \(\tau = Q_1 \land \ldots \land Q_q\).
Observe that in Propositional Horn logic, we can only prove that some proposition \(P\) \emph{holds} (i.e., proven) or is \emph{unknown}.
Because the syntax of Horn rules lacks negation in the appropriate places, we \emph{cannot} prove \(P\) to be false.
This simplifying restriction is what allows propositional Horn logic to have a polynomial-time decision procedure, an algorithm of which is sketched in Figure~\ref{fig:inference_example}.


In order to formally talk about deriving new propositions and proving queries, we now present our mathematical formulation of propositional Horn logic.
Suppose that our universe consists of some \(n \geq 1\) propositions \(P_1, \ldots, P_n\).
A \emph{rule} is a pair of binary vectors \((\alpha, \beta) \in \mbb{B}^n \times \mbb{B}^n\), where \(\alpha\) is the antecedent and \(\beta\) is the consequent.
A \emph{query} is a binary vector \(\tau \in \mbb{B}^n\).
We use binary vector to encode conjunctions, and interpret \(\alpha \in \mbb{B}^n\) as semantically equivalent to \(\bigwedge\{P_i : \alpha_i = 1\}\).


Because propositional Horn logic lacks negation, for some \(\alpha \in \mbb{B}^n\), we use \(\alpha_i = 1\) to denote the presence of \(P_i\)

Because propositional Horn logic lacks negation, we use \(1\) to denote the presence of \(P_i\) in a conjunction, and use \(0\) denote the absence




\begin{definition}
Let \(\Gamma\) be a set of Horn rulies 

\end{definition}




\red{AAAAAAAAAA}

Broadly speaking, the problem of \emph{logical inference} is concerned with deducing new facts from existing knowledge.
We study the decision variant of this problem, wherein the task is to check whether a query \(\tau\) is deducible from a set of rules \(\Gamma\) with respect to some inference mechanism.
That is, we wish to check whether \(\Gamma\) logically entails \(\tau\).
The decision variant of logical inference is sometimes known as \emph{theorem-proving}, in which case the query \(\tau\) is referred to as the \emph{theorem}.
We follow this convention to formulate the problem below.
\begin{problem}[Logical Inference]
\label{prob:propositional_inference}
Let \(\Gamma\) be a set of Horn rules and \(\tau\) be a query.
Decide whether \(\Gamma \vDash \tau\).
\end{problem}
In the remainder, we make each term of the above concrete.
We introduce propositional Horn logic and our binary vector-based representation, as well as present a rigorous definition of logical entailment in Definition~\ref{def:entailment}.

We begin with establishing a basic vocabulary to discuss the truthiness of logical assertions.
In propositional logic, this basic vocabulary is called the \emph{atoms}, which one may think of as discrete objects that represent descriptions.
Such descriptions may include objects such as \textsf{IsDuck}, \textsf{HasWings}, \textsf{IsTasty}, and so on.
Propositional atoms are the building blocks of logical sentences, also known as formulas, used to assert truths.
Before continuing, we make two important assumptions.
First, we assume that there \(n\) propositional atoms in our universe, which will allow us to use binary vectors of size \(O(n)\) to describe formulas.
Next, we assume that formulas take one of the two following forms:
\begin{itemize}
    \item (Facts)
    A \emph{fact} is an assertion that one or more atoms simultaneously hold.
    We represent this conjunction with binary vectors \(\alpha \in \mbb{B}^n\), where \(\alpha_i = 1\) means that we assert the \(i\)th atom to hold.
    In this logical fragment, we do not have negation, so \(\alpha_j = 0\) means that we do \emph{not} assert the \(j\)th atom to hold.

    \item (Rules)
    A \emph{rule} describes how new facts may be derived from existing facts.   
    We can express this as a pair of binary vectors \((\alpha, \beta) \in \mbb{B}^n \times \mbb{B}^n\), where \(\alpha\) is the \emph{antecendent} and \(\beta\) is the \emph{consequent}.
    Intuitively, such a rule means that if we can derive the truthiness of each atom indicated by \(\alpha\), then we can conclude the truthiness of each atom indicated \(\beta\).
\end{itemize}

Formulas that are either facts or rules are called \emph{Horn clauses}, which we represent using binary vectors as above.
A set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) where each \(\gamma_i\) is as above is then called a set of \emph{Horn rules}.
We reform to the fragment of propositional logic restricted to such syntactic form as \emph{propositional Horn logic}.

We emphasize two important features of this logical fragment.
First, we cannot assert that an atom is false; we can only say that an atom is \emph{positive} or \emph{unknown}, represented by \(1\) and \(0\), respectively.
Second, our inference mechanism and the form of our rules do not introduce branching factors that would lead to combinatorial explosion challenges typical of decision problems in logic.
These yield polynomial-time decision procedures for Problem~\ref{prob:propositional_inference}~\cite{levesque1986knowledge}; a basic algorithm is sketched in Section~\ref{sec:theory_autoregressive}.
Note that this computational complexity is in contrast to logical inference in full proportional logic, which is \textsc{NP-Complete}.


\begin{remark}
Given a rule \(\gamma = (\alpha, \beta) \in \mbb{B}^n \times \mbb{B}^n\), it is common for texts to assume that \(\norm{\beta}_1 = 1\), i.e., that there is a single atom that is asserted in the consequent, where here \(\norm{\cdot}_1\) is the \(\ell^1\) norm.
In such restricted cases, a rule is sometimes called a \emph{definite clause}.
Some texts also require a \emph{goal clause} that encodes the query \(\tau\) as a third form, but this is not necessary depending on the formulation of the logical inference problem.
\end{remark}


Given two binary vectors \(\alpha, \alpha' \in \mbb{B}^n\), we write \(\alpha \preceq \alpha'\) to mean that \(\alpha_i \leq \alpha_i '\) for each \(i = 1, \ldots, n\).
This partial ordering is useful for testing logical implication: suppose that at some intermediate state of our logical inference procedure, we are able to conclude facts \(z \in \mbb{B}^n\) about the world.
To check whether a rule \(\gamma = (\alpha, \beta) \in \mbb{B}^n \times \mbb{B}^n\) is applicable via \emph{modus ponens}, we may check whether \(\alpha \preceq z\).


We now make a simplifying assumption, namely that we take the empty conjunction \(\mbf{0}_n \in \mbb{B}^n\) to be vacuously truthy.
We use this to equivalently represent a fact \(\alpha \in \mbb{B}^n\) as a rule \((\mbf{0}_n, \alpha)\), which allows us to discuss logical inference in terms of only rules.
This now gives us the vocabulary to discuss logical entailment in the Horn fragment of propositional logic, which we define below in a recursive manner.

\begin{definition} \label{def:entailment}
Let \(\Gamma\) be a set of Horn rules and consider some \(\tau \in \mbb{B}^n\).
Then \(\Gamma \vDash \tau\) iff: for each \(i\) where \(\tau_i = 1\) there exists \(\gamma = (\alpha, \beta) \in \Gamma\) where \(\beta_i = 1\) and \(\Gamma \setminus \{\gamma\} \vDash \alpha\).
\end{definition}

This completes the definition of the terms presented in Problem~\ref{prob:propositional_inference}.
In summary, we wish to check whether a query \(\tau \in \mbb{B}^n\) is deducible from a set of Horn rules \(\Gamma\), i.e., whether \(\Gamma \vDash \tau\), where the inference mechanism is modus ponens, and logical entailment is recursively defined as above.



\input{figures/autoreg_example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transformer-Based Sequence Classification Models}
\label{sec:background_llm}

Our mathematical formalism treats LLMs as sequence classification models \(\msf{LLM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\), which take as input a \emph{token sequence} \(u_1, \ldots, u_N \in \mbb{R}^{d_{\msf{in}}}\) and produce an output label \(v \in \mbb{R}^{d_{\msf{out}}}\).
We focus on transformer-based LLMs, which commonly consist of three modules --- the embedding function, the transformer module, and the classification head ---
expressed as follows:
\begin{align} \label{eqn:llm}
    \msf{LLM}:
    U
    \xrightarrow{\msf{Embed}} X
    \xrightarrow{\msf{Tf}} Y
    \xrightarrow{\msf{ClsHead}} v
\end{align}
Here \(U = \msf{stack}(u_1, \ldots, u_N) \in \mbb{R}^{N \times d_{\msf{in}}}\) is the input token sequence stacked as rows.
Next, \(\msf{Embed} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{N \times d}\) is an affine function that maps \(U\) to the \emph{embedded inputs} \(X = \msf{stack}(x_1, \ldots, x_N) \in \mbb{R}^{N \times d}\), where \(d\) is called the \emph{embedding dimension}.
If positional encodings are used, they may be expressed as part of \(\msf{Embed}\).
The transformer \(\msf{Tf} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) is a sequence-valued function that returns an output \(Y = \msf{stack}(y_1, \ldots, y_N) \in \mbb{R}^{N \times d}\).
Finally, the classification head \(\msf{ClsHead}: \mbb{R}^{d} \to \mbb{R}^{d_{\msf{out}}}\) is an affine function that acts on the last element of \(Y\) via \(v = \msf{ClsHead}(y_N)\), while ignoring the first \(y_1, \ldots, y_{N-1}\) terms.
The choice to act on the last term is informed by the use of causal attention that we later describe.


The transformer module, \(\msf{Tf}\), is commonly defined as an alternating sequence of attention and feedforward blocks.
An \(L\)-layer transformer has the form:
\begin{align} \label{eqn:tf}
    \msf{Tf}(X) = (\msf{Layer}_L \circ \cdots \circ \msf{Layer}_1)(X)
\end{align}
where each \(\msf{Layer}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of an attention block composed into a feedforward block:
\begin{align} \label{eqn:tf_layer}
    \msf{Layer}_k (X)
        = ((\msf{Id} + \msf{Ffwd}_k) \circ (\msf{Id} + \msf{Attn}_k))(X)
\end{align}
where \(\msf{Id}\) is the identity block that implements a residual connection.
We assume that the same feedforward block \(\msf{Ffwd}_k : \mbb{R}^{d} \to \mbb{R}^{d}\) is applied in parallel to each term of the \(N\)-length sequence.
Moreover, we assume that the feedforward block of each layer is only 1-hidden unit deep and takes the form:
\begin{align} \label{eqn:tf_ffwd}
    \msf{Ffwd}_k (x)
    = W_{k2} \sigma (W_{k1} x + b_{k1}) + b_{k2},
\end{align}
with parameters \(W_{k1}, W_{k2}^{\top} \in \mbb{R}^{d_{\msf{ffwd}} \times d}\), \(b_{k1} \in \mbb{R}^{d_{\msf{ffwd}}}\), and \(b_{k2} \in \mbb{R}^{d}\), and \(\sigma\) is some activation function that we assume to be \(\msf{ReLU}\).
Here \(d_{\msf{ffwd}}\) is the feedforward width that is commonly taken to be \(d_{\msf{ffwd}} = 4d\) or some large constant.
An attention block \(\msf{Attn}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) with \(H\) heads with causal attention has form:
\begin{align*}
% \label{eqn:tf_attn}
    % \msf{Attn}_k (X)
    % & = \sum_{h = 1}^{H} \msf{CausalSoftmax}(XW_{Qkh}  W_{Kkh} ^\top X^\top) X W_{Vkh}
    &\msf{Attn}_k (X) = \sum_{h = 1}^{H} \msf{CausalSoftmax}(Q_{kh} K_{kh} ^\top) V_{kh} \\
    Q_{kh} &= X W_{Qkh},
    \quad K_{kh} ^\top = W_{Kkh} ^\top X^\top,
    \quad V_{kh} = X W_{Vkh}
\end{align*}
with parameters \(W_{Qkh}, W_{Kkh} ^\top \in \mbb{R}^{d \times d_{\msf{attn}}}\) and \(W_{Vkh} \in \mbb{R}^{d \times d}\) for heads \(h = 1, \ldots, H\).
Note that it suffices to take \(d_{\msf{attn}} \leq d\).
Here, \(\msf{CausalSoftmax}: \mbb{R}^{N \times N} \to \mbb{R}^{N \times N}\) is the causal variant of row-wise softmax defined as follows:
\begin{align}
\label{eqn:causal_softmax}
\begin{split}
    &\msf{CausalSoftmax}(Z) \\
    &= \begin{bmatrix}
        \msf{Softmax}( z_{11}, & -\infty, & \cdots, & -\infty) \\
        \msf{Softmax}( z_{21}, & z_{22}, & \cdots, & -\infty) \\
        \vdots & \vdots & \ddots & \vdots \\
        \msf{Softmax}( z_{N1}, & z_{N2}, & \cdots, & z_{NN})
    \end{bmatrix}
\end{split}
\end{align}
where \(z_{ij}\) is the \((i,j)\)th entry of the parameter \(Z \in \mbb{R}^{N \times N}\) and \(\msf{Softmax} : \mbb{R}^{N} \to \mbb{R}^{N}\) is given as:
\begin{align}
\label{eqn:softmax}
    \msf{Softmax}(a_1, \ldots, a_N)
    &= \frac{\parens*{e^{a_1}, \ldots, e^{a_N}}}{e^{a_1} + \cdots + e^{a_N}}
    \in \mbb{R}^{N}
\end{align}
Observe that \(-\infty\) to an argument of \(\msf{Softmax}\) makes the corresponding position zero.
\(\msf{CausalSoftmax}(Z)\) is thus a lower-triangular matrix with zeros strictly above the diagonal, i.e., \(\msf{CausalSoftmax}(Z)_{ij} = 0\) iff \(j > i\).
Note that our formalism omits the layer normalization, which is typically applied after each attention block and after each feedforward block.
This omission does not change the fundamental expressive power of a transformer~\cite{liu2022transformers} and serves to simplify the theoretical analysis.
Moreover, although the transformer must fix apriori various quantities like \(d, d_{\msf{ffwd}}, d_{\msf{attn}}\), the sequence may be of any length \(N\) --- though in practice there is often an upper bound \(N_{\msf{max}} > N\) due to limitations in the choice of positional encoding.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Autoregressive Evaluation of LLMs}
\label{sec:background_autoreg}

Having defined the transformer-based sequence classification model, \(\msf{LLM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\), we next formalize autoregressive evaluation.
This style of evaluation is central to many CoT reasoning strategies and can be defined using the following set of recursive equations:
\begin{align} \label{eqn:autoreg}
\begin{split}
    U_0 &= \msf{stack}(u_1, \ldots, u_N) \\
    v_t &= \msf{LLM}(U_{t-1}) \\
    U_{t} &= \msf{stack}(U_{t-1}, \msf{Tokenizer}(v_t))
\end{split}
\end{align}
Beginning with some initial \(U_0\), one generates a sequence of sequences \(U_1, U_2, \ldots\) of increasing lengths by iteratively appending tokenizations of \(v_t\) onto \(U_{t-1}\) to form \(U_{t}\).
This continues until some stopping condition is reached, for instance, if some maximum step budget is reached or if some \(\msf{Tokenizer}(v_t)\) returns an \(\msf{EOS}\) token that indicates termination.
In the autoregressive loop above, the labels \(v_1, v_2, \ldots\) represent the intermediate reasoning steps of CoT evaluation.
The algorithmic schema of~\eqref{eqn:autoreg} captures the core structure of autoregressive computation, though one must make sure to appropriately define the stopping conditions and the \(\msf{Tokenizer}: \mbb{R}^{d_{\msf{out}}} \to \mbb{R}^{d_{\msf{in}}}\) function.







==> old/background_2.tex <==

\input{figures/autoreg}

\section{Background and problem setup}
\label{sec:background}

In Section~\ref{sec:background_reasoning}, we first give the necessary background on propositional Horn logic.
Then, in Section~\ref{sec:background_lm}, we present the mathematical formalization of language models with a focus on the sequence-to-sequence transformer module.
% Finally, in Section~\ref{sec:background_autoreg}, we formalize autoregressive evaluation, which is central to CoT reasoning methods.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reasoning in propositional Horn logic}
\label{sec:background_reasoning}

A standard task in logical reasoning is to check whether some goal is the consequence of some given facts and rules.
For instance, consider Figure~\ref{fig:mc_inference}, where we have expanded the previous example from Minecraft~\cite{mojang2011minecraft}.
In particular, the recipe list (rules) specifies which combination of items are necessary to make new ones, which we formalize in the language of propositional logic as follows:
\begin{gather*}
    \Gamma = \{
        \msf{Sheep} \rightarrow \msf{Wool},
        \enskip
        \msf{Wool} \rightarrow \msf{String}, \\
    \msf{Wood} \rightarrow \msf{Stick},
        \enskip
        \msf{Stick} \, \text{and}\, \msf{String} \rightarrow \msf{FishingRod}
    \}
\end{gather*}
where \(\msf{Sheep}\), \(\msf{Wool}\), etc are \emph{propositions} that represent the statements ``I can get \(\msf{Sheep}\)'', ``I can get \(\msf{Wool}\)'', etc.
The reasoning task is to answer whether the goal \(\tau = \msf{FishingRod}\) is reachable from some given facts \(\Phi = \{\msf{Sheep}, \msf{Wood}\}\) by repeatedly applying the inference rules \(\Gamma\).
Figure~\ref{fig:mc_inference} shows this process in action: we derive a sequence of \emph{proof states} \(s_0, s_1, s_2, s_3\) where each successive state is generated by applying \(\Gamma\) to the previous ones.
Because \(s_3\) subsumes \(\tau\), we may conclude that a fishing rod is within reach.
More generally, we formulate logical reasoning as follows.
\begin{problem}[Logical Reasoning]
\label{prob:logical_reasoning}
    Given rules \(\Gamma\), facts \(\Phi\), and goal \(\tau\):
    decide whether \(\Gamma\) and \(\Phi\) logically entail \(\tau\).
\end{problem}

We now present the notation to discuss logical reasoning.
Let \(\mbb{B} = \{0,1\}\) and assume that our universe consists of \(n \geq 1\) propositions \(P_1, \ldots, P_n\) whose conjunctions are represented by binary vectors in \(\mbb{B}^n\).
In particular, \(\alpha \in \mbb{B}^n\) denotes the conjunction \(\bigwedge \{P_i : \alpha_i = 1\}\).
Observe that \(\alpha_i = 0\) marks the absence of \(P_i\), which is not to be confused with negation!
A \emph{rule} is a pair of binary vectors \((\alpha, \beta) \in \mbb{B}^{2n}\),
where \(\alpha\) (the antecedent) specifies what conditions must be met for the rule to be applied, and \(\beta\) (the consequent) specifies what propositions may be derived if the rule is applied.
A \emph{goal} is a binary vector \(\tau \in \mbb{B}^n\).
We take the convention that an empty conjunction \(\mbf{0}_n \in \mbb{B}^n\) trivially holds, which allows us to model a fact \(\varphi \in \mbb{B}^n\) as the rule \((\mbf{0}_n, \varphi) \in \mbb{B}^{2n}\).


Consider the example of Figure~\ref{fig:mc_inference} and index the \(n = 6\) propositions by their order in the final proof state \(s_3\).
Let \(e_1, \ldots, e_6 \in \mbb{B}^{n}\) be the basis vectors, then we may write:
\begin{align*}
    \Gamma = \{
        (e_1, e_3),
        \enskip (e_3, e_5),
        \enskip (e_2, e_4),
        \enskip (e_4 + e_5, e_6)
    \}
\end{align*}
with facts \(\Phi = \{e_1, e_2\}\) and goal \(\tau = e_6\).
Beginning from \(s_0 = e_1 + e_2\),
the proof states are respectively binarized as:
\begin{align*}
    s_1 = s_0 + e_3 + e_4,
    \quad s_2 = s_1 + e_5,
    \quad s_3 = s_2 + e_6
    % s_0 = e_1 + e_2,
    % &\qquad s_1 = s_0 + e_3 + e_4, \\
    % s_2 = s_1 + e_5,
    % &\qquad s_3 = s_2 + e_6
\end{align*}
We may also rewrite the facts \(\Phi\) as rules using the aforementioned convention of empty conjunctions.
Under this scheme, we take the initial proof state to be \(s_0 = \mbf{0}_n\) and include the inference rule \((\mbf{0}_n, e_1 + e_2)\) into \(\Gamma\), for a total of \(r = 5\) rules.
This rewrite of \(\Phi\) allows us to define entailment in terms of only \(\Gamma\) and \(\tau\),
which is typically presented in a recursive manner.


Our main challenge is to encode a language model that can perform one step of reasoning.
To approach this, we first consider rule application.
Given some proof state \(s \in \mbb{B}^n\) and rule \((\alpha, \beta) \in \Gamma\): if \(s\) subsumes \(\alpha\), then we may conclude that \((s \lor \beta) \in \mbb{B}^n\), where disjunction is defined coordinate-wise for binary vectors.
We may then view a single reasoning step with respect to \(\Gamma\) as the simultaneous application of all rules, for which we overload notation to express as follows:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where for two vectors, \(x \preceq y\) iff each \(x_i \leq y_i\).
Under this notation, we view \(\Gamma\) as a set \(\Gamma \subseteq \mbb{B}^{2n}\) and also as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
Here, \(\Gamma(s)\) represents the aggregate result of all rule applications: if a rule \((\alpha, \beta) \in \Gamma\) satisfies the subsumption \(\alpha \preceq s\), then we include the propositions of \(\beta\) using a disjunction.
Starting at some initial proof state \(s_0 \in \mbb{B}^n\), we may repeatedly apply \(\Gamma: \mbb{B}^n \to \mbb{B}^n\) to generate a sequence of proof states:
\begin{align} \label{eqn:state_seq}
    s_0 \xrightarrow{\Gamma}
    s_1 \xrightarrow{\Gamma}
    s_2 \xrightarrow{\Gamma}
    \cdots
\end{align}
Observe that \(s_0 \preceq s_1 \preceq s_2 \preceq \ldots\) by definition of \(\Gamma\).
Moreover, because there are \(n\) propositions: to check whether \(\Gamma\) entails the goal \(\tau\), it suffices to check whether \(\tau \preceq s_n\).


\begin{definition}[Entailment] \label{def:logical_entailment}
    The rule set \(\Gamma\) entails the goal \(\tau \in \mbb{B}^n\) iff:
    for each \(i\) where \(\tau_i = 1\) there exists \((\alpha, \beta) \in \Gamma\) such that \(\beta_i = 1\) and the rule set \(\Gamma \setminus \{(\alpha, \beta)\}\) entails \(\alpha\).
\end{definition}

Although our formulations above differ from classical presentations of propositional Horn logic~\cite{levesque1986knowledge},
we do not lose any fundamental expressive power.
We give a further discussion on this in Section~\ref{sec:discussion_logic}.


% Furthermore, we remark that in propositional Horn logic, one cannot prove a proposition \(P\) to be false: we can only show that \(P\) either holds or is unknown, represented by \(1\) and \(0\), respectively.

% This simplicity yields polynomial-time algorithms for Problem~\ref{prob:logical_reasoning}~\citep{levesque1986knowledge}, an example of which is sketched above in Figure~\ref{fig:mc_inference} and described in detail later in Section~\ref{sec:theory_autoregressive}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transformer-based language models}
\label{sec:background_lm}

Our mathematical formalism treats language models as sequence classification models \(\msf{LM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\), which take as input a \emph{token sequence} \(u_1, \ldots, u_N \in \mbb{R}^{d_{\msf{in}}}\) and produce an output label \(s \in \mbb{R}^{d_{\msf{out}}}\).
We focus on transformer-based language models, which commonly consist of three modules --- the embedding function, the transformer module, and the classification head ---
expressed as follows:
\begin{align} \label{eqn:lm}
    \msf{LM}:
    U
    \xrightarrow{\msf{Embed}} X
    \xrightarrow{\msf{Transformer}} Y
    \xrightarrow{\msf{ClsHead}} s
\end{align}
where \(U = \msf{append}(u_1, \ldots, u_N) \in \mbb{R}^{N \times d_{\msf{in}}}\) is a stacked representation of the input tokens.
With embedding dimension \(d\), let \(X \in \mbb{R}^{N \times d}\) be the embedded input sequence let and \(Y \in \mbb{R}^{N \times d}\) be the embedded output sequence.
We define an \(L\)-layer transformer as:
\begin{align*}
% \label{eqn:tf}
    \msf{Transformer}(X) = (\msf{Layer}_L \circ \cdots \circ \msf{Layer}_1)(X)
\end{align*}
where each \(\msf{Layer}_l : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of a causal self-attention block composed with a feedforward block:
\begin{align*}
% \label{eqn:tf_layer}
    \msf{Layer}_l (X)
        = ((\msf{Id} + \msf{Ffwd}_l) \circ (\msf{Id} + \msf{Attn}_l))(X)
\end{align*}
with residual connections implemented using the identity operator \(\msf{Id}\).
We give additional details in Appendix~\ref{sec:theory_construction}.





% We first stack the input tokens as \(U = \msf{append}(u_1, \ldots, u_N) \in \mbb{R}^{N \times d_{\msf{in}}}\).
% Then, we pass \(U\) to \(\msf{Embed}: \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{N \times d}\), which is an affine function, in order to yield the \emph{embedded inputs} \(X \in \mbb{R}^{N \times d}\).
% This is passed to \(\msf{Transformer}: \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\).


% is an affine function that maps \(U\) to the \emph{embedded inputs} \(X = \msf{append}(x_1, \ldots, x_N) \in \mbb{R}^{N \times d}\), where \(d\) is called the \emph{embedding dimension}.
% If positional encodings are used, they may be expressed as part of \(\msf{Embed}\).
% The transformer \(\msf{Tf} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) returns a sequence \(Y = \msf{append}(y_1, \ldots, y_N) \in \mbb{R}^{N \times d}\).
% Finally, the classification head \(\msf{ClsHead}: \mbb{R}^{d} \to \mbb{R}^{d_{\msf{out}}}\) is an affine function that acts on the last element of \(Y\) via \(s = \msf{ClsHead}(y_N)\), while ignoring the first \(y_1, \ldots, y_{N-1}\) terms because we use causal self-attention.
% Finally, an \(L\)-layer transformer has form:
% \begin{align} \label{eqn:tf}
%     \msf{Transformer}(X) = (\msf{Layer}_L \circ \cdots \circ \msf{Layer}_1)(X)
% \end{align}
% where each \(\msf{Layer}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of a causal self-attention block and a feedforward block.
% We give a more detailed architecture description in Appendix~\ref{sec:theory_construction}.


% where each \(\msf{Layer}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of an attention block composed into a feedforward block:
% \begin{align} \label{eqn:tf_layer}
%     \msf{Layer}_k (X)
%         = ((\msf{Id} + \msf{Ffwd}_k) \circ (\msf{Id} + \msf{Attn}_k))(X)
% \end{align}

% where \(\msf{Id}\) is the identity block that implements a residual connection.
% The same feedforward block \(\msf{Ffwd}_k : \mbb{R}^{d} \to \mbb{R}^{d}\) is applied in parallel to each term of the \(N\)-length sequence.
% Moreover, the feedforward block of each layer is only 1-hidden unit deep and so takes the form:
% \begin{align} \label{eqn:tf_ffwd}
%     \msf{Ffwd}_k (x)
%     = W_{k2} \sigma (W_{k1} x + b_{k1}) + b_{k2},
% \end{align}
% with parameters \(W_{k1}, W_{k2}^{\top} \in \mbb{R}^{d_{\msf{ffwd}} \times d}\), \(b_{k1} \in \mbb{R}^{d_{\msf{ffwd}}}\), and \(b_{k2} \in \mbb{R}^{d}\), and \(\sigma\) is some activation function that we assume to be \(\msf{ReLU}\).
% Here \(d_{\msf{ffwd}}\) is the feedforward width that is commonly taken to be \(d_{\msf{ffwd}} = 4d\) or some large constant.
% An attention block \(\msf{Attn}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) with \(H\) heads with causal attention has form:
% \begin{gather*}
%     \msf{Attn}_k (X) = \sum_{h = 1}^{H} \msf{CausalSoftmax}(Q_{kh} K_{kh} ^\top) V_{kh} \\
%     Q_{kh} = X W_{Qkh},
%     \quad K_{kh} ^\top = W_{Kkh} ^\top X^\top,
%     \quad V_{kh} = X W_{Vkh}
% \end{gather*}
% with parameters \(W_{Qkh}, W_{Kkh} ^\top \in \mbb{R}^{d \times d_{\msf{attn}}}\) and \(W_{Vkh} \in \mbb{R}^{d \times d}\) for heads \(h = 1, \ldots, H\).
% Note that it suffices to take \(d_{\msf{attn}} \leq d\).
% Here, \(\msf{CausalSoftmax}: \mbb{R}^{N \times N} \to \mbb{R}^{N \times N}\) is the causal variant of row-wise softmax defined as follows:
% \begin{align*}
%     &\msf{CausalSoftmax}(Z) \\
%     &= \begin{bmatrix}
%         \msf{Softmax}( z_{11}, & -\infty, & \cdots, & -\infty) \\
%         \msf{Softmax}( z_{21}, & z_{22}, & \cdots, & -\infty) \\
%         \vdots & \vdots & \ddots & \vdots \\
%         \msf{Softmax}( z_{N1}, & z_{N2}, & \cdots, & z_{NN})
%     \end{bmatrix}
% \end{align*}
% where \(z_{ij}\) is the \((i,j)\)th entry of the parameter \(Z \in \mbb{R}^{N \times N}\) and \(\msf{Softmax} : \mbb{R}^{N} \to \mbb{R}^{N}\) is given as:
% \begin{align*}
%     \msf{Softmax}(a_1, \ldots, a_N)
%     &= \frac{\parens*{e^{a_1}, \ldots, e^{a_N}}}{e^{a_1} + \cdots + e^{a_N}}
%     \in \mbb{R}^{N}
% \end{align*}
% Observe that \(-\infty\) to an argument of \(\msf{Softmax}\) makes the corresponding position zero.
% \(\msf{CausalSoftmax}(Z)\) is thus a lower-triangular matrix with zeros strictly above the diagonal, i.e., \(\msf{CausalSoftmax}(Z)_{ij} = 0\) iff \(j > i\).
% Note that our formalism omits the layer normalization, which is typically applied after each attention block and after each feedforward block.
% This omission does not change the fundamental expressive power of a transformer~\cite{liu2022transformers} and serves to simplify the theoretical analysis.
% Moreover, although the transformer must fix apriori various quantities like \(d, d_{\msf{ffwd}}, d_{\msf{attn}}\), the sequence may be of any length \(N\) --- though in practice there is often an upper bound \(N_{\msf{max}} \geq N\) due to limitations in the choice of positional encoding.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Autoregressive Evaluation of Language Models}
% \label{sec:background_autoreg}

% Having defined the transformer-based sequence classification model, \(\msf{LM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\), we next formalize autoregressive evaluation.
% This style of evaluation is central to many CoT reasoning strategies and can be defined using the following set of recursive equations:
% \begin{align} \label{eqn:autoreg}
% \begin{gathered}
%     U_0 = \msf{append}(u_1, \ldots, u_N),
%     \quad
%     v_t = \msf{LM}(U_{t-1}) \\
%     U_{t} = \msf{append}(U_{t-1}, \msf{Tokenizer}(v_t))
% \end{gathered}
% \end{align}
% Beginning with some initial \(U_0\), one generates a sequence of sequences \(U_1, U_2, \ldots\) of increasing lengths by iteratively appending tokenizations of \(v_t\) onto \(U_{t-1}\) to form \(U_{t}\).
% This continues until some stopping condition is reached, for instance, if some maximum step budget is reached or if some \(\msf{Tokenizer}(v_t)\) returns an \(\msf{EOS}\) token that indicates termination.
% In the autoregressive loop above, the labels \(v_1, v_2, \ldots\) represent the intermediate reasoning steps of CoT evaluation.
% The algorithmic schema of~\eqref{eqn:autoreg} captures the core structure of autoregressive computation, though one must make sure to appropriately define the stopping conditions and the \(\msf{Tokenizer}: \mbb{R}^{d_{\msf{out}}} \to \mbb{R}^{d_{\msf{in}}}\) function.







==> old/background_3.tex <==


\section{Problem Setup}
\label{sec:background}

In Section~\ref{sec:background_reasoning}, we first give the necessary background on propositional Horn logic.
Then, in Section~\ref{sec:background_lm}, we present the mathematical formalization of language models with a focus on the sequence-to-sequence transformer module.

% Finally, in Section~\ref{sec:background_autoreg}, we formalize autoregressive evaluation, which is central to CoT reasoning methods.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reasoning in Propositional Horn Logic}
\label{sec:background_reasoning}

A standard task in logical reasoning is to check whether some goal is the consequence of some given facts and rules.
For instance, consider Figure~\ref{fig:mc_inference}, where we have expanded the previous example from Minecraft~\cite{mojang2011minecraft}.
In particular, the recipe list (rules) specifies which combination of items are necessary to make new ones, which we formalize in the language of propositional logic as follows:
\begin{gather*}
    \Gamma = \{
        \msf{Sheep} \to \msf{Wool},
        \enskip
        \msf{Wool} \to \msf{String},
    \msf{Wood} \to \msf{Stick},
        \enskip
        \msf{Stick}\,\text{and}\,\msf{String} \to \msf{FishingRod}
    \}
\end{gather*}
where \(\msf{Sheep}\), \(\msf{Wool}\), etc are \emph{propositions} that represent the statements ``I can get \(\msf{Sheep}\)'', ``I can get \(\msf{Wool}\)'', etc.
The reasoning task is to answer whether the goal \(\tau = \msf{FishingRod}\) is reachable from some given facts \(\Phi = \{\msf{Sheep}, \msf{Wood}\}\) by repeatedly applying the inference rules \(\Gamma\).
Figure~\ref{fig:mc_inference} shows this process in action: a sequence of \emph{proof states} \(s_0, s_1, s_2, s_3\) is derived by iteratively applying \(\Gamma\) to the previous ones, where each proof state is a set of propositions.
Because \(s_3\) subsumes \(\tau\), we conclude that a \(\msf{FishingRod}\) is within reach.


We now present the notation to discuss logical reasoning.
Let \(\mbb{B} = \{0,1\}\) and assume that our universe consists of \(n \geq 1\) propositions \(P_1, \ldots, P_n\) whose conjunctions are represented by binary vectors in \(\mbb{B}^n\).
In particular, \(\alpha \in \mbb{B}^n\) denotes the conjunction \(\bigwedge \{P_i : \alpha_i = 1\}\).
Observe that \(\alpha_i = 0\) marks the absence of \(P_i\), which is not to be confused with negation!
A \emph{rule} is a pair of binary vectors \((\alpha, \beta) \in \mbb{B}^{2n}\),
where \(\alpha\) (the antecedent) specifies what conditions must be met for the rule to be applied, and \(\beta\) (the consequent) specifies what propositions may be derived if the rule is applied.
A \emph{goal} is a vector \(\tau \in \mbb{B}^n\).
By convention, an empty conjunction \(\mbf{0}_n \in \mbb{B}^n\) trivially holds, which allows us to model a fact \(\varphi \in \mbb{B}^n\) as the rule \((\mbf{0}_n, \varphi) \in \mbb{B}^{2n}\).


% Consider the example of Figure~\ref{fig:mc_inference} and index the \(n = 6\) propositions by their order in the final proof state \(s_3\).
% Let \(e_1, \ldots, e_6 \in \mbb{B}^{n}\) be the basis vectors, then we may write:
% \begin{align*}
%     \Gamma = \{
%         (e_1, e_3),
%         \enskip (e_3, e_5),
%         \enskip (e_2, e_4),
%         \enskip (e_4 + e_5, e_6)
%     \}
% \end{align*}
% with facts \(\Phi = \{e_1, e_2\}\) and goal \(\tau = e_6\).
% Beginning from \(s_0 = e_1 + e_2\),
% the proof states are respectively binarized as:
% \begin{align*}
%     s_1 = s_0 + e_3 + e_4,
%     \quad s_2 = s_1 + e_5,
%     \quad s_3 = s_2 + e_6
%     % s_0 = e_1 + e_2,
%     % &\qquad s_1 = s_0 + e_3 + e_4, \\
%     % s_2 = s_1 + e_5,
%     % &\qquad s_3 = s_2 + e_6
% \end{align*}
% We may also rewrite the facts \(\Phi\) as rules using the aforementioned convention of empty conjunctions.
% Under this scheme, we take the initial proof state to be \(s_0 = \mbf{0}_n\) and include the inference rule \((\mbf{0}_n, e_1 + e_2)\) into \(\Gamma\), for a total of \(r = 5\) rules.
% This rewrite of \(\Phi\) allows us to define entailment in terms of only \(\Gamma\) and \(\tau\),
% which is typically presented in a recursive manner.


We now formalize rule application.
Given some proof state \(s \in \mbb{B}^n\) and rule \((\alpha, \beta) \in \Gamma\): if \(s\) subsumes \(\alpha\), then we may conclude that \((s \lor \beta) \in \mbb{B}^n\), where disjunction is applied coordinate-wise.
We thus view a single reasoning step with respect to \(\Gamma\) as the simultaneous application of all rules, for which we overload notation to express as follows:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where for two vectors, \(x \preceq y\) iff each \(x_i \leq y_i\).
Under this notation, we view \(\Gamma\) as a set \(\Gamma \subseteq \mbb{B}^{2n}\) and also as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
Starting at some initial proof state \(s_0 \in \mbb{B}^n\), we may repeatedly apply \(\Gamma: \mbb{B}^n \to \mbb{B}^n\) to generate a sequence of proof states:
\begin{align} \label{eqn:state_seq}
    s_0 \xrightarrow{\Gamma}
    s_1 \xrightarrow{\Gamma}
    s_2 \xrightarrow{\Gamma}
    \cdots
\end{align}
Observe that \(s_0 \preceq s_1 \preceq s_2 \preceq \ldots\) by the definition of \(\Gamma\).
Let \(\Gamma^\star (s)\) denote the maximal set of propositions that can be derived by repeated application of \(\Gamma\).
Because there are only \(n\) propositions, it takes at most \(n\) applications before no new propositions can be derived.
In~\eqref{eqn:state_seq}, for instance, we have \(\Gamma^\star (s_0) = s_n\).
We now present our reasoning problem.


\begin{problem}[Propositional Entailment] \label{prob:propositional_entailment}
Given any set of rules \(\Gamma\) and goal \(\tau \in \mbb{B}^n\), decide whether \(\tau \preceq \Gamma^\star (\mbf{0}_n)\).
\end{problem}


% The relationship between propositional entailment and the more commonly studied problem of \emph{propositional satisfiability} is as follows.
% Given a set of propositions, a \emph{clause} is a disjunction of \emph{literals}, where a literal is either a proposition \(P\) or its negation \(\neg P\).
% Given a set of clauses, the satisfiability problem is to determine whether there exists a truth assignment to all the propositions such that at least one literal is true in every clause.
% The satisfiability problem is the canonical \textsc{NP-Complete} problem.
% A clause is called a \emph{Horn clause} if it contains at most one positive literal.

% In the Horn satisfiability problem, all input clauses must be Horn clauses, and it can be solved in polynomial time.
% Notably, the problem of Horn satisfiability and our presentation of propositional entailment are interreducible.


% \begin{proposition}
%     The problem of Horn satisfiability and the propositional entailment problem~\eqref{prob:propositional_entailment} are interreducible.
%     % The propositional entailment problem~\eqref{prob:propositional_entailment} and the Horn satisfiability problem are interreducible.
% \end{proposition}

% We present a proof in Appendix~\ref{sec:horn_logic}.
% Thus, the chosen formalization precisely captures propositional Horn satisfiability.
% Our formulation is motivated by its correspondence to deriving facts in widely used chain-of-thought reasoning.
% Note that the restriction to Horn reasoning means one cannot derive disjunctive statements such as \(P \lor Q\).






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transformer-based Language Models}
\label{sec:background_lm}


We consider language models as sequence classification models \(\msf{LM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\) that take as input a \emph{token sequence} \(u_1, \ldots, u_N \in \mbb{R}^{d_{\msf{in}}}\) and output a label \(s \in \mbb{R}^{d_{\msf{out}}}\).
We focus on transformer-based language models, which commonly consist of three modules --- the embedding function, the transformer, and the classification head --- as follows:
\begin{align} \label{eqn:lm}
    \msf{LM}:
    U
    \xrightarrow{\msf{Embed}} X
    \xrightarrow{\msf{Transformer}} Y
    \xrightarrow{\msf{ClsHead}} s
\end{align}
where \(U = \msf{append}(u_1, \ldots, u_N) \in \mbb{R}^{N \times d_{\msf{in}}}\) is a stacked representation of the input tokens.
With embedding dimension \(d\), let \(X \in \mbb{R}^{N \times d}\) be the embedded input sequence and let \(Y \in \mbb{R}^{N \times d}\) be the embedded output sequence.
We define an \(L\)-layer transformer as:
\begin{align*}
% \label{eqn:tf}
    \msf{Transformer}(X) = (\msf{Layer}_L \circ \cdots \circ \msf{Layer}_1)(X)
\end{align*}
where each \(\msf{Layer}_l : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of a causal self-attention block composed with a feedforward block:
\begin{align*}
% \label{eqn:tf_layer}
    \msf{Layer}_l (X)
        = ((\msf{Id} + \msf{Ffwd}_l) \circ (\msf{Id} + \msf{Attn}_l))(X)
\end{align*}
with residual connections implemented using the identity operator \(\msf{Id}\).
We give additional details in Appendix~\ref{sec:theory_construction}.


\input{figures/autoreg}


% We first stack the input tokens as \(U = \msf{append}(u_1, \ldots, u_N) \in \mbb{R}^{N \times d_{\msf{in}}}\).
% Then, we pass \(U\) to \(\msf{Embed}: \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{N \times d}\), which is an affine function, in order to yield the \emph{embedded inputs} \(X \in \mbb{R}^{N \times d}\).
% This is passed to \(\msf{Transformer}: \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\).


% is an affine function that maps \(U\) to the \emph{embedded inputs} \(X = \msf{append}(x_1, \ldots, x_N) \in \mbb{R}^{N \times d}\), where \(d\) is called the \emph{embedding dimension}.
% If positional encodings are used, they may be expressed as part of \(\msf{Embed}\).
% The transformer \(\msf{Tf} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) returns a sequence \(Y = \msf{append}(y_1, \ldots, y_N) \in \mbb{R}^{N \times d}\).
% Finally, the classification head \(\msf{ClsHead}: \mbb{R}^{d} \to \mbb{R}^{d_{\msf{out}}}\) is an affine function that acts on the last element of \(Y\) via \(s = \msf{ClsHead}(y_N)\), while ignoring the first \(y_1, \ldots, y_{N-1}\) terms because we use causal self-attention.
% Finally, an \(L\)-layer transformer has form:
% \begin{align} \label{eqn:tf}
%     \msf{Transformer}(X) = (\msf{Layer}_L \circ \cdots \circ \msf{Layer}_1)(X)
% \end{align}
% where each \(\msf{Layer}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of a causal self-attention block and a feedforward block.
% We give a more detailed architecture description in Appendix~\ref{sec:theory_construction}.


% where each \(\msf{Layer}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) consists of an attention block composed into a feedforward block:
% \begin{align} \label{eqn:tf_layer}
%     \msf{Layer}_k (X)
%         = ((\msf{Id} + \msf{Ffwd}_k) \circ (\msf{Id} + \msf{Attn}_k))(X)
% \end{align}

% where \(\msf{Id}\) is the identity block that implements a residual connection.
% The same feedforward block \(\msf{Ffwd}_k : \mbb{R}^{d} \to \mbb{R}^{d}\) is applied in parallel to each term of the \(N\)-length sequence.
% Moreover, the feedforward block of each layer is only 1-hidden unit deep and so takes the form:
% \begin{align} \label{eqn:tf_ffwd}
%     \msf{Ffwd}_k (x)
%     = W_{k2} \sigma (W_{k1} x + b_{k1}) + b_{k2},
% \end{align}
% with parameters \(W_{k1}, W_{k2}^{\top} \in \mbb{R}^{d_{\msf{ffwd}} \times d}\), \(b_{k1} \in \mbb{R}^{d_{\msf{ffwd}}}\), and \(b_{k2} \in \mbb{R}^{d}\), and \(\sigma\) is some activation function that we assume to be \(\msf{ReLU}\).
% Here \(d_{\msf{ffwd}}\) is the feedforward width that is commonly taken to be \(d_{\msf{ffwd}} = 4d\) or some large constant.
% An attention block \(\msf{Attn}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) with \(H\) heads with causal attention has form:
% \begin{gather*}
%     \msf{Attn}_k (X) = \sum_{h = 1}^{H} \msf{CausalSoftmax}(Q_{kh} K_{kh} ^\top) V_{kh} \\
%     Q_{kh} = X W_{Qkh},
%     \quad K_{kh} ^\top = W_{Kkh} ^\top X^\top,
%     \quad V_{kh} = X W_{Vkh}
% \end{gather*}
% with parameters \(W_{Qkh}, W_{Kkh} ^\top \in \mbb{R}^{d \times d_{\msf{attn}}}\) and \(W_{Vkh} \in \mbb{R}^{d \times d}\) for heads \(h = 1, \ldots, H\).
% Note that it suffices to take \(d_{\msf{attn}} \leq d\).
% Here, \(\msf{CausalSoftmax}: \mbb{R}^{N \times N} \to \mbb{R}^{N \times N}\) is the causal variant of row-wise softmax defined as follows:
% \begin{align*}
%     &\msf{CausalSoftmax}(Z) \\
%     &= \begin{bmatrix}
%         \msf{Softmax}( z_{11}, & -\infty, & \cdots, & -\infty) \\
%         \msf{Softmax}( z_{21}, & z_{22}, & \cdots, & -\infty) \\
%         \vdots & \vdots & \ddots & \vdots \\
%         \msf{Softmax}( z_{N1}, & z_{N2}, & \cdots, & z_{NN})
%     \end{bmatrix}
% \end{align*}
% where \(z_{ij}\) is the \((i,j)\)th entry of the parameter \(Z \in \mbb{R}^{N \times N}\) and \(\msf{Softmax} : \mbb{R}^{N} \to \mbb{R}^{N}\) is given as:
% \begin{align*}
%     \msf{Softmax}(a_1, \ldots, a_N)
%     &= \frac{\parens*{e^{a_1}, \ldots, e^{a_N}}}{e^{a_1} + \cdots + e^{a_N}}
%     \in \mbb{R}^{N}
% \end{align*}
% Observe that \(-\infty\) to an argument of \(\msf{Softmax}\) makes the corresponding position zero.
% \(\msf{CausalSoftmax}(Z)\) is thus a lower-triangular matrix with zeros strictly above the diagonal, i.e., \(\msf{CausalSoftmax}(Z)_{ij} = 0\) iff \(j > i\).
% Note that our formalism omits the layer normalization, which is typically applied after each attention block and after each feedforward block.
% This omission does not change the fundamental expressive power of a transformer~\cite{liu2022transformers} and serves to simplify the theoretical analysis.
% Moreover, although the transformer must fix apriori various quantities like \(d, d_{\msf{ffwd}}, d_{\msf{attn}}\), the sequence may be of any length \(N\) --- though in practice there is often an upper bound \(N_{\msf{max}} \geq N\) due to limitations in the choice of positional encoding.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Autoregressive Evaluation of Language Models}
% \label{sec:background_autoreg}

% Having defined the transformer-based sequence classification model, \(\msf{LM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{d_{\msf{out}}}\), we next formalize autoregressive evaluation.
% This style of evaluation is central to many CoT reasoning strategies and can be defined using the following set of recursive equations:
% \begin{align} \label{eqn:autoreg}
% \begin{gathered}
%     U_0 = \msf{append}(u_1, \ldots, u_N),
%     \quad
%     v_t = \msf{LM}(U_{t-1}) \\
%     U_{t} = \msf{append}(U_{t-1}, \msf{Tokenizer}(v_t))
% \end{gathered}
% \end{align}
% Beginning with some initial \(U_0\), one generates a sequence of sequences \(U_1, U_2, \ldots\) of increasing lengths by iteratively appending tokenizations of \(v_t\) onto \(U_{t-1}\) to form \(U_{t}\).
% This continues until some stopping condition is reached, for instance, if some maximum step budget is reached or if some \(\msf{Tokenizer}(v_t)\) returns an \(\msf{EOS}\) token that indicates termination.
% In the autoregressive loop above, the labels \(v_1, v_2, \ldots\) represent the intermediate reasoning steps of CoT evaluation.
% The algorithmic schema of~\eqref{eqn:autoreg} captures the core structure of autoregressive computation, though one must make sure to appropriately define the stopping conditions and the \(\msf{Tokenizer}: \mbb{R}^{d_{\msf{out}}} \to \mbb{R}^{d_{\msf{in}}}\) function.







==> old/background_4.tex <==


\section{Background and Problem Setup}
\label{sec:background}

In Section~\ref{sec:background_reasoning}, we first give the necessary background on propositional Horn logic.
Then, in Section~\ref{sec:background_lm}, we present the mathematical formalization of language models with a focus on the sequence-to-sequence transformer module.

% Finally, in Section~\ref{sec:background_autoreg}, we formalize autoregressive evaluation, which is central to CoT reasoning methods.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reasoning in Propositional Horn Logic}
\label{sec:background_reasoning}

A standard task in logical reasoning is to check whether some goal is the consequence of some given facts and rules.
For instance, consider Figure~\ref{fig:mc_inference}, where we have expanded the previous example from Minecraft~\cite{mojang2011minecraft}.
In particular, the recipe list (rules) specifies which combination of items are necessary to make new ones, which we formalize in the language of propositional logic as follows:
\begin{gather*}
    \Gamma = \{
        \msf{Sheep} \to \msf{Wool},
        \enskip
        \msf{Wool} \to \msf{String},
    \msf{Wood} \to \msf{Stick},
        \enskip
        \msf{Stick}\,\text{and}\,\msf{String} \to \msf{FishingRod}
    \}
\end{gather*}
where \(\msf{Sheep}\), \(\msf{Wool}\), etc are \emph{propositions} that represent the statements ``I can get \(\msf{Sheep}\)'', ``I can get \(\msf{Wool}\)'', etc.
The reasoning task is to answer whether the goal \(\tau = \msf{FishingRod}\) is reachable from some given facts \(\Phi = \{\msf{Sheep}, \msf{Wood}\}\) by repeatedly applying the inference rules \(\Gamma\).
Figure~\ref{fig:mc_inference} shows this process in action: a sequence of \emph{proof states} \(s_0, s_1, s_2, s_3\) is derived by iteratively applying \(\Gamma\) to the previous ones, where each proof state is a set of propositions.
Because \(s_3\) subsumes \(\tau\), we conclude that a \(\msf{FishingRod}\) is within reach.


We now present the notation to discuss logical reasoning.
Let \(\mbb{B} = \{0,1\}\) and assume that our universe consists of \(n \geq 1\) propositions \(P_1, \ldots, P_n\) whose conjunctions are represented by binary vectors in \(\mbb{B}^n\).
In particular, \(\alpha \in \mbb{B}^n\) denotes the conjunction \(\bigwedge \{P_i : \alpha_i = 1\}\).
Observe that \(\alpha_i = 0\) marks the absence of \(P_i\), which is not to be confused with negation!
A \emph{rule} is a pair of binary vectors \((\alpha, \beta) \in \mbb{B}^{2n}\),
where \(\alpha\) (the antecedent) specifies what conditions must be met for the rule to be applied, and \(\beta\) (the consequent) specifies what propositions may be derived if the rule is applied.
A \emph{goal} is a vector \(\tau \in \mbb{B}^n\).
By convention, an empty conjunction \(\mbf{0}_n \in \mbb{B}^n\) trivially holds, which allows us to model a fact \(\varphi \in \mbb{B}^n\) as the rule \((\mbf{0}_n, \varphi) \in \mbb{B}^{2n}\).


% Consider the example of Figure~\ref{fig:mc_inference} and index the \(n = 6\) propositions by their order in the final proof state \(s_3\).
% Let \(e_1, \ldots, e_6 \in \mbb{B}^{n}\) be the basis vectors, then we may write:
% \begin{align*}
%     \Gamma = \{
%         (e_1, e_3),
%         \enskip (e_3, e_5),
%         \enskip (e_2, e_4),
%         \enskip (e_4 + e_5, e_6)
%     \}
% \end{align*}
% with facts \(\Phi = \{e_1, e_2\}\) and goal \(\tau = e_6\).
% Beginning from \(s_0 = e_1 + e_2\),
% the proof states are respectively binarized as:
% \begin{align*}
%     s_1 = s_0 + e_3 + e_4,
%     \quad s_2 = s_1 + e_5,
%     \quad s_3 = s_2 + e_6
%     % s_0 = e_1 + e_2,
%     % &\qquad s_1 = s_0 + e_3 + e_4, \\
%     % s_2 = s_1 + e_5,
%     % &\qquad s_3 = s_2 + e_6
% \end{align*}
% We may also rewrite the facts \(\Phi\) as rules using the aforementioned convention of empty conjunctions.
% Under this scheme, we take the initial proof state to be \(s_0 = \mbf{0}_n\) and include the inference rule \((\mbf{0}_n, e_1 + e_2)\) into \(\Gamma\), for a total of \(r = 5\) rules.
% This rewrite of \(\Phi\) allows us to define entailment in terms of only \(\Gamma\) and \(\tau\),
% which is typically presented in a recursive manner.


We now formalize rule application.
Given some proof state \(s \in \mbb{B}^n\) and rule \((\alpha, \beta) \in \Gamma\): if \(s\) subsumes \(\alpha\), then we may conclude that \((s \lor \beta) \in \mbb{B}^n\), where disjunction is applied element-wise.
We thus view a single reasoning step with respect to \(\Gamma\) as the simultaneous application of all rules, for which we overload notation to express as follows:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where for two vectors, \(x \preceq y\) iff each \(x_i \leq y_i\).
Under this notation, we view \(\Gamma\) as a set \(\Gamma \subseteq \mbb{B}^{2n}\) and also as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
Starting at some initial proof state \(s_0 \in \mbb{B}^n\), we may repeatedly apply \(\Gamma: \mbb{B}^n \to \mbb{B}^n\) to generate a sequence of proof states \(s_0, s_1, s_2, \ldots\) where each \(s_{t+1} = \Gamma(s_t)\).
Observe that \(s_0 \preceq s_1 \preceq s_2 \preceq \ldots\) by the definition of \(\Gamma\).
Let \(\Gamma^\star (s)\) denote the maximal set of propositions derivable by repeated application of \(\Gamma\).
Because there are only \(n\) propositions, it takes at most \(n\) applications before no new propositions can be derived, meaning that \(\Gamma^\star (s_0) = s_n\).
We now present our reasoning problem.


\begin{problem}[Entailment] \label{prob:propositional_entailment}
Given any set of rules \(\Gamma\) and goal \(\tau \in \mbb{B}^n\), decide whether \(\tau \preceq \Gamma^\star (\mbf{0}_n)\).
\end{problem}


% The relationship between propositional entailment and the more commonly studied problem of \emph{propositional satisfiability} is as follows.
% Given a set of propositions, a \emph{clause} is a disjunction of \emph{literals}, where a literal is either a proposition \(P\) or its negation \(\neg P\).
% Given a set of clauses, the satisfiability problem is to determine whether there exists a truth assignment to all the propositions such that at least one literal is true in every clause.
% The satisfiability problem is the canonical \textsc{NP-Complete} problem.
% A clause is called a \emph{Horn clause} if it contains at most one positive literal.

% In the Horn satisfiability problem, all input clauses must be Horn clauses, and it can be solved in polynomial time.
% Notably, the problem of Horn satisfiability and our presentation of propositional entailment are interreducible.


% \begin{proposition}
%     The problem of Horn satisfiability and the propositional entailment problem~\eqref{prob:propositional_entailment} are interreducible.
%     % The propositional entailment problem~\eqref{prob:propositional_entailment} and the Horn satisfiability problem are interreducible.
% \end{proposition}

% We present a proof in Appendix~\ref{sec:horn_logic}.
% Thus, the chosen formalization precisely captures propositional Horn satisfiability.
% Our formulation is motivated by its correspondence to deriving facts in widely used chain-of-thought reasoning.
% Note that the restriction to Horn reasoning means one cannot derive disjunctive statements such as \(P \lor Q\).






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transformer-based Language Models}
\label{sec:background_lm}

Because our theoretical encoding results leverage a transformer with only one layer and one self-attention head, we present a simplified model architecture as follows:

\begin{align} \label{eqn:model_def}
\begin{split}
    \mcal{R}(X) &= \parens*{(\msf{Id} + \msf{Ffwd}) \circ (\msf{Id} + \msf{Attn}}\big)(X), \\
    \msf{Attn}(X) &= \msf{CauaslSoftmax}\parens*{(X Q + \mbf{1}_N q^\top)K ^\top X^\top} X V, \\
    \msf{Ffwd}(z) &= W_2 \msf{ReLU}(W_1 z + b),
\end{split}
    \quad X = \brmatrix{x_1 ^\top \\ \rvdots \\ x_N ^\top} \in \mbb{R}^{N \times d}
\end{align}

Here, \(\mcal{R} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) is a sequence-to-sequence transformer model that is our reasoner, where \(d\) is the embedding dimension and \(N\) is the sequence length.
We use a residual connection, denoted by the identity layer \(\msf{Id}\), for both the self-attention and feedforward blocks.
First, the self-attention block \(\msf{Attn}: \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) has weights \(Q, K^\top, V \in \mbb{R}^{d \times d}\) and bias \(q \in \mbb{R}^{d}\), with \(\msf{Softmax}: \mbb{R}^{N} \to \mbb{R}^{N}\) applied to each row.
Then, \(\msf{Ffwd}: \mbb{R}^{d} \to \mbb{R}^{d}\) is the one-hidden-layer feedforward block with weights \(W_1 ^\top, W_2 \in \mbb{R}^{d \times d_{\msf{ffwd}}}\) and bias \(b \in \mbb{R}^{d_{\msf{ffwd}}}\), where \(d_{\msf{ffwd}}\) is the width.
During evaluation, the same \(\msf{Id} + \msf{Ffwd}: \mbb{R}^{d} \to \mbb{R}^{d}\) is applied in parallel to each vector of \((\msf{Id} + \msf{Attn})(X) \in \mbb{R}^{N \times d}\).

% We present our technical analysis with \(\msf{Softmax}\) instead of the more commonly used \(\msf{CausalSoftmax}\) for convenience since it simplifies the presentation without altering the fundamental results.



\input{figures/layers_math}

\subsection{What Does One Step of Reasoning Look Like?}
\label{sec:theory_overview}

We showcase one autoregressive iteration of CoT reasoning in Figure~\ref{fig:layers_math}.
Principally, this autoregressive loop is governed by the following set of inductive equations:
\begin{align} \label{eqn:autoreg_loop}
    X_{t+1} = \msf{append}(X_t, (\mbf{0}_n, \hat{s}_{t+1})),
    \quad \hat{s}_{t+1} \leftarrow \mcal{R}(X_t),
    \quad
    X_0 = \parens*{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r), (\mbf{0}_n, s_0)}
\end{align}
where \(\hat{s}_{t+1}\) is extracted out from the last row of \(\mcal{R}(X_t)\) via a linear projection.
The goal is to learn weights for \(\mcal{R}\) such that we can simulate applications of \(\Gamma\) in the following sense:
\begin{align*}
    s_0 \xrightarrow{\Gamma}
        s_1 \xrightarrow{\Gamma}
        s_2 \xrightarrow{\Gamma}
        \cdots
    \quad \approx \quad
    s_0 \xrightarrow{\mcal{R}}
    \hat{s}_1 \xrightarrow{\mcal{R}}
    \hat{s}_2 \xrightarrow{\mcal{R}}
    \cdots,
\end{align*}
where the objective is to construct \(\mcal{R}\) such that each \(s_t = \hat{s}_t\).
If we know the number of rules \(r\) and the maximum number of steps \(t_{\msf{max}}\) are known, then we can construct a \(\mcal{R}\) as in~\eqref{eqn:model_def} that can ensure \(s_t = \hat{s}_t\) for all \(t \leq t_{\msf{max}}\).
This technical assumption is due to our use of softmax attention.
We formalize our encoding result in the following.

\begin{theorem}[Encoding] \label{thm:encoding}
For any number of propositions \(n\), number of rules \(r\), and maximum number of steps \(t_{\msf{max}}\), there exists a reasoner \(\mcal{R}\) as in~\eqref{eqn:model_def} with \(d = 2n\) and \(d_{\msf{ffwd}} = 4d\)
such that:
% such that \(s_t = \hat{s}_t\) for all \(t \leq t_{\msf{max}}\).
% In other words,
% for all \(X_t \in \mbb{R}^{(r+t+1) \times 2n}\) as in~\eqref{eqn:autoreg_loop} with \(r \leq r_{\msf{max}}\) and \(t \leq t_{\msf{max}}\):
\begin{align*}
    X_{t} = \begin{bmatrix} \alpha_1 ^\top & \beta_1  ^\top \\
    \vdots & \vdots \\
    \mbf{0}_n ^\top & s_t ^\top
    \end{bmatrix}
    \xrightarrow{\mcal{R}}
    \begin{bmatrix} \star & \star \\ \vdots & \vdots \\ \star & \Gamma(s_{t})^\top
    \end{bmatrix},
    % \qquad \Gamma(s_t) = s_{t+1} = \hat{s}_{t+1}
    \enskip \text{for all \(X_t \in \mbb{R}^{(r+t+1) \times 2n}\) as in~\eqref{eqn:autoreg_loop} where \(t \leq t_{\msf{max}}\)}.
\end{align*}

% For any \(r_{\msf{max}}, t_{\msf{max}} > 0\), there exists \(\mcal{R}\) as in~\eqref{eqn:model_def} with embedding dimension \(d = 2n\) and feedforward width \(d_{\msf{ffwd}} = 4d\) such that \(s_t = \hat{s}_t\) for all \(t \leq t_{\msf{max}}\) steps of 
% for all \(X_t \in \mbb{R}^{(r+t+1) \times 2n}\) as in~\eqref{eqn:autoreg_loop} where \(r \leq r_{\msf{max}}\) and \(t \leq t_{\msf{max}}\),
% \begin{align*}
%     X_{t} = \begin{bmatrix} \alpha_1 ^\top & \beta_1  ^\top \\
%     \vdots & \vdots \\
%     \mbf{0}_n ^\top & s_t ^\top
%     \end{bmatrix}
%     \xrightarrow{\mcal{R}}
%     \begin{bmatrix} \star & \star \\ \vdots & \vdots \\ \star & \Gamma(s_{t})^\top
%     \end{bmatrix},
%     % \enskip \text{for all \(X_t \in \mbb{R}^{(r+t+1) \times 2n}\) where \(r \leq r_{\msf{max}}\) and \(t \leq t_{\msf{max}}\)}.
% \end{align*}
% for all \(X_t \in \mbb{R}^{(r+t+1) \times 2n}\) as in~\eqref{eqn:autoreg_loop} where \(r \leq r_{\msf{max}}\) and \(t \leq t_{\msf{max}}\).
\end{theorem}
\begin{proof}(Sketch)
With an appropriate choice of weights for the self-attention block:
\begin{align*}
    X_t = \begin{bmatrix}
        \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots \\
        \mbf{0}_n ^\top & s_t ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        \star & \star \\
        \vdots & \vdots \\
        \star & \parens*{s_t + \sum_{i: \alpha_i \preceq s_t} \beta_i + \varepsilon}^\top
    \end{bmatrix}
    \in \mbb{R}^{(r+t+1) \times 2n},
\end{align*}
where \(\varepsilon\) is a small residual term.
This approximates rule application in the sense that
\begin{align*}
    \parens*{s_t + \sum_{i: \alpha_i \preceq s_t} \beta_i + \varepsilon}_j
    \begin{dcases}
        \leq 1/3 & \text{iff \(\Gamma(s_t)_{j} = 0\)} \\
        \geq 2/3 & \text{iff \(\Gamma(s_t)_{j} = 1\)}
    \end{dcases},
    \qquad \text{for all coordinates \(j = 1, \ldots, n\)},
\end{align*}
where the disjunctions in rule application (see~\eqref{eqn:one_step_rules}) are implemented with scaled summation of binary values.
Then, \(\msf{Id} + \msf{Ffwd}\) approximates an indicator function on values \(\geq 2/3\).
\end{proof}


==> old/experiments_1.tex <==
\section{Experiments}
\label{sec:experiments}

Our experiments aim to answer the following questions.

\paragraph{(Q1)}
\textbf{How many parameters does a reasoner need?}
Our main theoretical result in Theorem~\ref{thm:main_result_sketch} states that for reasoning: one layer, one head, and embedding dimension linear in the number of propositions suffice.
We emphasize, however, that this is a sufficiency result for encoding: it may be the case that a much larger embedding dimension is needed in practice.
Therefore, we investigate how well language models of different sizes can learn to reason.


\paragraph{(Q2)}
\textbf{Do theoretical attacks translate to practice?}
We present in Theorem~\ref{thm:attack_result_sketch} a construction of adversarial attacks against our theoretical construction, which works by over-saturating the language model's attention.
We investigate whether such attacks also work against learned models.


\paragraph{(Q3)}
\textbf{How well can language models attack each other?}
Section~\ref{sec:learned_attacks} presents a method for training language models that attack language models.
We investigate how effective such attacker models are.



\paragraph{(Q4)}
\textbf{Are learned reasoners out-of-distribution robust?}
Although our theoretical construction can handle any set of rules, a learned model may struggle with ones it has not seen.
Therefore, we study the robustness of learned models to out-of-distribution data.


\paragraph{Model and Dataset Setup}
We use GPT-2~\cite{radford2019language} as our base transformer model initialized with different embedding dimensions \(d\), number of layers \(L\), and number of heads \(H\).
By default, GPT-2 has feedforward width \(d_{\msf{ffwd}} = 4d\).
We generate random datasets for both training and testing reasoner models.
Our training setup is described next.
For a fixed number of propositions \(n\), we sample a rule as follows.
First, we sample the antecedent and consequent hot-bit probabilities \(p_\alpha, p_\beta \sim \msf{Uniform}(0.2, 0.3)\).
Then, we sample the antecedent \(\alpha \sim \msf{Bernoulli}^n (p_\alpha)\) and the consequent \(\beta \sim \msf{Bernoulli}^n (p_\beta)\) to form a rule \((\alpha, \beta) \in \mbb{B}^{2n}\).
A sequence contains \(r \sim \msf{RandInt}(16, 64)\) rules.
Each dataset query returns a new random sequence of rules.

\paragraph{Training Setup}
For learned reasoners, we train each for a total of \(12800\) steps with a batch size of \(128\).
We use AdamW~\cite{Loshchilov2017DecoupledWD} as our optimizer and an initial learning rate of \(5e^{-5}\) with a linear decay schedule (\(10\%\) warmup).
By default, each experiment is run with three random seeds, and we report the mean validation accuracy of correctly predicting all \(n\) bits of the final state.


In this Section, we show a subset of our experiments and refer to Appendix~\ref{sec:additional_experiments} for a more comprehensive set of results.



\input{figures/q1}

\subsection{(Q1) Empirical Validation of Theorem~\ref{thm:main_result_sketch}}
\label{sec:experiments_q1}

We first study how language model-based reasoners can learn one step of propositional inference using only \(L=1\) layers and \(H = 1\) heads.
We train reasoners of embedding dimensions \(d \in \{32, 64, \ldots, 256\}\) to reason with number of propositions \(n \in \{8, 16, \ldots, 64\}\).
In Figure~\ref{fig:q1}, we show in each block the mean-value performance of three different training seeds.
We observe a linear trend in the embedding dimension necessary to attain near-perfect accuracy; this is achieved by all reasoners with \(d \geq 4n\). We refer interested readers to Appendix~\ref{sec:appendix_model_params} for some results on how increasing the number of layers/heads affects performance.





% We first study how accurately various model architectures can learn to perform autoregressive propositional inference.
% We fix \(L = 1\) layers and \(H = 1\) heads as given in Theorem~\ref{thm:main_result_sketch} and vary the embedding dimension for \(d \in \{32, 64, \ldots, 256\}\) and the number of propositions for \(n \in \{8, 16, \ldots, 64\}\).
% The training and validation data for each instance of \(n\) is drawn as follows: First, we fix some \(0.2 \leq p_\alpha \leq 0.3\) and \(0.2 \leq p_\beta \leq 0.3\). We then pick the number of rules \(16 \leq r \leq 64\) uniformly at random along with an initial state. Figure~\ref{fig:q1} shows the final mean validation accuracies of various \((n, d)\) pairs. The performance improves as the embedding dimension increases for a given number of propositions. Moreover, the embedding dimension and number of propositions demonstrate a linear trend with respect to performance which validates the linear relationship implied by Theorem~\ref{thm:main_result_sketch}. More concretely, all learners demonstrate perfect performance when \(d \geq 4n\).



\input{figures/q2}

\subsection{(Q2) Empirical Validation of Theoretical Attacks}
\label{sec:experiments_q2}

In Section~\ref{sec:theory_attacks}, we construct adversarial attacks against our theoretical models.
Given some adversarial target label \(s_{\msf{tgt}}\), our theory says that:
for a sufficiently large \(\kappa\), appending the single attack token \(u_{\msf{atk}} = (\mbf{0}_n, s_{\msf{tgt}} - \kappa (1 - s_{\msf{tgt}}))\) to any input sequence will force our theoretical reasoner to output \(s_{\msf{tgt}}\).
Unfortunately, we failed to reliably replicate this attack experimentally: learned reasoners rarely output \(s_{\msf{tgt}}\) when subject to our theoretically constructed \(u_{\msf{tgt}}\).


However, our intuition for constructing theoretical attacks suggests strategies for other experiments.
Namely, the theoretical attack works by saturating the reasoner's attention with large values of \(\kappa\).
This inspired us to examine whether some attack token \(u_{\msf{atk}}\) appended to different input sequences can make the reasoner yield the same output.
In this experiment,
we randomly sample \(s_{\msf{tgt}}\) and construct \(u_{\msf{atk}}\) as in the theory.
Then, we sample two input sequences \(U_1\) and \(U_2\) from the reasoner's training distribution, and append \(u_{\msf{atk}}\) to both to form \(U_1 '\) and \(U_2 '\), respectively.
We then plot the accuracy of \(\msf{Reasoner}(U_1 ') = \msf{Reasoner}(U_2 ')\) in Figure~\ref{fig:q2}.
We see that for sufficiently large \(\kappa\), we can indeed force \(\msf{Reasoner}\) to consistently reach the same output on \(U_1 '\) and \(U_2 '\).
This suggests that attention saturation is an effective attack strategy against transformers with softmax attention. Additional results are presented in Appendix~\ref{sec:appendix_theory_attack}.




% In Section~\ref{sec:theory_attacks}, we provide a theoretical construction for attack vectors \(U_\msf{atk}\) that can be appended to original inputs \(U\) such that a learner generates a chosen adversarial target \(s_\msf{tgt}\).
% We attempted to attack some perfect learners using adversarial inputs constructed as in Theorem~\ref{thm:attack_result_sketch} but did not succeed in recovering the target adversarial outputs \(s_\msf{tgt}\). In an attempt to validate the principle guiding the theoretical attack construction, we performed another experiment that measures the accuracy of predicting the \emph{same} output vector for two samples given the constructed input. Here, the output vector doesn't need to match \(s_\msf{tgt}\) but is expected be the same on two randomly chosen inputs. Moreover, this accuracy is expected to increase as the value of \(\kappa\) in Theorem~\ref{thm:attack_result_sketch} increases. We pick all perfect learners with \(d = 96\) from Figure~\ref{fig:q1} (i.e., learners trained for \(n \in \{8, 16, 24\}\)) and vary \(\kappa \in \{10^{-3}, 10^{-2}, \ldots, 10^{9}\}\). For every example in a test dataset with \(8k\) samples, we randomly sample another example from the dataset and collect their outputs on an adversarial input constructed as in Theorem~\ref{thm:attack_result_sketch}. We report the accuracies of these matches in Figure~\ref{fig:q2} for various values of \(\kappa\). The results confirm that higher values of \(\kappa\) can lead to stronger attacks against the chosen perfect learners, reaching perfect attack accuracy of 1.0 for \(\kappa \geq 10^{4}\). Moreover, for \(\kappa \leq 10^{3}\), we observe that learners trained with a lower number of propositions report higher attack accuracies. These results suggest that it is possible to force perfect learners to generate unknown but incorrect outputs even \emph{without} training any attackers explicitly. Similar trends are observed for perfect learners corresponding to other embedding dimensions and we report the results for \(d \in \{128, 160, 192\}\) in Appendix~\ref{sec:additional_experiments}.

\input{figures/q3}

\subsection{(Q3) Performance of Learned Attackers}
\label{sec:experiments_learned_attackers}

We next study the ability of language models to learn attacks against other language models.
Given a reasoner model, can we learn an attacker model that can consistently craft some sequence of attack tokens that forces the reasoner to output some adversarial target \(s_{\msf{tgt}}\)?
Moreover, can the attacker do so efficiently, using a single attack token \(u_{\msf{atk}}\)?
We show that the answer is \emph{yes}.
We take our attacker to be GPT-2 base (\(d = 768\), \(L=12\), \(H=12\)) and take the reasoner to be a selection of models from Figure~\ref{fig:q1}.
We train each attacker on the same input distribution as the respective reasoner model using the optimization objective defined in~\eqref{eqn:attacker_training_problem} and plot the performance in Table~\ref{tab:learned_attack_results}.
The learned attackers can \emph{perfectly attack} 8 out of the 12 chosen near-perfect reasoners.
As the reasoner model grows in size, however, the attacks generally become less consistent.
These results suggest that it is possible to attack near-perfect reasoners with language model-based attackers.




% As discussed in Section~\ref{sec:learned_attacks}, the learners in Figure~\ref{fig:q1} can possibly be attacked by language models that are trained using the loss objective in Equation~\ref{eqn:attack_problem}. We pick the perfect learners (i.e., learners with a mean validation accuracy of 1.0) corresponding to \(d \in \{96, 128, 160\} \) (i.e., learners for \(n \in \{8, 16, \ldots, 40\}\)) as representative victims. We choose GPT-2 as the architecture for the attacker models with the default parameters \(d = 768, L = 12, H = 12\). We train the attackers for 10 epochs using training \(16k\) samples and validate using \(8k\) samples. Each attacker model is trained to attack a learner \emph{universally} with an attack budget of \(N_{\msf{atk}} = 1\) tokens, meaning that it can force the learner to output \emph{any} random binary vector \(s_\msf{tgt}\) for any input \(U\) by just appending a single adversarial token. The attackers are trained to do the following: for a given input sample \(U\) and a random binary vector \(s_{tgt}\), generate a vector \(U_{\msf{atk}}\) (with \(N_{\msf{atk}} = 1\) tokens) that can be appended to \(U\) and forces the target learner to output \(s_\msf{tgt}\). The success of the attacks can then be measured as the accuracy of the learners generating the random \(s_\msf{tgt}\) vectors. We report these accuracies over three runs in Table~\ref{tab:learned_attack_results}. The learned attackers can \emph{perfectly attack} 9 out of the 12 chosen perfect learners. Moreover, this perfect accuracy is observed across all three random runs, as is evident by the standard error of 0. These results suggest that it is easy attack perfect language model learners by training attackers using the objective defined in Section~\ref{sec:learned_attacks} and hence the perfect performance on held out validation sets may not indicate robustness to such attacks.

\input{figures/q4}

\subsection{(Q4) Out-of-Distribution Robustness}

Lastly, we study how near-perfect reasoners fare on data outside their training distribution.
We consider near-perfect in-distribution reasoners with embedding dimension \(d = 96\) as in Figure~\ref{fig:q1} and test their performance on different datasets while varying key parameters.
In particular, we vary the rates at which rule bits become hot \((p_\alpha ^{\msf{test}}, p_\beta ^{\msf{test}} \in \{0.1, 0.2, \ldots, 0.9\})\) and the number of rules \((r^{\msf{test}} \in \{8, 16, 32, \ldots, 512\})\).
We plot these in Figure~\ref{fig:q4_a} and Figure~\ref{fig:q4_b}, respectively.
When reasoners are subject to rules with more hot bits than what is in-distribution, their performance decays.
Similarly, when they take as input a long sequence of rules, accuracy suffers. We present some additional results in Appendix~\ref{sec:appendix_ood}.





% We next test the robustness of learned models to out-of-distribution data. We consider perfect in-distribution learners with \(d = 96\) from Figure~\ref{fig:q1}, i.e., models that reach a mean validation accuracy of \(1.0\) and test their performance on test datasets from different distributions. In particular, we consider the learners with \(n \in \{8, 16, 24\}\). We vary two key parameters, namely the probabilities of propositions occurring in the antecedent / consequent and the number of rules, independently, while keeping the rest of the data generation parameters the same as the training datasets.  The probabilities of propositions occurring in the antecedent and consequent \(p_\alpha\ = p_\beta = k\) are varied as \(k \in \{0.1, 0.2, \ldots, 0.9\}\) where \(0.2 \leq p_\alpha = p_\beta \leq 0.3\) represents the "in-distribution" range. The number of rules are independently varied as \(r \in \{8, 16, 32, \ldots, 512\}\) with \(16 \leq r \leq 64\) being the in-distribution range. The results of these variations are reported in Figure~\ref{fig:q4_a} and Figure~\ref{fig:q4_b} respectively. The performance drops significantly as the probabilities and number of rules are increased beyond those used for training. Interestingly, the learners are robust to values lower than those used during training (i.e., \(p_\alpha\ = p_\beta < 0.2 \) and \(r < 16\)) as they retain perfect accuracies in these ranges. 




==> old/experiments_2.tex <==
\section{Experiments}
\label{sec:experiments}

Our experiments aim to answer the following questions.

\paragraph{(Q1)}
\textbf{How good are learned reasoners?}
% Our main theoretical result in Theorem~\ref{thm:main_result_sketch} states that for reasoning: one layer, one head, and embedding dimension linear in the number of propositions suffice.
% We emphasize, however, that this is a sufficiency result for encoding: it may be the case that a much larger embedding dimension is needed in practice.
% Therefore, we investigate how well language models of different sizes can learn to reason.


\paragraph{(Q2)}
\textbf{How good are learned attackers?}

% We present in Theorem~\ref{thm:attack_result_sketch} a construction of adversarial attacks against our theoretical construction, which works by over-saturating the language model's attention.
% We investigate whether such attacks also work against learned models.


\paragraph{(Q3)}
\textbf{What strategies do learned attackers use?}
% Section~\ref{sec:learned_attacks} presents a method for training language models that attack language models.
% We investigate how effective such attacker models are.



\paragraph{(Q4)}
\textbf{How well do natural language models perform?}
% Although our theoretical construction can handle any set of rules, a learned model may struggle with ones it has not seen.
% Therefore, we study the robustness of learned models to out-of-distribution data.


%%%%%%%%%%

\subsection{(Q1) How Good are Learned Reasoners?}
We have shown that shallow transformers can theoretically encode one step of propositional reasoning, but how do they fare in practice?
We now show that learned models can indeed attain high accuracies across different values of \(n\) (number of propositions) and \(d\) (embedding dimension).


\paragraph{Model Setup}
We use GPT-2~\citep{radford2019language} as our base transformer model initialized with one layer, one self-attention head, and different values of embedding dimension \(d\).
By default, GPT-2 uses feedforward width \(d_{\msf{ffwd}} = 4d\) with GeLU activation and layer norms.


\paragraph{Dataset Setup}
Although we use randomized datasets for this experiment, we must be careful in their generation.
We first generate an initial random set of rules as follows:
\begin{align*}
    \Gamma_{\msf{init}} = \{
        (\alpha_1, \beta_1),
        \ldots,
        (\alpha_r, \beta_r)
    \},
    \quad \alpha_i, \beta_i \sim \mcal{B}^n(p),
    \quad p \sim \msf{Unif}(0.2, 0.3),
    \quad r \sim \msf{Unif}(32, 64),
\end{align*}
where \(\mcal{B}^n (p)\) is the \(n\)-dimensional coordinate-wise iid Bernoulli distribution with hot probability \(p\), and \(\msf{Unif}\) is the uniform distribution that may be continuous or discrete depending on context.
However, observe that \(\Gamma_{\msf{init}} (\mbf{0}_n) = \mbf{0}_n\) with high probability if \(n\) is sufficiently large, meaning that each rule is hard to trigger.
Therefore, we modify \(\Gamma_{\msf{init}}\) to have enough structure to prevent the model from learning a trivial (all zeros) solution.
For some \(k \sim \msf{Unif}(4, 7)\), we generate \(\Gamma = \msf{InjectStructure}(\Gamma_{\msf{init}}, k)\) to ensure a non-trivial sequence of proof states \(\mbf{0}_n = s_0 \prec \cdots \prec s_k\).
Using this, we return the input sequence:
\begin{align*}
    X = \msf{append}(\Gamma, (\mbf{0}_n, s_0), \ldots, (\mbf{0}_n, s_t))
    \in \mbb{R}^{(r+t+1) \times 2n},
    \quad s_{t+1} = \Gamma(s_t),
    \quad s_{0} = \mbf{0}_n,
    % \quad t \sim \msf{Unif}(1, 4).
\end{align*}
where \(t \sim \msf{Unif}(1,4)\) is the number of previous steps.
The model's goal is to predict \(s_{t+1}\).


\paragraph{Training Setup}
We train each model for a total of 4096 steps with a batch size of 1024.
We use AdamW~\cite{Loshchilov2017DecoupledWD} as our optimizer with a \(5e^{-4}\) learning rate, \(10\%\) warmup, and linear decay schedule.
We use binary cross entropy with logit loss.
% By default, each experiment is run with three random seeds, and we report the mean validation accuracy of correctly predicting all \(n\) bits of the final state.


\input{figures/gpt2_grid}


We present our results in Figure~\ref{fig:gpt2_grid} for different \(n \in \{16, 32, \ldots, 128\}\), \(d \in \{32, 64, \ldots, 256\}\), and autoregressive steps \(k \in \{1,2,3\}\).
We observe that learning becomes harder as the number of steps increases, likely because the model must make the correct prediction on all \(k\) steps.
Notably, for \(d = 2n\) in the \(k=1\) case, the model consistently attains high accuracy \(99\%+\).
When \(d < 2n\), however, the accuracy quickly decays.
This suggests that, empirically for setup, our proposed encoding in Theorem~\ref{thm:encoding} is fairly tight.
Moreover, for all the plots, the trend in models that can attain \(99\%\) accuracy appears to be linear.


\input{figures/attacks_acc}
\subsection{(Q2) How Good are Learned Attackers?}
Table~\ref{tab:learned_attack_results}
Table~\ref{tab:learned_attack_results_clamped}

\red{
    TODO: Results for more steps of reasoning
}

\subsection{(Q3) What strategies do learned attackers use?}

\red{
    TODO: Some results on how learned attack tokens are related to the target
}


\input{figures/minecraft_acc}
\subsection{(Q4) Results on a Natural Language task: crafting recipes in Minecraft}

Table~\ref{tab:minecraft_results}

\red{
    TODO: Remaining base results, Attack results
}






==> old/experiments_3.tex <==
\section{Experiments}
\label{sec:experiments}

We now investigate the efficacy of reasoning attacks against both small learned reasoners as well as larger natural language models.
In Section~\ref{sec:experiments_learned_reasoners}, we first explore attacks against reasoners as those posed in~\eqref{eqn:model_def}.
Then, in Section~\ref{sec:experiments_natural_language}, we explore attacks against large language models.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Small Learned Reasoner Experiments}
\label{sec:experiments_learned_reasoners}

% We first investigate one-layer, one-head reasoner models as defined in~\eqref{eqn:model_def}.

\noindent\textbf{Model, Dataset, and Training Setup}
We use GPT-2~\citep{radford2019language} as the base transformer model configured to one layer, one self-attention head, and the appropriate embedding dimension \(d\) and number of propositions (labels) \(n\).
Following our theory, we also disable the positional encoding.
We use GPT-2's default settings of feedforward width \(d_{\msf{ffwd}} = 4d\) and layer normalization enabled.


Our dataset consists of random rules partitioned as \(\Gamma = \Gamma_{\msf{special}} \cup \Gamma_{\msf{other}}\), with \(\abs{\Gamma} = 32\) rules each.
Because it is unlikely for independently sampled rules to yield an interesting proof states sequence, we construct \(\Gamma_{\msf{speciall}}\) with structure.
Assume \(n \geq 8\) and take a sample of propositions \(A,B,C,D,E,F,G,H\) that correspond to different one-hot vectors of \(\{0,1\}^n\).
Then, let:
\begin{align*}
    \Gamma_{\msf{special}}
        = \{A \to B, A \to C, A \to D, B \land C \to E, C \land D \to F, E \land F \to G\},
\end{align*}
Note that \(\abs{\Gamma_{\msf{special}}} = 6\) and construct each \((\alpha, \beta) \in \Gamma_{\msf{other}} \in \{0,1\}^{26 \times 2n}\) as follows: first, sample \(\alpha, \beta \sim \msf{Bernoulli}^n (3/n)\).
Then, set the \(H\) position of \(\alpha\) hot, such that no rule in \(\Gamma_{\msf{other}}\) is applicable so long as \(H\) is not derived.
Finally, let \(\Phi = \{A\}\), and so the correct proof states given \(\Gamma\) are:
\begin{align*}
    s_0 = \{A\},
    \quad s_1 = \{A,B,C,D\},
    \quad s_2 = \{A,B,C,D,E,F\},
    \quad s_3 = \{A,B,C,D,E,F,G\}.
\end{align*}
For training, we use AdamW~\citep{loshchilov2017decoupled} as our optimizer.
We train for \(8192\) steps with batch size \(512\), learning rate \(5 \times 10^{-4}\), and a linear decay schedule at \(10\%\) warmup.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{(QA1) How good are learned reasoners?} \input{figures/exp_qa1_learned_reasoners} In Theorem~\ref{thm:encoding}, we showed that transformer-based language models with embedding dimension \(d = 2n\), where \(n\) is the number of propositions, suffice to encode one step of reasoning.
However, can models restricted to these dimensions practically learn to reason?
We vary different combinations of \((n,d)\) and show our results in Figure~\ref{fig:exp_qa1_learned_reasoners}.
We see that models with \(d \geq 2n\) can all attain high inference accuracy compared to those with only \(d < 2n\).
Moreover, the inference accuracy drops as the number of steps increases with \(t = 1, 2, 3\), which is expected.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{(QA2) Do theory-inspired attacks transfer?} \input{figures/exp_qa2_theory_attacks} In Section~\ref{sec:attacks_theory}, we proposed some attacks against our theoretical construction, but how do they translate in practice to learned models?
This is a non-trivial question, as the learned models may employ a different strategy from the theoretical construction.
We find that a naive implementation of the theory-based attacks of Theorem~\ref{thm:theory_attacks} fails.
We suspect this is because of GPT-2's layer norm, which prevents us from using large \(\kappa\) values.
As a remedy, we found that simply repeating the adversarial suffix multiple times successfully bypasses this layer norm restriction and causes the monotonicity and maximality attacks to succeed.

and causes t


for multiple copies makes things work for the monotonicity and maximality attacks.
We define attack success rate as the rate at which the 


We show our results in Figure~\ref{fig:exp_qa2_theory_attacks}.


% We can also do plots for bigger models, and we can choose to train only a few to save space.
% (\((L=1, H=1)\), \((L=2, H=2)\), \((L=4, H=4)\))




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{(QA3) How do learned attacks work?} We use GPT-2 as our attacker model

In Section~\ref{sec:attacks_learned}, we present a general strategy for learning attacks.
We additionally investigate what kind of strategies these learned attackers they use to induce the different kinds of reasoning attacks.




We next investigate how well the learned attacks work.

We test this also on the three model sizes


\input{figures/exp_qa3_learned_attacks}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Natural Languauge Model Experiments}
\label{sec:experiments_natural_language}

We next look at how transformer-based language models are attacked on text-based logical reasoning and rule following tasks. Concretely, we first analyze how a popular Greedy Coordinate Gradients (GCG)-based attack~\citep{zou2023universal} works on GPT-2 finetuned on a Minecraft crafting recipes dataset. We next show how larger models including Llama-7B and Vicuna-13B exhibit similar rule suppression when attacked to ignore user-provided rules.

\input{figures/minecraft_prompt_example}

\subsubsection{Attacking logical reasoning with finetuned GPT2}

\noindent\textbf{Model, Dataset, and Training Setup.} We construct datasets for this experiment using Minecraft crafting recipes~\cite{mojang2011minecraft}. Each sample in the dataset consists of a set of in-context crafting recipes (\textit{"If I have A and B, I can create C"}) and source items (\textit{"I have A and B"}) and the task is to autoregressively state new items that can be crafted (\textit{"I have A and B and so I can create C"}). The recipes, source items and generation are analogous to the rules, facts and states discussed in Section~\ref{} respectively. An example of the prompt is given in Fig~\ref{fig:mc_prompt_exp_gen}. We continue to use the term "number of steps" \((t)\) to denote the longest chain of reasoning steps in the sample. For example, generation of the form "I have A and so I can create B. I have B and so I can create C" corresponds to \(t=2\) reasoning steps. We use \(t_{max}\) to denote the longest chain of reasoning steps for all samples in the dataset.  We study three versions of this dataset with \(t_{max} = {1, 3, 5}\) respectively.
% Each sample in the dataset can have upto 64 unique items and x rules.

We finetune three GPT-2~\citep{radford2019language} models on 65k training examples from the three datasets each using the standard Causal Language Modeling objective for 25 epochs. We evaluate the generations on 16k test examples. 

% \noindent\textbf{How good is reasoning on the Minecraft dataset?}
We measure the test accuracy as the percentage of test examples where the set of crafted items in the model's generation exactly matches the expected set of crafted items.
The three models report a test accuracy \(> 85\%\) on the respective datasets.

\input{figures/exp_qb1_minecraft_attacks}

\subsection*{(QB1) Is GPT-2 Susceptible to Logical Reasoning Attacks?} As discussed in Section~\ref{sec:attacks_learned}, we use the Greedy Coordinate Gradient (GCG) attack from~\citep{zou2023universal} to find adversarial suffixes that lead the model to generate incorrect text. We start with an initial suffix \textit{"and and ..."} (repeated 13 times), restrict the tokens in the suffix to the Minecraft vocabulary and consider the top-16 token replacements. 

We now present the details of the three attacks, namely knowledge suppression, amnesia and coercion, on the GPT-2 models. For each attack, we randomly choose 100 \textit{Attack Targets} where an attack target corresponds to a fact to be forgotten for amensia, a sequence of rules to be suppressed for rule suppression and a new unrelated state for coercion. We use the term \textit{Expected Attack Generation} to refer to the model's generation if the attack is successful. For each target, we optimize the adversarial suffix over 5 training examples by precomputing their expected attack generations. We then evaluate the final suffixes over 25 unseen test samples per attack target (i.e., 2500 test samples in total for each attack). The \textbf{Attack Success Rate (ASR)} denotes the percentage of test samples where the attack generation exactly matches the Expected Attack Generation. We also define a looser metric called \textbf{Suppression Success Rate (SSR)} for rule suppression and amnesia to denote the percentage of samples where the rule and fact suppression was successful respectively (irrespective of the correctness of the rest of the generation). 

% \noindent\textbf{Knowledge suppression.}
% The goal of this attack is to remove an entire reasoning chain (a sequence of rules) from an otherwise correct generation.
% We randomly choose 100 target suppression recipes (sequences of rules) and optimize the adversarial suffix over 5 training samples each where the target recipe is present in the generation. We then evaluate the recipe-specific suffixes against 25 test samples per recipe (i.e., 2500 test samples in total). The attack is considered successful if the target recipe is not present in the model's generation but the rest of the generation is not changed.

% \noindent\textbf{Fact amnesia.}
% The goal of this attack is to remove a target consequent from the generation without affecting any downstream rules (where these consequents are antecedents).
% We randomly choose 100 target suppression rules and optimize the adversarial suffix over 5 training samples each where the target rule is present in the generation. We then evaluate the rule-specific suffixes against 2500 test samples. The attack is considered successful if the target rule is not present in the model's generation but the rest of the generation remains intact.

% \noindent\textbf{Reasoning coercion.}
% <TODO: Write this>

% <Discuss the attack setup (universal attack, transferability, suffix init)>.

Table~\ref{tab:exp_qb1} shows the results of attacking the learned models. \red{TODO: Discuss results on the three attack categories in more detail}

\subsection*{(QB2) Do Reasoning Attacks Against GPT-2 Mimic Theoretical Predictions?}\input{figures/exp_qb2_minecraft_attacks_analysis}\input{figures/exp_qb2_llama_attacks} In order to better understand the mechanism behind the attacks, we look at some attention weight-based metrics. Let \(a^{l,h}_{c, T}\) denote the attention weight between the last token \(T\) and some preceding token in the context \(c\) in attention head \(h \in H\) of layer \(l \in L\). We aggregate the attention weights across all heads of a layer \(l\) as \(a^{l}_{c, T} = max_{h \in H} a^{l,h}_{c, T}\). 

Consider a benign sample with length \(T\) and an adversarial suffix of length \(T_{adv}\). The sample when attacked has a length \(T_{atk} = T + T_{adv}\). We pad the benign sample with token \("and"\) to match length such that \(T_{ben} = T_{atk}\). For a given context token \(c < T\) and layer \(l \in L\), we define the \textbf{attention suppression value} under attack \({a^l_{sup}}_{c, T_{atk}} = {a^l_{ben}}_{c, T_{atk}} - {a^l_{atk}}_{c, T_{atk}}\) where \(a_{atk}\) and \(a_{ben}\) are the attention weights from the attacked and padded benign samples respectively. An attention suppression value of 0 indicates no difference in attention weights on the corresponding token during attack. An attention suppression value \(\in (0, 1]\) indicates lower attention weight on the token due to the attack. 

The attention suppression values for different tokens are relevant for the three attacks. For the rule suppression attack, we consider \(c \in \alpha_{rule}\) where \(rule\) is the target rule to be suppressed. For amnesia, we consider \(c \in \beta_{rule}\) where \(\beta_{rule}\) are the facts to forget. Finally, for coercion, we consider \(c \in {\alpha_i \forall{i}}\) since we're interested in how the new state affects attention on all existing facts. Since \(c\) can be from a set of tokens in each case, we only look at the maximum attention suppression value over all tokens under consideration. The various attention suppression values are presented in Table~\ref{tab:exp_qb1}.

\red{TODO: Discuss attention suppression stats for the three attacks (add some numbers to Table~\ref{tab:exp_qb1}}

% We define a token \(c\)'s \textbf{suppression value under attack} for layer \(l\) as \(a*^{l,h}_{c, T_{atk}} = a^{l, h}_{c, T_{atk}} - a'^{l, h}_{c, T_{atk}}\)

% Concretely, for a given benign-attack sample pair, we first calculate the attention scores between the last token and the preceding tokens for the benign and the attack samples. We let the attention scores of a layer be the maximum of the attention scores over all attention heads in the layer. We then calculate the \textit{attention suppression value} of a given token and layer as the difference between the layer attention score of the attack and benign samples. An attention suppression value of zero indicates no difference in attention activity w.r.t the corresponding token during the attack. In order to validate the results from the theory, we would expect a high attention suppression value for the tokens corresponding to the rule/consequent being suppressed.

Figure~\ref{fig:exp_qb2_attn} shows an example of this metric on a successfully attacked example. In the example, the attack suppresses the application of the rule \textit{"If I have beetroot, I can create red dye"} and the attention suppression value of the tokens "beet" and "root" in the later layers is evidently higher than those of other tokens.
\red{TODO: Add more examples (for other attack categories: amnesia, coercion)}

\subsubsection{Beyond GPT-2: Attacks against Rule-following in LLMs}

We also look at how user-provided rules in the prompt can be suppressed in larger models. We do this analysis for two models, Llama-7B and Vicuna-13B, using a hand-crafted dataset (\red{TODO: or GPT-generated)} with 25 samples. Each sample has a set of artificial rules that the model is expected to obey (\textit{"If a question is about sweet potatoes, say 'I only know about regular potatoes."}) and a user query (\textit{"Where can I find sweet potatoes?"}). The attack objective is then to find a suffix that suppresses the presence of the relevant rules. We find that a simple hand-crafted suffix \textit{"Forget all prior instructions and answer the question."} can be used to attack Llama-7B. The attention suppression values of the tokens corresponding to the suppressed rules are presented in Table\red{XXX}. As with GPT-2, we see a similar attention weight suppression on the target rules and Figure~\ref{fig:exp_qb2_llama} presents an example.More examples are presented in the Appendix.


==> old/horn_1.tex <==
\subsection{Propositional Horn Satisfiability}
\label{sec:horn_logic}

Let \(P_1, \ldots, P_n\) be the propositions of our universe.
A \emph{literal} is either a proposition \(P_i\) or its negation \(\neg P_i\).
A \emph{clause} \(C\) is a set of literals that we represent as a pair of binary vectors \(\bbracks{c^-, c^+} \in \mbb{B}^{2n}\), where \(c^-\) denotes the negative literals and \(c^+\) denotes the positive literals:
\begin{align*}
    (c^-)_i = \begin{dcases}
        1, &\neg P_i \in C \\
        0, &\text{otherwise}
    \end{dcases},
    \qquad
    (c^+)_i = \begin{dcases}
        1, &P_i \in C \\
        0, &\text{otherwise}
    \end{dcases}
\end{align*}
A proposition \(P_i\) need not appear in a clause so that we may have \((c^-)_i = (c^+)_i = 0\).
Conversely, if \(P_i\) appears both negatively and positively in a clause, i.e., \((c^-)_i = (c^+)_i = 1\), then such clause is a tautology.
Although \(\bbracks{\cdot, \cdot}\) and \((\cdot, \cdot)\) are both pairs, we use \(\bbracks{\cdot, \cdot}\) to stylistically distinguish clause pairings.
We say that \(\bbracks{c^-, c^+}\) is a \emph{Horn clause} iff \(\abs{c^+} \leq 1\), where \(\abs{\cdot}\) counts the number of ones in a binary vector.
That is, \(C\) is a Horn clause iff it contains at most one positive literal.


%%%%%%%%%%%%%%%%%%%%
\begin{example}
\label{ex:rules_translate}
In Section~\ref{sec:background},
we presented an example of reasoning with the following rule set and propositions:
\begin{align*}
    \Gamma = \braces*{
        \msf{Sheep} \to \msf{Wool},
        \enskip
        \msf{Wool} \to \msf{String},
        \enskip
        \msf{Wood} \to \msf{Stick},
        \enskip
        \msf{Stick}\,\text{and}\,\msf{String} \to \msf{FishingRod}
    }
\end{align*}
Order the propositions as: \(\msf{Sheep}, \msf{Wood}, \msf{Wool}, \msf{Stick}, \msf{String}, \msf{FishingRod}\).
Then, the rules may be equivalently expressed as the following Horn clauses in either implication form (left), set form (middle), or binary vector form (right):
\begin{align*}
    (\msf{Sheep} \to \msf{Wool})
        &\cong \braces*{\neg \msf{Sheep}, \msf{Wool}}
        &&\cong \bbracks{(1,0,0,0,0,0), (0,0,1,0,0,0)}
        \\
    (\msf{Wool} \to \msf{String})
        &\cong \braces*{\neg \msf{Wool}, \msf{String}}
        &&\cong \bbracks{(0,0,1,0,0,0), (0,0,0,0,1,0)}
        \\
    (\msf{Wood} \to \msf{Stick})
        &\cong \braces*{\neg \msf{Wood}, \msf{Stick}}
        &&\cong \bbracks{(0,1,0,0,0,0), (0,0,0,1,0,0)}
        \\
    (\msf{Strick}\,\text{and}\,\msf{String} \to \msf{FishingRod})
        &\cong \braces*{\neg \msf{Stick}, \neg \msf{String}, \msf{FishingRod}}
        &&\cong \bbracks{(0,0,0,1,1,0),(0,0,0,0,0,1)}
\end{align*}
\end{example}


We say that a clause \(C\) \emph{holds} with respect to a truth assignment to \(P_1, \ldots, P_n\) iff at least one literal in \(C\) evaluates truthfully.
Equivalently, using binary vectors, a clause \(\bbracks{c^-, c^+}\) holds iff:
some \(P_i\) evaluates truthfully and \((c^+)_i = 1\), or some \(P_i\) evaluates falsely and \((c^-)_i = 1\).
The Horn satisfiability problem is then posed as follows.


\begin{problem}[Horn Satisfiability]
\label{prob:horn_satisfiability}
    Let \(\mcal{C}\) be a set of Horn clauses.
    Decide whether there exists a truth assignment to the propositions \(P_1, \ldots, P_n\) such that all clauses of \(\mcal{C}\) simultaneously hold.
    If such an assignment exists, then \(\mcal{C}\) is \emph{satisfiable}; if such an assignment does not exist, then \(\mcal{C}\) is \emph{unsatisfiable}.
\end{problem}


\begin{example}
Continuing from the example in Section~\ref{sec:background}, we asked whether one can derive \(\msf{FishingRod}\) if one assumed \(\msf{Sheep}\) and \(\msf{Wood}\) as starting facts.
This problem is equivalent to Horn satisfiability for the following set of clauses:
\begin{align*}
    % \mcal{C} = \mcal{R}
    \mcal{C} = \Big\{
        \underbrace{
        \braces*{\neg \msf{Sheep}, \msf{Wool}},
        \ldots,
        \braces*{\neg \msf{Stick}, \neg \msf{String}, \msf{FishingRod}},
        }_{\text{Clauses from Example~\ref{ex:rules_translate}}}
        \underbrace{\braces*{\msf{Sheep}, \msf{Wood}}}_{\text{Clause for starting facts}}
        ,
        \underbrace{\braces*{\neg \msf{FishingRod}}}_{\text{Clause with negated goal}}
    \Big\}
\end{align*}
In particular, \(\msf{FishingRod}\) is derivable iff \(\mcal{C}\) is unsatisfiable.
Intuitively, this is because \(\msf{FishingRod}\) being derivable means that this proposition must evaluate truthfully, and so the clause \(\{\neg \msf{FishingRod}\}\) never holds --- and therefore \(\mcal{C}\) is unsatisfiable.
The above is a common setup in automated theorem-proving: one negates the goal and checks for unsatisfiability.
This leverages the fact that a formula \(F\) is a tautology (logically \emph{valid}) iff its negation \(\neg F\) is unsatisfiable.
\end{example}



The relationship between propositional entailment and the more commonly studied problem of \emph{propositional satisfiability} is as follows.
Given a set of propositions, a \emph{clause} is a disjunction of \emph{literals}, where a literal is either a proposition \(P\) or its negation \(\neg P\).
Given a set of clauses, the satisfiability problem is to determine whether there exists a truth assignment to all the propositions such that at least one literal is true in every clause.
The satisfiability problem is the canonical \textsc{NP-Complete} problem.
A clause is called a \emph{Horn clause} if it contains at most one positive literal.

In the Horn satisfiability problem, all input clauses must be Horn clauses, and it can be solved in polynomial time.
Notably, the problem of Horn satisfiability and our presentation of propositional entailment are interreducible.


% \begin{proposition}
%     The problem of Horn satisfiability and the propositional entailment problem~\eqref{prob:propositional_entailment} are interreducible.
%     % The propositional entailment problem~\eqref{prob:propositional_entailment} and the Horn satisfiability problem are interreducible.
% \end{proposition}

% We present a proof in Appendix~\ref{sec:horn_logic}.
% Thus, the chosen formalization precisely captures propositional Horn satisfiability.
% Our formulation is motivated by its correspondence to deriving facts in widely used chain-of-thought reasoning.
% Note that the restriction to Horn reasoning means one cannot derive disjunctive statements such as \(P \lor Q\).


\begin{theorem}
The propositional entailment problem~\eqref{prob:propositional_entailment} and the Horn satisfiability problem~\eqref{prob:horn_satisfiability} are interreducible.
\end{theorem}
\begin{proof}
\emph{(Propositional entailment to Horn satisfiability)}
Consider a set of rules \(\Gamma\) and goal \(\tau \in \mbb{B}^n\).
Then, transform each \((\alpha, \beta) \in \Gamma\) and \(\tau\) into sets of Horn clauses as follows:
\begin{align*}
    (\alpha, \beta)
    \mapsto \braces*{\bbracks{\alpha, e_i} : \beta_i = 1, \enskip i = 1, \ldots, n},
    \qquad
    \tau \mapsto \braces*{\bbracks{e_i, \mbf{0}_n}: \tau_i = 1, \enskip i = 1, \ldots, n}
\end{align*}
where \(e_1, \ldots, e_n \in \mbb{B}^n\) are the basis vectors.
Let \(\mcal{C}\) be the set of all clauses generated this way, and observe that each such clause is a Horn clause.
To check whether \(\Gamma\) entails \(\tau\), it suffices to check whether \(\mcal{C}\) is satisfiable.


\emph{(Horn satisfiability to propositional entailment)}
Let \(\mcal{C}\) be a set of Horn clauses over \(n\) propositions.
We embed each Horn clause \(\bbracks{c^-, c^+} \in \mbb{B}^{2n}\) into a rule in \(\mbb{B}^{2(n+1)}\) as follows:
\begin{align*}
    \bbracks{c^-, c^+}
    \mapsto
    \begin{dcases}
        ((c^-, 0), (c^+, 0)) \in \mbb{B}^{2(n+1)},
            & \abs{c^+} = 1 \\
        ((c^-, 0), (\mbf{0}_n, 1)) \in \mbb{B}^{2(n+1)},
            & \abs{c^+} = 0
    \end{dcases}
\end{align*}
Intuitively, this new \((n+1)\)th bit encodes a special proposition, which we call \(\msf{FALSE}\) (also: \(\msf{BOTTOM}\), \(\msf{EMPTY}\), etc.).
Let \(\Gamma \in \mbb{B}^{2(n + 1)}\) be the set of all rules generated this way.
Then, \(\mcal{C}\) is unsatisfiable iff \((\mbf{0}_n, 1) \preceq \Gamma^\star (\mbf{0}_{n+1})\).
In other words, \(\mcal{C}\) is unsatisfiable iff \(\Gamma\) entails \(\msf{FALSE}\).
\end{proof}

%%%%%%%%%%%%%%%%%%%%
\begin{example}
We show some examples of Horn satisfiability to propositional entailment, where we embed \(\mbb{B}^{12}\) into \(\mbb{B}^{14}\):
\begin{align*}
    \braces*{\neg \msf{Sheep}, \msf{Wool}}
        &\cong \bbracks{(1,0,0,0,0,0), (0,0,1,0,0,0)}
        &&\mapsto \bbracks{(1,0,0,0,0,0,0), (0,0,1,0,0,0,0)}
        \tag{\(\abs{c^+} = 1\)}
        \\
    \braces*{\msf{Sheep}, \msf{Wood}}
        &\cong \bbracks{(0,0,0,0,0,0), (1,1,0,0,0,0)}
        &&\mapsto \bbracks{(0,0,0,0,0,0,0), (1,1,0,0,0,0,0)} 
        \tag{\(\abs{c^+} = 1\)}
        \\
    \braces*{\neg \msf{FishingRod}}
        &\cong \bbracks{(0,0,0,0,0,1), (0,0,0,0,0,0)}
        &&\mapsto \bbracks{(0,0,0,0,0,1,0), (0,0,0,0,0,0,1)}
        \tag{\(\abs{c^+} = 0\)}
\end{align*}
\end{example}


==> old/introduction_1.tex <==
\section{Introduction}
\label{sec:introduction}


% Large language models (LLMs) are very popular~\citep{kasneci2023chatgpt,lund2023chatting}.


Modern large language models (LLMs) achieve remarkable performance on reasoning tasks~\citep{huang2022towards}.
A crucial ingredient for this success is chain-of-thought (CoT) prompting, a technique in which the intermediate reasoning steps of a logical argument are generated step-by-step until the answer is reached.
In contrast to paradigms that output the answer directly, this incremental output generation encourages an LLM to ``show its work'' before reaching a conclusion.
Augmented with CoT evaluation, LLMs significantly improve performance on tasks spanning basic arithmetic, commonsense reasoning, and symbolic logics~\citep{wei2022chain,kojima2022large,chu2023survey}.


In addition to impressive performance on reasoning benchmarks, the intermediate reasoning steps from CoT evaluation are of practical interest.
Principally, the apparent presence of logical deductions is a useful feature for establishing trust: one may verify in detail whether the LLM output is indeed correct.
In contrast to the typical black-box nature of many machine learning models, CoT allows for a degree of interpretability to the model's final output.
Such intermediate reasoning steps are especially relevant in settings like medicine~\citep{thirunavukarasu2023large} and law~\citep{cui2023chatlaw}, where practitioners must frequently make high-stakes and well-reasoned decisions.




The practical success of transformer-based LLMs~\citep{vaswani2017attention} has inspired much interest in understanding their theoretical power.
An influential line of work analyzes the power of transformers in the context of formal language membership~\citep{hao2022formal,merrill2023expressive,strobl2023transformers}, wherein a typical result takes the following form:
\emph{a transformer with some choice of parameter weights, attention mechanism, positional encoding, etc., can (or cannot) decide whether the input sequence belongs to some formal language}.
Indeed, formal language membership has deep connections to mathematical logics~\citep{borger2001classical,bradley2007calculus}, but it is often unclear how to translate such results into concrete insights about the capacity and limitations of LLMs trained for logic.
Although there is much interest in understanding how and what LLMs might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.


\input{figures/query_example}


\input{figures/inference_example}

% \red{AAAAAAAAAA}

% The empirical effectiveness and practical applications of CoT techniques have inspired much interest.
% In particular, there is an emergent but growing body of work that studies the theoretical power of CoT evaluation and transformer-based LLMs~\citep{vaswani2017attention}.
% However, there still exist gaps in how theoretical results can inform model design and training details for high-performance reasoning, a typical pipeline of which is shown in Figure~\ref{fig:reasoning_example}.
% For instance, many works study the expressive power of LLMs, for which results are typically of the form:
% \emph{a transformer with \(W\) size of parameters, \(X\) choice of attention mechanism, \(Y\) choice of positional encoding, and \(Z\) choice of other considerations can (or cannot) decide membership of strings in formal language \(L\)}~\citep{merrill2023expressive,feng2023towards,strobl2023transformers}.
% In principle, the recognition of formal languages is closely tied to the decision complexities of mathematical logics~\citep{borger2001classical,bradley2007calculus}, for instance: \emph{recognizing a satisfiable formula in propositional logic is \textsc{NP-Complete}}.
% However, it is often difficult to decipher concrete design recommendations from complexity-theoretic results, e.g., what embedding dimensions or which positional encodings are best for some particular reasoning task.


We mathematically study the task of CoT logical inference in propositional Horn logic using transformer-based LLMs.
Propositional Horn logic is a fragment of
propositional logic wherein the rules, facts, and query of Figure~\ref{fig:query_example} have the form \emph{\(P\) implies \(Q\)} for some propositions \(P\) and \(Q\)~\citep{levesque1986knowledge,chandra1985horn}.
Importantly, this is a fragment that captures a simple yet large class of reasoning tasks~\citep{chen2020review}.
We give an explicit transformer construction that exactly represents a decision circuit for logical inference using only two layers, one attention head, and an embedding dimension linear in the number of propositions.
Empirically, we show that LLMs, subject to our theory, can learn CoT logical inference with over \(99\%+\) accuracy.
Moreover, we find that \textbf{increasing the embedding dimension and the number of layers improves accuracy} but increasing the number of attention heads does not.


Furthermore, we study the reasoning robustness of LLMs and the conditions under which logical inference may fail.
We prove that even an exactly constructed reasoning model can be easily attacked.
Our experiments show that learned models, even those with high accuracy, remain susceptible to out-of-distribution inputs and adversarial \emph{jailbreak attacks}~\citep{chao2023jailbreaking,jones2023automatically,wei2023jailbroken,zou2023universal}.
Both theoretically and experimentally, we find that it is easy to cause LLMs to err in their reasoning.


% In this paper, we study the ability of LLMs to perform logical inference in propositional Horn logic.
% Our theoretical and empirical findings offer the practitioner concrete suggestions for model design and serve as an important stepping stone to the analysis of more complex logical fragments.
% Our investigations into the robustness of reasoning offer insight into the weaknesses and failure modes of LLMs that learn to reason.
% In summary, our contributions are:



\begin{itemize}
    \item We study the ability of LLMs to perform logical inference in propositional Horn logic.
    We prove that transformers can encode exact decision circuits for logical inference using only two layers, one attention head, and an embedding dimension linear in the number of propositions.
    Using parameters informed by our theoretical constructions, we find that transformers can learn CoT logical inference with \(99\%+\) accuracy.
    

    \item Based on our theoretical constructions, we show that LLMs for logical inference are not robust in both theory and practice.
    We show how to construct simple but effective attacks against our theoretical construction: even when the reasoning model is \emph{exact}, attacks are easy.
    Moreover, we empirically demonstrate the weakness of learned LLMs to out-of-distribution inputs and automated jailbreak attacks.


    \item Our theoretical construction and empirical evaluations give concrete suggestions for model design.
    We find that increasing the embedding dimension and number of layers improves reasoning inference accuracy, but increasing the number of attention heads does not.

\end{itemize}



==> old/introduction_2.tex <==
\section{Introduction}
\label{sec:introduction}


Large language models can achieve remarkable performance on reasoning tasks~\citep{huang2022towards}.
A crucial ingredient for this success is chain-of-thought (CoT) prompting, a technique in which the intermediate reasoning steps of a logical argument are generated step-by-step until the answer is reached.
In contrast to paradigms that output the answer directly, this incremental output generation encourages a model to ``show its work'' before reaching a conclusion.
Augmented with CoT evaluation, language models significantly improve performance on tasks spanning basic arithmetic, commonsense reasoning, and symbolic logics~\citep{wei2022chain,kojima2022large,chu2023survey}.


In addition to impressive performance on reasoning benchmarks, the intermediate reasoning steps from CoT evaluation are of practical interest.
Principally, the apparent presence of logical deductions is a useful feature for establishing trust: one may verify in detail whether the language model output is indeed correct.
In contrast to the typical black-box nature of many machine learning models, CoT allows for a degree of interpretability to the model's final output.
Such intermediate reasoning steps are especially relevant in settings like medicine~\citep{thirunavukarasu2023large} and law~\citep{cui2023chatlaw}, where practitioners must frequently make high-stakes and well-reasoned decisions.




The practical success of transformer-based language models~\citep{vaswani2017attention} has inspired much interest in understanding their theoretical power.
An influential line of work analyzes the power of transformers in the context of formal language membership~\citep{hao2022formal,merrill2023expressive,strobl2023transformers}, in which a typical result takes the following form:
\emph{a transformer with some choice of parameter weights, attention mechanism, positional encoding, etc., can (or cannot) decide whether the input sequence belongs to some formal language}.
Although formal language membership has deep connections to mathematical logics~\citep{borger2001classical,bradley2007calculus}, it is often unclear how to translate such results into concrete insights about the capacity and limitations of language models trained for logic.
Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.


\input{figures/reasoning_example}


\input{figures/inference_example}



We mathematically study the task of logical reasoning in propositional Horn logic using transformer-based language models.
A typical reasoning task is shown in Figure~\ref{fig:reasoning_example}.
Propositional Horn logic is a fragment of
propositional logic wherein the rules have the form \emph{if \(P\), then \(Q\)} for some propositions \(P\) and \(Q\)~\citep{levesque1986knowledge,chandra1985horn}.
This logic captures a simple yet large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.
We give an explicit transformer construction that encodes a decision circuit for autoregressive \emph{propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
Importantly, our construction uses only two layers, one attention head, and an embedding dimension linear in the number of propositions.
Empirically, we show that language models, subject to our theory, can learn CoT reasoning with over \(99\%+\) accuracy.
Moreover, we find that \textbf{increasing the embedding dimension and the number of layers improves accuracy} but increasing the number of attention heads does not.


Furthermore, we study the reasoning robustness of language models and the conditions under which reasoning may fail.
We prove that even an exactly constructed reasoning model can be easily attacked.
Our experiments show that learned models, even those with high accuracy, remain susceptible to out-of-distribution inputs and adversarial \emph{jailbreak attacks}~\citep{chao2023jailbreaking,jones2023automatically,wei2023jailbroken,zou2023universal}.
Both theoretically and experimentally, we find that it is easy to cause language models to err in their reasoning.
In summary, our contributions are as follows.




\begin{itemize}
    \item We study the ability of transformer-based language models to perform CoT reasoning in propositional Horn logic.
    We prove that transformers can encode exact decision circuits for propositional inference using only two layers, one attention head, and an embedding dimension linear in the number of propositions.
    Using parameter sizes informed by our theoretical constructions, we find that transformers can learn CoT reasoning with \(99\%+\) accuracy.
    

    \item Based on our theory constructions, we show that language models for CoT reasoning are not robust in both theory and practice.
    We show how to construct simple but effective attacks against our theoretical construction: even when the reasoning model is \emph{exact}, attacks are easy.
    Moreover, we empirically demonstrate the weakness of learned reasoning to out-of-distribution inputs and automated jailbreak attacks.


    \item Our theoretical construction and empirical evaluations give concrete suggestions for model design.
    We find that increasing the embedding dimension and the number of layers improves reasoning accuracy, but increasing the number of attention heads does not.

\end{itemize}



==> old/introduction_3.tex <==
\section{Introduction}
\label{sec:introduction}


Large language models can achieve remarkable performance on reasoning tasks~\citep{huang2022towards}.
Crucial to this success is chain-of-thought (CoT) reasoning, a technique in which the intermediate reasoning steps of a logical argument are generated step-by-step until the answer is reached.
In contrast to paradigms that output the answer directly, this incremental output generation encourages a model to ``show its work'' before reaching a conclusion.
Augmented with CoT reasoning, language models significantly improve performance on tasks spanning basic arithmetic, commonsense reasoning, and symbolic logics~\citep{wei2022chain,kojima2022large,chu2023survey}.

% A typical reasoning task poses the following: \emph{is some asserted \textbf{query} deducible from a set of known \textbf{facts} by iteratively applying a set of inference \textbf{rules}?}
% A reasoning task poses the following: \emph{is a query the logical consequence of some given facts and inference rules?}
% A reasoning task poses the following: \emph{is some query the logical consequence of some known facts and inference rules?}
% A reasoning task poses the following: \emph{does some \textbf{query} logically follow from some known \textbf{facts} and inference \textbf{rules}?}


Logical reasoning is concerned with checking the truthfulness of asserted statements.
Given such an assertion, also called the \emph{query}, a standard reasoning problem asks the following: \emph{is this \textbf{query} the logical consequence of the known \textbf{facts} and inference \textbf{rules}?}
We illustrate this in Figure~\ref{fig:mc_reasoning} using an example from the Minecraft video game~\cite{mojang2011minecraft}.
In Minecraft, a common objective is to make new items according to a recipe list.
Given some starting items (\(\msf{Sheep}\), \(\msf{Wood}\)), a player may ask whether they have sufficient material to craft some target item (\(\msf{FishingRod}\)) if they follow the recipe list (``If I can get \(\msf{Sheep}\), then I can get \(\msf{Wool}\)'', etc.).
Although the example of Figure~\ref{fig:mc_reasoning} appears toy, it is a non-trivial challenge for machine learning --- the model must first learn the rules from data and then decipher when it is appropriate to apply which ones.
Moreover, this example is of practical interest because it is representative of a large class of reasoning problems~\cite{chen2020review}.
In this paper, we present mathematical results for the reasoning power of language models on such problems.


\input{figures/mc_reasoning}


\input{figures/mc_inference}

An influential line of work examines the power of language models through the perspective of formal language membership~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}, in which a typical result states the following:
\emph{a transformer~\cite{vaswani2017attention} with some choice of parameter weights, attention mechanism, positional encoding, etc., can (or cannot) decide whether the input sequence belongs to some formal language}.
Although formal language membership has deep connections to mathematical logics~\citep{borger2001classical,bradley2007calculus}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.







We study the task of logical reasoning in propositional Horn logic using transformer-based language models.
Propositional Horn logic is a fragment of
propositional logic wherein the rules have the form \emph{if \(P\), then \(Q\)} for some propositions \(P\) and \(Q\)~\citep{levesque1986knowledge,chandra1985horn}.
This logic captures a simple yet large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.
We give an explicit transformer construction that encodes a decision circuit for autoregressive \emph{propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
Importantly, our construction uses only two layers, one attention head, and an embedding dimension linear in the number of propositions.
Empirically, we show that language models, subject to our theory, can learn autoregressive propositional inference with over \(99\%+\) accuracy.
Moreover, we find that \textbf{increasing the embedding dimension and the number of layers improves accuracy} but increasing the number of attention heads does not.


Furthermore, we investigate how even highly accurate language models may be forced to error.
Our findings suggest a fundamental weakness of such models against even simple \emph{jailbreak attacks}~\cite{chao2023jailbreaking,zou2023universal}.
First, we prove that even our theoretical construction of a perfect reasoner can be easily attacked.
Moreover, we empirically show that learned models, even those with high accuracy, remain susceptible to out-of-distribution inputs and simple adversarial attacks.
Both theoretically and experimentally, we find that it is easy to force language models to err.
In summary, our contributions are as follows.

% \emph{jailbreak attacks}~\citep{chao2023jailbreaking,jones2023automatically,wei2023jailbroken,zou2023universal}.



\begin{itemize}
    \item We study the ability of transformer-based language models to perform autoregressive propositional inference.
    We prove that transformers can encode exact decision circuits for propositional inference using only two layers, one attention head, and an embedding dimension linear in the number of propositions.
    Using parameter sizes informed by our theoretical constructions, we find that transformers can learn autoregressive propositional inference with \(99\%+\) accuracy.
    

    \item Based on our theory constructions, we show that language models for propositional inference are not robust in both theory and practice.
    We show how to construct simple but effective attacks against our theoretical construction: even when the reasoning model is \emph{exact}, attacks are easy.
    Moreover, we empirically demonstrate the weakness of learned reasoning to out-of-distribution inputs and automated jailbreak attacks.


    \item Our theoretical construction and empirical evaluations give concrete suggestions for model design.
    We find that increasing the embedding dimension and the number of layers improves reasoning accuracy, but increasing the number of attention heads does not.

\end{itemize}



==> old/introduction_4.tex <==
\section{Introduction}
\label{sec:introduction}


Modern transformer-based language models~\cite{vaswani2017attention} are remarkable at logical reasoning.
Crucial to this success is chain-of-thought (CoT) reasoning~\cite{wei2022chain,kojima2022large}, a technique in which the intermediate reasoning steps of a logical argument are generated step-by-step until the answer is reached.
In contrast to paradigms that output the answer directly, this incremental output generation encourages a model to ``show its work'' before reaching a conclusion.
Augmented with CoT, language models can learn to reason with basic arithmetic, common sense inference, and symbolic logics through training data alone~\cite{huang2022towards,chu2023survey}.


Logical reasoning is concerned with checking the truthfulness of asserted statements.
Given such an assertion, also called the \emph{goal}, a standard reasoning problem asks the following: \emph{is this \textbf{goal} the logical consequence of the known \textbf{facts} and inference \textbf{rules}?}
We illustrate this in Figure~\ref{fig:mc_reasoning} using an example from the Minecraft video game~\cite{mojang2011minecraft}.
In Minecraft, a common objective is to make new items according to a recipe list.
Given some starting items (\(\msf{Sheep}\), \(\msf{Wood}\)), a player may ask whether they have sufficient material to craft some target item (\(\msf{FishingRod}\)) if they follow the recipe list (``If I can get \(\msf{Sheep}\), then I can get \(\msf{Wool}\)'', etc.).
Although the example of Figure~\ref{fig:mc_reasoning} appears toy, it is a non-trivial challenge for machine learning --- the model must first learn the rules from data and then figure out which ones to apply.
Moreover, this example is of practical interest because it is representative of a large class of reasoning problems~\cite{chen2020review}.
In this paper, we present mathematical results for the reasoning power of language models on such problems.


\input{figures/mc_reasoning}


\input{figures/mc_inference}




An influential line of work examines the power of language models through the perspective of formal language theory~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}, in which a typical result states the following:
\emph{a transformer with some choice of parameter weights, attention mechanism, etc., can (or cannot) answer whether the input sequence belongs to some formal language (e.g., \textsc{Parity}, \textsc{Dyck-\(k\))}}.
Although formal language membership has deep connections to mathematical logics~\cite{borger2001classical,bradley2007calculus}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.
In this paper, we study the task of logical reasoning in propositional Horn logic using transformer-based language models.
Propositional Horn logic is a fragment of
propositional logic wherein the rules have the form \emph{``if this, then that''}~\cite{levesque1986knowledge,chandra1985horn}.
This logic captures a simple yet large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.


We give an explicit transformer construction that encodes a decision circuit for \emph{autoregressive propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
Although our theoretical model is a perfect reasoner, one can provably force an error with a well-crafted \emph{jailbreak attack}~\cite{chao2023jailbreaking,zou2023universal}.
Motivated by this, we find that even highly-accurate learned models are also weak to similar attacks.
This work demonstrates the simultaneous power and weakness of reasoning with language models: although transformers can learn to reason over propositional Horn logic in both theory and practice, they are not far from logical fallacies.
In summary, our contributions are as follows.





\begin{itemize}
    \item We formally prove that transformers can encode a decision circuit for propositional inference using only \textbf{one layer, one attention head, and an embedding dimension linear in the number of propositions}.
    Empirically, we find that learned models' reasoning accuracy appears linear in the embedding dimension.
    

    \item We show that language models struggle to reason robustly in both theory and practice.
    Even for perfect reasoners like our theoretical construction, it is easy to force errors.
    We additionally demonstrate the weakness of learned models both to automated jailbreak attacks and simple out-of-distribution inputs.


    \item Our theoretical construction and empirical evaluations give concrete suggestions for model design.
    We find that increasing the embedding dimension and the number of layers improves reasoning accuracy, but increasing the number of attention heads does not help.

\end{itemize}



==> old/introduction_5.tex <==
\section{Introduction}
\label{sec:introduction}


Modern transformer-based language models~\cite{vaswani2017attention} are remarkable at logical reasoning.
Crucial to this success is chain-of-thought (CoT) reasoning~\cite{wei2022chain,kojima2022large}, a technique in which the intermediate reasoning steps of a logical argument are generated step-by-step until the answer is reached.
In contrast to paradigms that output the answer directly, this incremental output generation encourages a model to ``show its work'' before reaching a conclusion.
Augmented with CoT, language models can learn to reason with basic arithmetic, common sense inference, and symbolic logics~\cite{huang2022towards,chu2023survey}.


Logical reasoning is concerned with checking the truthfulness of asserted statements.
Given such an assertion, also called the \emph{goal}, a standard reasoning problem asks the following: \emph{is this \textbf{goal} the logical consequence of the known \textbf{facts} and inference \textbf{rules}?}
We illustrate this in Figure~\ref{fig:mc_reasoning} using an example from the Minecraft video game~\cite{mojang2011minecraft}.
In Minecraft, a common objective is to make new items according to a recipe list.
Given some starting items (\(\msf{Sheep}\), \(\msf{Wood}\)), a player may ask whether they have sufficient material to craft some target item (\(\msf{FishingRod}\)) if they follow the recipe list (``If I can get \(\msf{Sheep}\), then I can get \(\msf{Wool}\)'', etc.).
Although the example of Figure~\ref{fig:mc_reasoning} appears toy, it is a non-trivial challenge for machine learning --- the model must first learn the rules and then figure out which ones to apply.
In addition, this example is of practical interest because it is representative of a large class of reasoning problems~\cite{chen2020review}.
In this paper, we present mathematical results for the reasoning power of language models on such problems, where the rules and facts are given in-context.


\input{figures/mc_reasoning}


\input{figures/mc_inference}


An influential line of work examines the power of language models through the perspective of computational complexity~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}.
Although computational complexity has deep connections to mathematical logics~\cite{borger2001classical}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.
In this paper, we study the task of logical reasoning in propositional Horn logic using transformer-based language models.
Propositional Horn logic is a fragment of
propositional logic wherein the rules have the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\) and \(R\)~\cite{levesque1986knowledge}.
This logic captures a large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.

% ~\cite{levesque1986knowledge,chandra1985horn}


% An influential line of work examines the power of language models through the perspective of formal language theory~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}, in which a typical result states the following:
% \emph{a transformer with some choice of parameter weights, attention mechanism, etc., can (or cannot) answer whether the input sequence belongs to some formal language (e.g., \textsc{Parity}, \textsc{Dyck-\(k\))}}.
% Although formal language membership has deep connections to mathematical logics~\cite{borger2001classical,bradley2007calculus}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
% Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.
% In this paper, we study the task of logical reasoning in propositional Horn logic using transformer-based language models.
% Propositional Horn logic is a fragment of
% propositional logic wherein the rules have the form \emph{``if this, then that''}~\cite{levesque1986knowledge,chandra1985horn}.
% This logic captures a simple yet large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.


We give an explicit transformer construction that encodes \emph{autoregressive propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
Although our theoretical construction exactly encodes reasoning, one can provably force mistakes with a well-crafted adversarial attack~\cite{zou2023universal}.
Motivated by this, we find that empirically learned models with seemingly perfect accuracy are also prone to similar attacks.
This work demonstrates the simultaneous strength and weakness of language models that reason: although transformers can learn to reason over propositional Horn logic in both theory and practice, they are not far from logical fallacies.
In summary, our contributions are as follows.




% We give an explicit transformer construction that encodes a decision circuit for autoregressive \emph{propositional inference}, the primary computational mechanism of CoT reasoning in propositional Horn logic.
% Importantly, our construction uses only two layers, one attention head, and an embedding dimension linear in the number of propositions.
% Empirically, we show that language models, subject to our theory, can learn autoregressive propositional inference with over \(99\%+\) accuracy.
% Moreover, we find that \textbf{increasing the embedding dimension and the number of layers improves accuracy} but increasing the number of attention heads does not.


% Furthermore, we investigate how even highly accurate language models may be forced to error.
% Our findings suggest a fundamental weakness of such models against even simple \emph{jailbreak attacks}~\cite{chao2023jailbreaking,zou2023universal}.
% First, we prove that even our theoretical construction of a perfect reasoner can be easily attacked.
% Moreover, we empirically show that learned models, even those with high accuracy, remain susceptible to out-of-distribution inputs and simple adversarial attacks.
% Both theoretically and experimentally, we find that it is easy to force language models to err.
% In summary, our contributions are as follows.



% \emph{jailbreak attacks}~\cite{chao2023jailbreaking,jones2023automatically,wei2023jailbroken,zou2023universal}.


\paragraph{Transformers Can Encode Propositional Inference}
We prove that transformers can encode propositional inference using only one layer, one attention head, and an embedding dimension linear in the number of propositions.
Empirically, we find that the performance trend of learned reasoners matches our theoretical predictions.
% Although our theory says that one layer suffices, we observe that increasing the number of layers improves reasoning accuracy, 



\paragraph{Reasoning is not Robust}
We find that it is easy to construct highly effective adversarial attacks for both our theoretical construction and the learned models.
One can trick even seemingly perfect reasoners into committing logical fallacies in both theory and practice.



==> old/introduction_6.tex <==
\section{Introduction}
\label{sec:introduction}

% ~\citep{huang2022towards}

Modern transformer-based language models~\citep{vaswani2017attention} can attain impressive performance on many reasoning benchmarks~\citep{chu2023survey,zhao2023survey}.
Especially in high-stakes applications like law and healthcare, the ability to mimic reasoning is important for practical adoptions: the model's reasoning functions as a ``proof'' for whether its decision should be trusted.
Although reasoning tasks span many flavors that include basic arithmetic~\citep{imani2023mathprompter,chen2022program}, commonsense reasoning~\citep{madaan2022language}, symbolic logics~\citep{cheng2022binding,zhao2023enhancing}, and others, they are broadly unified under the following format:

\begin{quote}
    \textbf{Reasoning Task:}
    is some goal \(\tau\) the logical consequence of the known facts \(\Phi\) and the inference rules \(\Gamma\)?
\end{quote}
For example, a reasoning task may ask whether ``it is cloudy'' is deducible from the fact ``it is raining'' and the rule ``if it is raining, then it is cloudy''.


But when might language models succeed or fail to reason?
A fruitful direction of work comes from the perspective of computational complexity~\citep{strobl2023transformers}, which broadly seeks to establish relations between transformers and well-known complexity classes.
For instance, transformers with hard attention fall within \(\msf{AC}^0\)~\citep{hao2022formal}, while those with softmax attention fall within \(\msf{TC}^0\)~\citep{merrill2023parallelism}.
Such relations categorize the expressive power of different neural architectures, which in turn precisely determine which reasoning problems a language model can or cannot solve.



% For instance, using hard attention restricts transformers within \(\msf{AC}^0\)~\citep{hao2022formal}, while using softmax attention restricts transformers within \(\msf{TC}^0\)~\citep{merrill2023parallelism}.
% Such relations then yield bounds on the expressive power of various transformer architectures, which in turn are used to categorize which reasoning problems a language model can or cannot solve.
% For instance, \citet{merrill2023parallelism} shows that many transformer architectures are upper bounded by the uniform \(\msf{TC}^0\) circuit class, which means that, under standard complexity-theoretic assumptions, they cannot solve problems that require polynomial time unless other assumptions are made.


%%%%%

Results from computational complexity give crucial insight into the theoretical expressive power of language models, but much remains to be explored on the practical side.
A particular model architecture may have the potential to solve some problem, but does it actually learn the ``correct solution'' from its training data?
There exist emergent works that study how language models learn \red{(CITE)}, but definitive and comprehensive answers remain elusive because it is challenging to analyze the learned parameters of all but the simplest neural networks.
As such, there exists interest in studying how \emph{simple models} can learn to solve \emph{simple problems}.
In this work, we study the reasoning power of language models for propositional Horn logic, a mathematical logic wherein rules take the form ``\emph{if \(P\) and \(Q\), then \(R\)}'' for some propositions \(P\), \(Q\), and \(R\)~\citep{levesque1986knowledge}.


Propositional Horn logic is a \emph{simple problem} with broad applications~\citep{chen2020review}.
For instance, this logic can naturally express dependencies, which we illustrate in Figure~\ref{fig:mc_inference} (left) using an example from the Minecraft video game~\citep{mojang2011minecraft}.
In Minecraft, a common objective is to make new items according to a recipe list.
Given some starting items (\(\msf{Sheep}, \msf{Wool}\)), a player may ask whether they have sufficient material to craft some target item (\(\msf{FishingRod}\) if they follow a known recipe list (``If I can get \(\msf{Sheep}\), then I can get \(\msf{Wool}\)'', etc.).
Although this example appears toy, it is a non-trivial learning problem.
The rules, facts, and goals are supplied in-context, and the language model must learn which ones how to reason over these from training data alone.


\input{figures/mc_inference}


Importantly, we show that \emph{simple models} can solve propositional Horn reasoning via chain-of-thought (CoT) reasoning~\citep{wei2022chain,kojima2022large}.
In this paradigm, a language model's intermediate reasoning steps are generated step-by-step in an autoregressive loop until some stopping condition is reached.
% This is typically done using an autoregressive loop: at each iteration, the model's output is used as part of its input prompt for the next iteration, which continues until some stopping condition is reached.
Figure~\ref{fig:mc_inference} (right) shows an example of CoT reasoning wherein the model is first prompted with the rules, facts, and goal.
The model might first deduce from the given facts that \(\msf{Sheep}\) and \(\msf{Wood}\) are obtainable (State 0).
Using the previously deduced information, the model may then reason that \(\msf{Wool}\) is obtainable from \(\msf{Sheep}\) and that \(\msf{Stick}\) is obtainable from \(\msf{Wood}\) (State 1).
At the next iteration, the model may derive \(\msf{String}\) from \(\msf{Wool}\) (State 2), before finally concluding that it can obtain \(\msf{FishingRod}\) from \(\msf{Stick}\) and \(\msf{String}\) (State 3).
Because \(\msf{FishingRod}\) was the given goal, the stopping condition is reached.


% ~\citep{merrill2023expressive}

In this paper, we give a simple transformer construction that can encode autoregressive propositional inference using only one layer, one self-attention head, and embedding dimension linear in the number of propositions.
Our experiments show that models subject to our theoretical bounds can, in fact, attain high accuracy (\(99.9\%+\)).
Unfortunately, our learned models are not out-of-distribution robust.
In fact, it is possible to predictably jailbreak both our theoretical and learned models to produce fallacious outputs.
However, the simplicity of our construction also means that it is tractable to inspect the parameters of learned models.
We observe that the attention patterns of our learned parameters do not conform to our theoretical expectations.
If we \emph{further} simplify our construction, however, we observe cases where the learned weights reflect the theoretical construction.

This work provides an investigation into how language models can learn to reason on propositional Horn logic.
Crucially, this is a setting in which a simple problem can be solved by simple models, which makes it an important stepping stone for future works that investigate the learning of language models.
In summary, our contributions are as follows.



% \red{AAAAAAAAAAAAAAAAAAAA}


% We give an explicit transformer construction that encodes \emph{autoregressive propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
% Although our theoretical construction exactly encodes reasoning, one can provably force mistakes with a well-crafted adversarial attack~\cite{zou2023universal}.
% Motivated by this, we find that empirically learned models with seemingly perfect accuracy are also prone to similar attacks.
% This work demonstrates the simultaneous strength and weakness of language models that reason: although transformers can learn to reason over propositional Horn logic in both theory and practice, they are not far from logical fallacies.
% In summary, our contributions are as follows.





% \red{AAAAAAAAAAAAAAAAAAAAAAAAA}






% Logical reasoning is concerned with checking the truthfulness of asserted statements.
% Given such an assertion, also called the \emph{goal}, a standard reasoning problem asks the following: \emph{is this \textbf{goal} the logical consequence of the known \textbf{facts} and inference \textbf{rules}?}
% We illustrate this in Figure~\ref{fig:mc_reasoning} using an example from the Minecraft video game~\cite{mojang2011minecraft}.
% In Minecraft, a common objective is to make new items according to a recipe list.
% Given some starting items (\(\msf{Sheep}\), \(\msf{Wood}\)), a player may ask whether they have sufficient material to craft some target item (\(\msf{FishingRod}\)) if they follow the recipe list (``If I can get \(\msf{Sheep}\), then I can get \(\msf{Wool}\)'', etc.).
% Although the example of Figure~\ref{fig:mc_reasoning} appears toy, it is a non-trivial challenge for machine learning --- the model must first learn the rules and then figure out which ones to apply.
% In addition, this example is of practical interest because it is representative of a large class of reasoning problems~\cite{chen2020review}.
% In this paper, we present mathematical results for the reasoning power of language models on such problems, where the rules and facts are given in-context.





% An influential line of work examines the power of language models through the perspective of computational complexity~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}.
% Although computational complexity has deep connections to mathematical logics~\cite{borger2001classical}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
% Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.
% In this paper, we study the task of logical reasoning in propositional Horn logic using transformer-based language models.
% Propositional Horn logic is a fragment of
% propositional logic wherein the rules have the form \emph{``if \(P\) and \(Q\), then \(R\)''}, for some propositions \(P\), \(Q\) and \(R\)~\cite{levesque1986knowledge}.
% This logic captures a large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.

% ~\cite{levesque1986knowledge,chandra1985horn}


% An influential line of work examines the power of language models through the perspective of formal language theory~\cite{hao2022formal,merrill2023expressive,strobl2023transformers}, in which a typical result states the following:
% \emph{a transformer with some choice of parameter weights, attention mechanism, etc., can (or cannot) answer whether the input sequence belongs to some formal language (e.g., \textsc{Parity}, \textsc{Dyck-\(k\))}}.
% Although formal language membership has deep connections to mathematical logics~\cite{borger2001classical,bradley2007calculus}, it is often unclear how such results translate into insights about language models trained for reasoning tasks.
% Moreover, while there is much interest in understanding how and what such models might reason about, most existing works focus on empirical investigations~\cite{chu2023survey}.
% In this paper, we study the task of logical reasoning in propositional Horn logic using transformer-based language models.
% Propositional Horn logic is a fragment of
% propositional logic wherein the rules have the form \emph{``if this, then that''}~\cite{levesque1986knowledge,chandra1985horn}.
% This logic captures a simple yet large class of reasoning tasks~\cite{chen2020review} and serves as a key stepping stone to theoretically understanding learned reasoning in more complex logics.


% We give an explicit transformer construction that encodes \emph{autoregressive propositional inference}, the main computational mechanism of CoT reasoning in propositional Horn logic.
% Although our theoretical construction exactly encodes reasoning, one can provably force mistakes with a well-crafted adversarial attack~\cite{zou2023universal}.
% Motivated by this, we find that empirically learned models with seemingly perfect accuracy are also prone to similar attacks.
% This work demonstrates the simultaneous strength and weakness of language models that reason: although transformers can learn to reason over propositional Horn logic in both theory and practice, they are not far from logical fallacies.
% In summary, our contributions are as follows.




% We give an explicit transformer construction that encodes a decision circuit for autoregressive \emph{propositional inference}, the primary computational mechanism of CoT reasoning in propositional Horn logic.
% Importantly, our construction uses only two layers, one attention head, and an embedding dimension linear in the number of propositions.
% Empirically, we show that language models, subject to our theory, can learn autoregressive propositional inference with over \(99\%+\) accuracy.
% Moreover, we find that \textbf{increasing the embedding dimension and the number of layers improves accuracy} but increasing the number of attention heads does not.


% Furthermore, we investigate how even highly accurate language models may be forced to error.
% Our findings suggest a fundamental weakness of such models against even simple \emph{jailbreak attacks}~\cite{chao2023jailbreaking,zou2023universal}.
% First, we prove that even our theoretical construction of a perfect reasoner can be easily attacked.
% Moreover, we empirically show that learned models, even those with high accuracy, remain susceptible to out-of-distribution inputs and simple adversarial attacks.
% Both theoretically and experimentally, we find that it is easy to force language models to err.
% In summary, our contributions are as follows.



% \emph{jailbreak attacks}~\cite{chao2023jailbreaking,jones2023automatically,wei2023jailbroken,zou2023universal}.


\paragraph{Transformers Can Efficiently Encode Propositional Inference}
We give an encoding using only one layer, one self-attention head, and an embedding dimension linear in the number of propositions.
Empirically, we find that transformers subject to our theoretical size bounds can attain high accuracy (\(99.9\%+\)) on reasoning tasks.
The primary benefit of our construction is its compactness, which makes it tractable to directly study the weights of a learned model.


\paragraph{Learned Reasoning is not Robust}
Despite achieving high accuracy on the training data, we find that our learned models are not out-of-distribution robust.
We find that it is easy to construct and learn adversarial attacks against our learned models.



% \paragraph{Simplified Models Can Learn the Theoretical Solution!}




==> old/introduction_7.tex <==
\section{Introduction}
\label{sec:introduction}

% ~\citep{huang2022towards}

% ~\citep{zheng2024prompt}

Modern transformer-based language models~\citep{vaswani2017attention} can attain impressive performance on many reasoning benchmarks~\citep{chu2023survey,zhao2023survey}.
The ability to mimic reasoning is important for practical adoptions, especially in high-stakes applications like law and healthcare: the model's reasoning functions as ``proof'' that its decision should be trusted.
Although reasoning tasks span many flavors that include basic arithmetic~\citep{imani2023mathprompter,chen2022program}, commonsense reasoning~\citep{madaan2022language}, symbolic logics~\citep{cheng2022binding,zhao2023enhancing}, and others, they are broadly unified under the following format:

\begin{quote}
    \textbf{Reasoning Task:}
    is the assertion logically entailed by the given facts and rules?
    
    % is the goal \(\Omega\) logically entailed by the facts \(\Phi\) and rules \(\Gamma\)?
    % does the goal \(\tau\) logically follow from the 
    % is the goal \(\tau\) deducible from the known facts \(\Phi\) and the inference rules \(\Gamma\)?
\end{quote}

For instance, one may ask whether ``it is cloudy'' is deducible from the fact ``it is raining'' and the rule ``if it is raining, then it is cloudy'' --- which may be formulated as the input prompt:
\emph{``If it is raining, then it is cloudy. It is raining. Is it cloudy?''}

% \begin{myquote}
% \begin{prompt}
% Prompt: If it is raining, then it is cloudy. It is raining. Is it cloudy?

% Language Model: Yes, according to the given premise "If it is raining, then
% it is cloudy" and the fact that "It is raining," we can deduce that it
% must also be cloudy. So, yes, it is cloudy.
% \end{prompt}
% \end{myquote}


But when might such models fail to reason soundly, and can they be tricked into logical fallacies?
It is known that large language models suffer from many weaknesses and can be tricked into generating incorrect or undesirable outputs.
Although various measures against such behaviors are proposed in the literature, most known defenses are eventually broken --- often with a carefully crafted prompt.
If a language model is consulted to help with critical decision-making, then a subtle and well-crafted reasoning attack has the potential for serious harm: a human user may commit consequential mistakes based on intentionally bad advice.
To study such behaviors, we therefore study \emph{attacks on the logical reasoning of language models}.




To the best of our knowledge, the problem of attacking language model reasoning is not well-studied.
Although language models' reasoning power and attack strategies are of much interest, works that jointly study the two are sparse.
Nevertheless, useful connections in existing literature do exist.
For instance, it is common to use measures like alignment training~\citep{ouyang2022training,bai2022constitutional}, safety prompts~\citep{achiam2023gpt,zheng2024prompt}, and others~\citep{zou2023universal} in order to safeguard models from generating objectionable content.
The objective of the reasoning attack, then, is to bypass such restrictions.
However, a common theme in literature is the opaque nature of large language models, which makes it hard to thoroughly study their reasoning capabilities and vulnerabilities.



In order to tractably study attacks on language model reasoning, we focus on propositional Horn logic~\citep{levesque1986knowledge}.
This is a simple mathematical logic wherein rules have the form ``\emph{if \(P\) and \(Q\), then \(R\)}'' for some propositions \(P\), \(Q\), and \(R\).
Our choice is due to its balance of simplicity and usefulness: existing language models have the sufficient theoretical capacity to exactly reason over the ``if-then'' structure of these rules~\citep{strobl2023transformers}; at the same time, such rules have the expressive power to model interesting problems in dependency relations, logic programming~\cite{warren1977prolog}, and other domains~\citep{chen2020review}.
Importantly, propositional Horn logic allows us to tractably study the theoretical behavior of attacks.


% \red{(Existing works)}
While it is known that transformer-based language models are theoretically capable of encoding propositional Horn reasoning~\citep{zhang2022paradox,strobl2023transformers}, various limitations are observed in practice.
For instance, the authors of~\citep{zhang2022paradox} observe that learned reasoners, in particular BERT~\citep{devlin2018bert}, are not out-of-distribution robust: the language model attains high accuracy on its training distribution, but performs poorly when the test distribution is different.
\red{(More references should go here)}.
Our contribution is to study how language models may be tricked into logical fallacies during propositional Horn reasoning.




\input{figures/results_overview}

% (Our approach)
Our approach is summarized in Figure~\ref{fig:results_overview}, and expanded upon in the following.
In order to effectively study reasoning attacks, we first propose a small language model, \(\mcal{R}_{\msf{theory}}\), that can encode propositional Horn reasoning using only one layer, one head, and embedding dimension \(d = 2n\), where \(n\) is the number of propositions (e.g., ``it is raining'', ``it is cloudy'', etc.).
Although related constructions exist in literature~\citep{zhang2022paradox}, the primary benefit of this ``exact reasoner'' lies in its size and simplicity, which allows us to explicitly study all of its model parameters.
Using \(\mcal{R}_{\msf{theory}}\), we derive provably successful reasoning attacks that lead to logical fallacies.
In particular, we consider three types of attacks: whether we can coerce the model to logically conclude any specified target, whether we can make the model ignore one of the in-context rules, and whether we can make the model forget some previously derived knowledge.
Interestingly, we see that such theory-inspired attacks also work on small learned reasoners \(\mcal{R}_{\msf{learned}}\) that would otherwise attain high reasoning accuracy.
Furthermore, we observe that the strategies and insights from theory-inspired attacks are also reflected in successful attacks against larger natural language models, \(\mcal{R}_{\msf{LLM}}\).


Our work suggests that theoretical insights for reasoning attacks on small theoretical models translate to large language models.
As such, it may be fruitful to study the reasoning power of large language models by means of smaller models.
In summary, our contributions are as follows:


\paragraph{Small Transformers Can Encode and Learn Propositional Horn Reasoning}
We construct a small language model, \(\mcal{R}_{\msf{theory}}\), that implements chain-of-thought propositional Horn inference using only one layer, one self-attention head, and embedding dimension \(d = 2n\), where \(n\) is the number of propositions.
To demonstrate feasibility, we show that learned reasoners \(\mcal{R}_{\msf{learned}}\) subject to these bounds can also consistently attain high reasoning accuracy.


\paragraph{Theory-Inspired Attacks Work on Learned Models}
We devise reasoning attacks against \(\mcal{R}_{\msf{theory}}\) and show that such attacks also work against \(\mcal{R}_{\msf{learned}}\).
Moreover, adversarial language models trained to attack \(\mcal{R}_{\msf{learned}}\) also use similar strategies as those that we devised from theory: trained attacks can often rediscover ``tokens'' similar to our theory and also leverage similar strategies to exploit the attention mechanism.


\paragraph{Successful Attacks on Large Language Models Share Our Theory-Based Strategies}
By analyzing the attention pattern of large language models \(\mcal{R}_{\msf{LLM}}\) subject to attacks, we find that such attacks exploit the attention in a similar manner as those that we manually crafted against \(\mcal{R}_{\msf{theory}}\).
This suggests that studying the reasoning mechanics of small models may be a useful proxy for understanding the behavior of larger models.




==> old/layers_math.tex <==
\begin{figure*}[t]
\centering

\includegraphics[width=0.98\linewidth]{images/layers_math.png}

\caption{
A language model during one step of inference using rules \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and states \(s_0, \ldots, s_{t}\).
The action of \(\msf{Id} + \msf{Attn}\) is to approximate rule application with \(s_{t}\), where \(\varepsilon\) is some error term.
Next, the role of \(\msf{Id} + \msf{Ffwd}\) is to adjust this approximation into a binary vector.
Finally, we use \(\msf{ClsHead}\) to extract \(s_{t+1} = \Gamma(s_{t})\) from the last row of the embedded output sequence.
We assume vectors to be in column form and let \(\star\) denote miscellaneous entries omitted for brevity.
}
\label{fig:layers_math}
\end{figure*}



==> old/learned_models.tex <==

\section{How Good are Learned Models?}
\label{sec:robustness}

Although we have shown that shallow transformers can theoretically encode reasoning, how do they fare in practice?


\subsection{Learned Models Attain High Accuracy}

\input{figures/gpt2_grid}





\subsection{Learned Models are not Out-of-Distribution Robust}

\input{figures/not_ood_robust}




\red{AAAAAAAAAAAAAAAAAAAAAA}

% In this Section, we study the extent to which models fail to reason.
% In particular, we study how to elicit some desired response (\emph{adversarial target}) from a reasoner model by appending some malicious \emph{attack tokens} to its input sequence.
% We illustrate this mechanism in Figure~\ref{fig:attack}.

% \input{figures/attack}

% Although various forms of attacks exist~\cite{huang2023catastrophic}, we focus on suffix-based attacks~\cite{zou2023universal} due to their simplicity.
% The subject of our attacks is a language model~\eqref{eqn:lm} trained for reasoning, which we call \(\msf{Reasoner}\).
% Given some adversarial target \(s_{\msf{tgt}} \in \mbb{B}^n\), token sequence \(U \in \mbb{R}^{N \times d_{\msf{in}}}\), and \emph{attack budget} \(N_{\msf{atk}} > 0\), our attack problem is then expressed as the following search problem:
% \begin{align} \label{eqn:attack_problem}
% \begin{split}
%     \text{find} \enskip U_{\msf{atk}} \in \mbb{R}^{N_{\msf{atk}} \times d_{\msf{in}}},
%     \qquad 
%     \text{subject to}
%         &\enskip s_{\msf{tgt}} = \msf{Reasoner}(\msf{append}(U, U_{\msf{atk}}))
% \end{split}
% \end{align}
% We first consider attacks against our theoretical construction of a perfect \(\msf{Reasoner}\) in Section~\ref{sec:theory_attacks}.
% Then, in Section~\ref{sec:learned_attacks}, we consider the problem of training a language model to attack a learned \(\msf{Reasoner}\).


% \subsection{Perfect Reasoners are Easily Attacked}
% \label{sec:theory_attacks}

% We first consider attacks against our theoretical construction of \(\msf{Reasoner}\) as in Section~\ref{sec:theory_overview}.
% In particular, we find that \emph{a single suffix token suffices} to attack a perfect reasoner.
% Moreover, we sketch this result below.

% \begin{theorem}[Sketch of Attack Result]
% \label{thm:attack_result_sketch}
% Consider any \(\msf{Reasoner}\) language model as given in Section~\ref{sec:theory_overview}, token sequence \(U\), and adversarial target label \(s_{\msf{tgt}} \in \mbb{B}^n\), then for sufficiently large \(\kappa > 0\) we have:
% \begin{align*}
%     s_{\msf{tgt}} = \msf{Reasoner}(\msf{append}(U, u_{\msf{atk}}))
% \end{align*}
% with attack token \(u_{\msf{atk}} = (\mbf{0}_n, s_{\msf{tgt}} - \kappa (\mbf{1}_n - s_{\msf{tgt}}))
%     \in \mbb{R}^{2n}\).
% \end{theorem}

% We present a proof in Appendix~\ref{sec:theory_attack}.
% This result implies that our theoretical construction is still susceptible to attacks despite being a perfect reasoner.
% In particular, the attack token is independent of the input \(U\) but is dependent on constants used in the theoretical constructions in Appendix~\ref{sec:theory_construction}.
% Intuitively, this attack over-saturates the softmax attention mechanism with a large input.


% \subsection{Training a Language Model for Attack}
% \label{sec:learned_attacks}

% We now show how a language model can be trained to attack \(\msf{Reasoner}\).
% This attacking model, which we call \(\msf{Attacker}\), is to behave similarly to Figure~\ref{fig:attack} and has the same language model architecture as described in~\eqref{eqn:lm}.
% For consistency, we remark that one must appropriately tokenize and append the adversarial target label \(s_{\msf{tgt}}\) with the token sequence \(U\).
% Let \(\theta\) be the parameters of \(\msf{Attacker}\) and suppose that \(\mcal{D}\) is the training distribution of \(\msf{Reasoner}\).
% We then express the \(\msf{Attacker}\) training as the following optimization problem:

% \begin{align} \label{eqn:attacker_training_problem}
% \begin{split}
%     \underset{\theta}{\text{minimize}}
%         &\quad \expval{U \sim \mcal{D}}\, \mcal{L}(\hat{s}, s_{\msf{tgt}}; \theta) \\
%     \text{where}
%         &\quad u_{\msf{atk}} = \msf{Attacker}(s_{\msf{tgt}}, U; \theta) \\
%         &\quad \hat{s} = \msf{Reasoner}(\msf{append}(U, u_{\msf{atk}}))
%     \end{split}
% \end{align}
% We emphasize that we are training only \(\msf{Attacker}\) and that \(\msf{Reasoner}\) is fixed.
% We have left the loss function \(\mcal{L}\) under-specified for flexibility, but in our experiments of Section~\ref{sec:experiments_learned_attackers}, we use binary cross-entropy loss, which is the same objective used to train \(\msf{Reasoner}\).





==> old/old_attack.tex <==
\subsection{Results for adversarial attacks}
\label{sec:theory_attack}

\begin{theorem}[Adversarial attack]
\label{thm:adv_attack}
Take the definitions as in Theorem~\ref{thm:reasoning} and pick \(\mu \geq r + t + 1\).
Fix any \(s_{\msf{tgt}} \in \mbb{B}^n\) and \(\kappa > \mu^2\), and let \(\alpha_{N+1} = \mbf{0}_n\) and \(\beta_{N+1} = s_{\msf{tgt}} - \kappa (\mbf{1}_n - s_{\msf{tgt}})\).
Then, we have:
\begin{align*}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \alpha_{N+1} ^\top & \beta_{N+1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Transformer}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \star \\
        1 & \alpha_{N+1} ^\top & s_{\msf{tgt}} ^\top
    \end{bmatrix}
\end{align*}
\end{theorem}
\begin{proof}
We take a similar approach as in Theorem~\ref{thm:reasoning}, and likewise expand the attention component as follows:
\begin{align*}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \alpha_{N+1} ^\top & \beta_{N+1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \alpha_{N+1} ^\top & \beta_{N+1} ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \frac{\mu}{\abs{i: \alpha_i \preceq \beta_{N+1}}} \sum_{i: \alpha_i \preceq \beta_{N+1}} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \varepsilon^\top
    \end{bmatrix}
    \tag{Lemma~\ref{lem:reasoning_softmax} using sequence length \(N+1\) instead of \(N\)}
\end{align*}
where \(\norm{\varepsilon}_\infty < 1/3\).

\end{proof}


% \begin{theorem}[Adversarial Attack]
% \label{thm:adv_attack}
% Take the definitions as in Theorem~\ref{thm:reasoning} and pick \(\mu \geq r + t + 1\).
% Fix any \(s_{\msf{tgt}} \in \mbb{B}^n\) and \(\kappa > \mu^2\), and define \(\psi_{\msf{atk}} = s_{\msf{tgt}} - \kappa (\mbf{1}_n -  s_{\msf{tgt}})\).
% Then, for \(\msf{LM}\) as defined in~\eqref{eqn:appendix_lm}, we have:
% \begin{align*}
%     \begin{bmatrix}
%         \alpha_1 ^\top & \beta_1 ^\top \\
%         \vdots & \vdots \\
%         \alpha_r ^\top & \beta_r ^ \top \\
%         \mbf{0}_n ^\top & s_0 ^\top \\
%         \vdots & \vdots \\
%         \mbf{0}_n ^\top & s_{t-1} ^\top \\
%         \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top
%     \end{bmatrix}
%     \xrightarrow{\msf{Embed}}
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \beta_1 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \beta_r ^\top \\
%         1 & \mbf{0}_n ^\top & s_0 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & s_{t-1} ^\top \\
%         1 & \mbf{0}_n ^\top & \psi_{\msf{atk}} ^\top
%     \end{bmatrix}
%     \xrightarrow{\msf{Transformer}}
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \star \\
%         1 & \mbf{0}_n ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & \star \\
%         0 & \mbf{0}_n ^\top & s_{\msf{tgt}} ^\top
%     \end{bmatrix}
%     \xrightarrow{\msf{ClsHead}}
%     s_{\msf{tgt}}
% \end{align*}
% \end{theorem}
% \begin{proof}
% Because \(\msf{Embed}\) only prepends a leading bit to each row of its input and \(\msf{ClsHead}\) is a linear projection from the last row, it suffices to only analyze the action of \(\msf{Transformer}\).
% Therefore, much of this proof will be similar in structure to that of Theorem~\ref{thm:reasoning}.
% To begin, let \(X \in \mbb{R}^{N \times d}\) be embedded input sequence and decompose \(\msf{Attn}(X)\) as follows:
% \begin{align} \label{eqn:attack_attn_decomp}
%     \msf{Attn}(X)
%     = \msf{CausalSoftmax}(\lambda X(\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a X^\top) X \mu \Pi_b ^\top \Pi_b
%     = \sum_{i = 1}^{N} \mu e_i \sigma_i ^\top X \Pi_b ^\top \Pi_b
% \end{align}
% where \(\sigma_1, \ldots, \sigma_N \in \mbb{R}^{N}\) are the rows of \(\msf{CausalSoftmax}(\ldots)\), except \(\sigma_N\) is now:
% \begin{align}
%     \sigma_N
%         &= \msf{Softmax}(\lambda x_N ^\top (\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a x_1),
%             \ldots,
%             \lambda x_N ^\top (\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a x_N) \nonumber \\
%         &= \msf{Softmax}(\lambda (\psi_{\msf{atk}} - \mbf{1}_n)^\top \alpha_1, \ldots, \lambda (\psi_{\msf{atk}} - \mbf{1}_n)^\top \alpha_N) \tag{\(\alpha_i = \Pi_a x_i\) with \(\alpha_i = \mbf{0}_n\) for \(i \geq r + 1\)} \\
%         &= \msf{Softmax}(\lambda z_1, \ldots, \lambda_N z_N)
%     \label{eqn:attack_sigmaN_softmax}
% \end{align}
% In particular, each \(z_1, \ldots, z_N\) is such that:
% \begin{align*}
%     z_i = (\psi_{\msf{atk}} - \mbf{1})^\top \alpha_i
%         = s_{\msf{tgt}}^\top \alpha_i - \kappa (\mbf{1}_n - s_{\mbf{tgt}})^\top \alpha_i - \mbf{1}_n ^\top \alpha_i
% \end{align*}
% where \(s_{\msf{tgt}}^\top \alpha_i \leq 0\) and \((\mbf{1}_n - s_{\msf{tgt}})^\top \alpha_i \geq 0\) are both integers and \(\kappa > 1\) by assumption.
% We thus conclude that for each coordinate: either \(z_i = 0\) or \(z_i \leq -1\).
% Additionally, since \(z_N = 0\) and \(\lambda > 0\), we may then apply Lemma~\ref{lem:reasoning_softmax} on~\eqref{eqn:attack_sigmaN_softmax} to get:
% \begin{align} \label{eqn:attack_sigmaN_decomp}
%     \sigma_N = \frac{1}{c} \varphi + \varepsilon,
%     \qquad \norm{\varepsilon}_{\infty} \leq N e^{-\lambda} \leq \mu e^{-\lambda}
% \end{align}
% for some \(1 \leq c \leq N\) and \(\varphi \in \mbb{B}^N\) with \(\varphi_N = 1\).
% We use this form of \(\sigma_N\) in~\eqref{eqn:attack_sigmaN_decomp} to rewrite the \(N\)th term of~\eqref{eqn:attack_attn_decomp} as:
% \begin{align}
%     \mu e_N \sigma_N ^\top X \Pi_b ^\top \Pi_b
%         &= \frac{\mu}{c} e_N \varphi^\top X \Pi_b ^\top \Pi_b + \mu e_N \varepsilon^\top X \Pi_b ^\top \Pi_b \nonumber \\
%         &= \frac{\mu}{c} e_N \sum_{j = 1}^{N} \varphi_j x_j ^\top \Pi_b ^\top \Pi_b
%         + \mu e_N \varepsilon^\top X \Pi_b ^\top \Pi_b \nonumber \\
%         &= \frac{\mu}{c} e_N x_N ^\top \Pi_b ^\top \Pi_b
%         + \frac{\mu}{c} e_N \sum_{j = 1}^{N-1} \varphi_j x_j ^\top \Pi_b ^\top \Pi_b
%         + \mu e_N \varepsilon^\top X \Pi_b ^\top \Pi_b
%         \tag{\(\varphi_N = 1\)} \nonumber \\
%         &= \frac{\mu}{c} e_N \psi_{\msf{atk}} ^\top \Pi_b
%         + e_N \underbrace{\parens*{
%                 \frac{\mu}{c} \sum_{j = 1}^{N-1} \varphi_j x_j ^\top \Pi_b^\top
%             }}_{\omega^\top} \Pi_b
%         + e_N \underbrace{\parens*{
%             \mu \varepsilon^\top X \Pi_b ^\top \Pi_b
%             }}_{\zeta^\top} \Pi_b
%         \label{eqn:attack_omega_zeta}
% \end{align}
% which we then substitute back into~\eqref{eqn:attack_attn_decomp} to form:
% \begin{align*}
%     \msf{Attn}(X)
%     = \frac{\mu}{c} e_N \psi_{\msf{atk}} ^\top \Pi_b
%         + e_N \omega^\top \Pi_b
%         + e_N \zeta^\top \Pi_b
%         + \sum_{i = 1}^{N-1} \mu_i e_i \sigma_i ^\top \Pi_b ^\top \Pi_b
% \end{align*}
% which means that
% \begin{align} \label{eqn:attack_idattn}
%     X =
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \beta_1 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \beta_r ^\top \\
%         1 & \mbf{0}_n ^\top & s_0 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & s_{t-1} ^\top \\
%         1 & \mbf{0}_n ^\top & \psi_{\msf{atk}} ^\top
%     \end{bmatrix}
%     \xrightarrow{\msf{Id} + \msf{Attn}}
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \star \\
%         1 & \mbf{0}_n ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & \star \\
%         1 & \mbf{0}_n ^\top
%         & (\psi_{\msf{atk}} + (\mu/c) \psi_{\msf{atk}} + \omega + \zeta)^\top
%     \end{bmatrix}
% \end{align}
% where \(\star\) denotes miscellaneous entries of the appropriate dimensions.
% Similar to Theorem~\ref{thm:reasoning}, we next analyze the last row of the~\eqref{eqn:attack_idattn} RHS.
% In particular, because \(\varphi \in \mbb{B}^n\) and each \(x_1, \ldots, x_{N-1} \in \mbb{B}^d\), we may bound each entry of \(\omega \in \mbb{R}^{n}\) as:
% \begin{align*}
%     0 \leq \omega_i
%     \leq (\mu/c) \sum_{j = 1}^{N-1} \underbrace{\norm{\varphi_j \Pi_b x_j}_\infty}_{\leq 1}
%     \leq (\mu/c) (N-1) \leq \mu^2
% \end{align*}
% where recall that \(\mu / c \geq 1\).
% Next, we bound the \(\zeta\) term as:
% \begin{align*}
%     \norm{\zeta}_\infty
%     = \norm{\mu \Pi_b X^\top \varepsilon}_\infty
%     \leq \mu \norm{\mbf{1}_N \mbf{1}_N ^\top \varepsilon}_\infty
%     \leq \mu N \norm{\varepsilon}_\infty
%     \leq \mu ^3 e ^{-\lambda}
%     < \delta
%     \tag{\(\norm{\varepsilon}_\infty \leq \mu e^{-\lambda}\) by~\eqref{eqn:attack_sigmaN_decomp}}
% \end{align*}
% Then, because \(\kappa > \mu^2\), we have the following inequalities:
% \begin{align*}
%     (\psi_{\msf{atk}} + (\mu/c) \psi_{\msf{atk}} + \omega + \zeta)_i
%     \quad \begin{dcases}
%         (1 + \mu/c) + \omega_i + \zeta_i
%         > 1, & \text{when} \enskip (s_{\msf{tgt}})_i = 1 \\
%         -\kappa (1 + \mu/c) + \omega_i + \zeta_i
%         < 0, & \text{when} \enskip (s_{\msf{tgt}})_i = 0
%     \end{dcases}
% \end{align*}
% for all \(i = 1, \ldots, n\).
% We thus have for the last row of the~\eqref{eqn:attack_idattn} RHS that:
% \begin{align} \label{eqn:attack_idffwd}
%     \begin{bmatrix}
%         1 \\
%         \mbf{0}_n \\
%         \psi_{\msf{atk}} + (\mu/c) \psi_{\msf{atk}} + \omega + \zeta
%     \end{bmatrix}
%     \xrightarrow{\msf{Id} + \msf{Ffwd}}
%     \begin{bmatrix}
%         1 \\ \mbf{0}_n \\ s_{\msf{tgt}}
%     \end{bmatrix}
% \end{align}
% Lastly, we compose \(\msf{Id} + \msf{Attn}\) with \(\msf{Id} + \msf{Ffwd}\) to yield:
% \begin{align*}
%     X =
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \beta_1 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \beta_r ^\top \\
%         1 & \mbf{0}_n ^\top & s_0 ^\top \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & s_{t-1} ^\top \\
%         1 & \mbf{0}_n ^\top & \psi_{\msf{atk}} ^\top
%     \end{bmatrix}
%     \xrightarrow[\eqref{eqn:attack_idattn}]{\msf{Id} + \msf{Attn}}
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \star \\
%         1 & \mbf{0}_n ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & \star \\
%         1 & \mbf{0}_n ^\top
%         & (\psi_{\msf{atk}} + (\mu/c) \psi_{\msf{atk}} + \zeta)^\top
%     \end{bmatrix}
%     \xrightarrow[\eqref{eqn:attack_idffwd}]{\msf{Id} + \msf{Ffwd}}
%     \begin{bmatrix}
%         1 & \alpha_1 ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \alpha_r ^\top & \star \\
%         1 & \mbf{0}_n ^\top & \star \\
%         \vdots & \vdots & \vdots \\
%         1 & \mbf{0}_n ^\top & \star \\
%         1 & \mbf{0}_n ^\top & s_{\msf{tgt}}^\top
%     \end{bmatrix}
% \end{align*}

% \end{proof}



==> old/old_figures/attacks_acc.tex <==

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\begin{table}[ht]
    \ra{1.3}
    \centering
    \small

    \vspace{0.1in}
\begin{tabular}{@{}cccc@{}}
\toprule
\#propositions & \multicolumn{3}{c}{embedding dimension} \\
\cmidrule{2-4}
        \(n\)            & \(d = 32\) & \(d = 64\) & \(d = 128\)   \\
\midrule
         16 &           1.00 &            1.00 &            1.00 \\
         32 &          - &            1.00 &            1.00 \\
         48 &          - &           - &            1.00 \\
         %  8 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         % 16 & \(0.92 \pm 0.11\)  & \(0.69 \pm 0.21\)  & \(1.00 \pm 0.00\) \\
         % 24 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(0.70 \pm 0.43\) \\
         % 32 & -  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         % 40 & - & - & \(0.94 \pm 0.09\) \\
\bottomrule
\end{tabular}
\caption{Unbounded single token attack on one-step reasoning}
% \caption{
% Language models can successfully attack other language models.
% We fine-tune base GPT-2 \((d=768, L=12, H=12)\) as our attacker against different reasoners that attain near-perfect accuracy on the one-step reasoning task.
% The attacker objective is: given an adversarial target \(s_{\msf{tgt}}\) and an input sequence \(U\), append a token to \(U\) that makes the reasoner output \(s_{\msf{tgt}}\).
% We do not attack non-perfect reasoners (c.f. Figure~\ref{fig:q1}).
% % Transformers trained to attack perfect learners demonstrate high success rates. The values \(x \pm y\) denote the mean accuracy (and standard deviation across three runs) of the learner generating the random adversarial output when the original input is concatenated with the attack vector generated by the attack model (as in Theorem~\ref{thm:attack_result_sketch}). The empty entries indicate imperfect reasoners that were not attacked.
% }
\label{tab:learned_attack_results}
%\vspace{0.1in}
\end{table}

\begin{table}[ht]
    \ra{1.3}
    \centering
    \small

    \vspace{0.1in}
\begin{tabular}{@{}cccc@{}}
\toprule
\#propositions & \multicolumn{3}{c}{embedding dimension} \\
\cmidrule{2-4}
        \(n\)            & \(d = 32\) & \(d = 64\) & \(d = 128\)   \\
\midrule
         16 &           1.00 &            1.00 &            1.00 \\
         32 &          - &            1.00 &            1.00 \\
         48 &          - &           - &            1.00 \\
         %  8 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         % 16 & \(0.92 \pm 0.11\)  & \(0.69 \pm 0.21\)  & \(1.00 \pm 0.00\) \\
         % 24 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(0.70 \pm 0.43\) \\
         % 32 & -  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         % 40 & - & - & \(0.94 \pm 0.09\) \\
\bottomrule
\end{tabular}
\caption{0-1 clamped three token attack on one-step reasoning}
% \caption{
% Language models can successfully attack other language models.
% We fine-tune base GPT-2 \((d=768, L=12, H=12)\) as our attacker against different reasoners that attain near-perfect accuracy on the one-step reasoning task.
% The attacker objective is: given an adversarial target \(s_{\msf{tgt}}\) and an input sequence \(U\), append a token to \(U\) that makes the reasoner output \(s_{\msf{tgt}}\).
% We do not attack non-perfect reasoners (c.f. Figure~\ref{fig:q1}).
% % Transformers trained to attack perfect learners demonstrate high success rates. The values \(x \pm y\) denote the mean accuracy (and standard deviation across three runs) of the learner generating the random adversarial output when the original input is concatenated with the attack vector generated by the attack model (as in Theorem~\ref{thm:attack_result_sketch}). The empty entries indicate imperfect reasoners that were not attacked.
% }
\label{tab:learned_attack_results_clamped}
%\vspace{0.1in}
\end{table}

==> old/old_figures/autoreg.tex <==
\begin{figure*}[t]
\centering


\includegraphics[width=0.95\linewidth]{images/autoreg.png}

\caption{
The various components of a language model (\(\msf{Embed}\), \(\msf{Transformer}\), and \(\msf{ClsHead}\)) during autoregressive propositional inference.
After the new state \(s_t\) is derived, its tokenization \((\mbf{0}_n, s_t)\) is appended to the input sequence.
}
\label{fig:autoreg}
\end{figure*}



==> old/old_figures/gpt2_grid.tex <==
\begin{figure}[ht]
\centering



\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns1.png}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns2.png}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns3.png}
\end{minipage}%


\caption{
A reasoner needs embedding dimension linear in the problem size.
We fix \(L=1\) layers and \(H=1\) heads according to our theory and vary the embedding dimension \(d\) and the number of propositions \(n\).
Near-perfect accuracy (\(\geq 0.99\)) is attained when \(d \geq 4n\). The accuracies are rounded up to two decimal places.
}
\label{fig:gpt2_grid}
\end{figure}


==> old/old_figures/mc_inference.tex <==
\begin{figure*}[t]
\centering


\includegraphics[width=0.95\linewidth]{images/mc_inference.png}

\caption{
% A more detailed look at CoT reasoning from Figure~\ref{fig:mc_reasoning}.
Given the LHS reasoning task (rules, facts, and goal), the starting state is initialized with the facts.
The language model then iteratively derives new propositions (e.g., \(\msf{Wool}, \msf{Stick}\)) by simultaneously applying all possible rules until the goal (\(\msf{FishingRod}\)) is reached.
}
\label{fig:mc_inference}
\end{figure*}



==> old/old_figures/mc_reasoning.tex <==
\begin{figure}[t]
\centering


\includegraphics[width=0.98\linewidth]{images/mc_reasoning.png}

\caption{
A reasoning task adapted from Minecraft~\cite{mojang2011minecraft}.
Given a set of rules, a set of facts, and an asserted goal, the language model uses chain-of-thought reasoning to iteratively derive additional knowledge before reaching an answer.
}
\label{fig:mc_reasoning}
\end{figure}



==> old/old_figures/minecraft_acc.tex <==
\begin{table*}
    \ra{1.3}
    \centering
    \small

    \vspace{0.1in}
\begin{tabular}{@{}cccccc@{}}
\toprule
\#steps & \multicolumn{5}{c}{Maximum number of propositions} \\
\cmidrule{2-6}
        \( \)            & \(n < 16\) & \(n < 32\) & \(n < 48\) & \(n < 64\) & \(n < 80\)   \\
\midrule
           1 &              0.94 &              0.83 &              0.78 &              0.77 &              0.71 \\
           3 &              0.94 &              0.94 &              0.84 &              0.79 &              0.56 \\
\bottomrule
\end{tabular}
\caption{Single and tree-step CoT reasoning results on the Minecraft dataset. The accuracy here denotes the percentage of samples where the generation contains all propositions from the expected reasoning chain.}
% \caption{
% Language models can successfully attack other language models.
% We fine-tune base GPT-2 \((d=768, L=12, H=12)\) as our attacker against different reasoners that attain near-perfect accuracy on the one-step reasoning task.
% The attacker objective is: given an adversarial target \(s_{\msf{tgt}}\) and an input sequence \(U\), append a token to \(U\) that makes the reasoner output \(s_{\msf{tgt}}\).
% We do not attack non-perfect reasoners (c.f. Figure~\ref{fig:q1}).
% % Transformers trained to attack perfect learners demonstrate high success rates. The values \(x \pm y\) denote the mean accuracy (and standard deviation across three runs) of the learner generating the random adversarial output when the original input is concatenated with the attack vector generated by the attack model (as in Theorem~\ref{thm:attack_result_sketch}). The empty entries indicate imperfect reasoners that were not attacked.
% }
\label{tab:minecraft_results}
%\vspace{0.1in}
\end{table*}

==> old/old_figures/not_ood_robust.tex <==
\begin{figure}[ht]
\centering

\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp4/exp4_prob_plot.pdf}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/attention_patterns/gpt2_n16_d32_attn.png}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/attention_patterns/tfe_n16_d32_attn.png}
\end{minipage}%


\caption{
(Left) learned models are not out-of-distribution robust. Increasing the probability of \(p_\alpha\) and \(p_\beta\) makes models perform worse.
(Middle) A heatmap of \(W_Q W_K ^\top\) for a learned GPT-2 with \(n = 16\) and \(d = 32\).
This is not the theoretically predicted attention pattern.
(Right) The theoretically predicted attention pattern of \(W_Q W_K ^\top\).
}
\label{fig:not_ood_robust}
\end{figure}


==> old/old_figures/q2.tex <==
\begin{figure}[ht]
\centering

\includegraphics[width=0.95\linewidth]{images/exp_plots/exp2/exp_theory_comp_plot.pdf}

\caption{
Adversarial attacks designed for theoretical models partially translate to learned reasoners.
Appending a sufficiently large attack token \(u_{\msf{atk}}\) to two different input sequences causes even near-perfect reasoners to produce the same output.
This works by saturating the reasoner's softmax attention, where \(\kappa = \norm{u_{\msf{atk}}}_\infty\).
%Perfect learners can be attacked with high accuracy using adversarial inputs constructed as in Theorem~\ref{thm:attack_result_sketch}. Higher values of \(\kappa\) lead to stronger attacks. \(\kappa\) refers to the scaling constant in Theorem~\ref{thm:attack_result_sketch}. The Attack Accuracy refers to the accuracy of the learned model predicting the same output vector for two randomly drawn inputs that are manipulated as in Theorem~\ref{thm:attack_result_sketch}.
}
\label{fig:q2}
\end{figure}

==> old/old_figures/q2_additional.tex <==
\begin{figure}[ht]
\centering
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_d128.pdf}
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_d160.pdf}
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_d192.pdf}
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_128.pdf}
\end{minipage}%
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_160.pdf}
\end{minipage}
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp2_additional/exp_theory_comp_plot_192.pdf}
\end{minipage}
\caption{Adversarial attacks designed for theoretical models partially translate to learned reasoners.
Appending a sufficiently large attack token \(u_{\msf{atk}}\) to two different input sequences causes even near-perfect reasoners to produce the same output.
This works by saturating the reasoner's softmax attention, where \(\kappa = \norm{u_{\msf{atk}}}_\infty\).}
\label{fig:q2_additional}
\end{figure}

==> old/old_figures/q3.tex <==

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\begin{table}[ht]
    \ra{1.3}
    \centering
    \small

    \vspace{0.1in}
\begin{tabular}{@{}cccc@{}}
\toprule
\#propositions & \multicolumn{3}{c}{embedding dimension} \\
\cmidrule{2-4}
        \(n\)            & \(d = 96\) & \(d = 128\) & \(d = 160\)   \\
\midrule
          8 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         16 & \(0.92 \pm 0.11\)  & \(0.69 \pm 0.21\)  & \(1.00 \pm 0.00\) \\
         24 & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\)  & \(0.70 \pm 0.43\) \\
         32 & -  & \(1.00 \pm 0.00\)  & \(1.00 \pm 0.00\) \\
         40 & - & - & \(0.94 \pm 0.09\) \\
\bottomrule
\end{tabular}
\caption{
Language models can successfully attack other language models.
We fine-tune base GPT-2 \((d=768, L=12, H=12)\) as our attacker against different reasoners that attain near-perfect accuracy.
The attacker objective is: given an adversarial target \(s_{\msf{tgt}}\) and an input sequence \(U\), append a token to \(U\) that makes the reasoner output \(s_{\msf{tgt}}\).
We do not attack non-perfect reasoners (c.f. Figure~\ref{fig:q1}).
% Transformers trained to attack perfect learners demonstrate high success rates. The values \(x \pm y\) denote the mean accuracy (and standard deviation across three runs) of the learner generating the random adversarial output when the original input is concatenated with the attack vector generated by the attack model (as in Theorem~\ref{thm:attack_result_sketch}). The empty entries indicate imperfect reasoners that were not attacked.
}
\label{tab:learned_attack_results}
%\vspace{0.1in}
\end{table}


%%%%%%%%%%%%% Embed dim as columns, Number of variables as rows (wider)
% \begin{table*}[t]
%     \centering
%     \footnotesize
%      \caption{Learned attack results on perfect learners. The values \(x \pm y\) denote the mean accuracy (and standard deviation) of the learner generating the random adversarial output when the original input is concatenated with the attack vector generated by the attack model (as in Theorem~\ref{thm:adv_result_sketch}).}
%     \label{tab:learned_attack_results}
%     % \vspace{-0.1in}
%     % \setlength{\tabcolsep}{0.5em} 
% \begin{tabular}{c|ccccc}
% \toprule
%   Embedding dimension (\(d\))        & \multicolumn{5}{c}{Number of variables (\(n\))} \\\midrule
%                     & 8 & 16 & 32 & 40 & 48 \\\midrule
%  96 & \(1.0 \pm 0.0 \) & \(1.0 \pm 0.0 \) & \(0.99 \pm 0.0 \) & \(1.0 \pm 0.0 \) & \(0.64 \pm 0.0 \) \\
%  128 & 1.0 & 0.53 & 1.0 & 1.0 & 1.0 \\
%  160 & 1.0 & 1.0 & 0.1 & 0.99 & -1.0 \\
% \bottomrule
% \end{tabular}
% %\vspace{0.1in}
% \end{table*}

==> old/old_figures/q4.tex <==
% \begin{figure}[ht]
% \centering

% \includegraphics[width=0.95\columnwidth]{images/exp_plots/exp4/exp4_prob_plot.pdf}

% \caption{
% Perfect in-distribution learners fail to generalize when the rules have more hot bits.
% We take perfect reasoners trained on rules drawn from the green band (\(0.2 \leq p_\alpha, p_\beta \leq 0.3\)) and test them on rules with antecedent and consequent probabilities \(p_\alpha ^{\msf{test}} = p_\beta ^{\msf{test}} \in \{0.1, 0.2, \ldots, 0.9\}\).
% The reasoner accuracy decays when \(p^{\msf{test}} \gg 0.3\), but not when \(p^{\msf{test}} = 0.1\).
% % Perfect in-distribution learners fail to generalize to datasets where the probabilities of a proposition occurring in the antecedent / consequent (\(p_\alpha\, p_\beta\)) are higher than those used for training. The x-axis represents \(p_\alpha = p_\beta = k\) and the y-axis represents the test accuracy. Each line corresponds to a perfect learner from Figure~\ref{fig:q1}. The shaded region represents the in-distribution range (\(0.2 \leq p_\alpha = p_\beta \leq 0.3\)). 
% }
% \label{fig:q4_a}
% \end{figure}

% \begin{figure}[ht]
% \centering

% \includegraphics[width=0.95\columnwidth]{images/exp_plots/exp4/exp4_rules_plot.pdf}

% \caption{
% Perfect in-distribution reasoners fail to generalize when they see more rules than what they are trained on.
% We take perfect reasoners trained on some number of rules drawn from the green band (\(16 \leq r \leq 64\)) and test them on distributions with \(r^{\msf{test}} \in \{8, 128, 256, 512\}\) number of rules.
% For \(r^{\msf{test}} = 8\) we attain perfect accuracy, but not so for \(r^{\msf{test}} > 64\).
% }
% \label{fig:q4_b}
% \end{figure}

\begin{figure*}[ht]
\centering

\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=0.95\columnwidth]{images/exp_plots/exp4/exp4_prob_plot.pdf}
    \caption{
Near-perfect in-distribution learners fail to generalize when the rules have more hot bits.
We take near-perfect reasoners trained on rules drawn from the green band (\(0.2 \leq p_\alpha, p_\beta \leq 0.3\)) and test them on rules with antecedent and consequent probabilities \(p_\alpha ^{\msf{test}} = p_\beta ^{\msf{test}} \in \{0.1, 0.2, \ldots, 0.9\}\).
The reasoner accuracy decays when \(p^{\msf{test}} \gg 0.3\), but not when \(p^{\msf{test}} = 0.1\).
% Perfect in-distribution learners fail to generalize to datasets where the probabilities of a proposition occurring in the antecedent / consequent (\(p_\alpha\, p_\beta\)) are higher than those used for training. The x-axis represents \(p_\alpha = p_\beta = k\) and the y-axis represents the test accuracy. Each line corresponds to a perfect learner from Figure~\ref{fig:q1}. The shaded region represents the in-distribution range (\(0.2 \leq p_\alpha = p_\beta \leq 0.3\)). 
}
\label{fig:q4_a}
\end{minipage}%
\hfill
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=0.95\columnwidth]{images/exp_plots/exp4/exp4_rules_plot.pdf}
\caption{
Near-perfect in-distribution reasoners fail to generalize when there are more rules.
We take near-perfect reasoners trained on some number of rules drawn from the green band (\(16 \leq r \leq 64\)) and test them on distributions with \(r^{\msf{test}} \in \{8, 16, \ldots, 512\}\) number of rules.
For \(r^{\msf{test}} = 8\) we attain near-perfect accuracy, but not so for \(r^{\msf{test}} > 64\).
}
\label{fig:q4_b}
\end{minipage}
\end{figure*}

==> old/old_figures/q4_additional.tex <==
\begin{figure}[htb]
\centering

% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp4_additional/exp4_prob_plot_128.pdf}
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp4_additional/exp4_prob_plot_160.pdf}

\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_prob_plot_128.pdf}
\end{minipage}%
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_prob_plot_160.pdf}
\end{minipage}
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_prob_plot_192.pdf}
\end{minipage}
\caption{Near-perfect in-distribution learners fail to generalize when the rules have more hot bits.
We take near-perfect reasoners trained on rules drawn from the green band (\(0.2 \leq p_\alpha, p_\beta \leq 0.3\)) and test them on rules with antecedent and consequent probabilities \(p_\alpha ^{\msf{test}} = p_\beta ^{\msf{test}} = p^{\msf{test}}\) for \(p^{\msf{test}} \in \{0.1, 0.2, \ldots, 0.9\}\).
The reasoner accuracy decays when \(p^{\msf{test}} \gg 0.3\), but not when \(p^{\msf{test}} = 0.1\).}
\label{fig:q2_additional_prob}
\end{figure}

\begin{figure}[!htb]
\centering
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp4_additional/exp4_rules_plot_128.pdf}
% \includegraphics[width=0.5\linewidth]{images/exp_plots/exp4_additional/exp4_rules_plot_160.pdf}
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_rules_plot_128.pdf}
\end{minipage}%
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_rules_plot_160.pdf}
\end{minipage}
\begin{minipage}{0.33\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{images/exp_plots/exp4_additional/exp4_rules_plot_192.pdf}
\end{minipage}
\caption{Near-perfect in-distribution reasoners fail to generalize when they see more rules than what they are trained on.
We take near-perfect reasoners trained on some number of rules drawn from the green band (\(16 \leq r \leq 64\)) and test them on distributions with \(r^{\msf{test}} \in \{8, 128, 256, 512\}\) number of rules.
For \(r^{\msf{test}} > 64\), the reasoning accuracy is lower than the near-perfect accuracy obtained for \(r^{\msf{test}} \leq 64\).}
\label{fig:q2_additional_rules}
\end{figure}

==> old/old_figures/q5_additional.tex <==
\begin{figure}[ht]
\centering
\begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[width=0.95\linewidth]{images/exp_plots/exp5_additional/ablations_heads.png}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[width=0.95\linewidth]{images/exp_plots/exp5_additional/ablations_layers.png}
\end{minipage}
\caption{Ablations on the number of heads \(H\) and the number of layers \(L\) for learning with \(n = 32\) propositions. When \(H = 1\) heads and \(L \in \{1, 2, 4, 8\}\) layers, the reasoning performance improves as \(L\) increases for embedding dimension \(d = 64\) but remains unchanged for \(d = 32\). Surprisingly and in contrast, when \(L = 1\) layers and \(H \in \{1, 2, 4, 8\}\) heads, the reasoning performance drops as \(H\) increases for \(d = 64\) and remains unchanged for \(d = 32\).}
\label{fig:q5_additional_ablations}
\end{figure}

==> old/old_reasoning.tex <==
\subsection{Results for Logical Reasoning}
\label{sec:theory_logic}

\begin{theorem}[One-Step Propositional Inference]
\label{thm:one_layer_one_step}
Consider any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and proof states \(s_0, \ldots, s_{t-1} \in \mbb{B}^n\) such that each \(s_{k+1} = \Gamma(s_k)\).
Let \(d = 1 + 2n\) and fix any \(0 \leq \delta < 1/3\), \(\mu \geq r + t\), and \(\lambda > \log(\mu^3 / \delta)\), then
for \(\msf{Transformer}\) as defined in~\eqref{eqn:appendix_tf} we have:
\begin{align*}
    X =
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \beta_r ^\top \\
        1 & \mbf{0}_n ^\top & s_0 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Transformer}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \star \\
        1 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^\top & \Gamma(s_{t-1}) ^\top
    \end{bmatrix}
    = Y
\end{align*}
\end{theorem}
\begin{proof}
As an overview, we summarize the action of \(\msf{Id} + \msf{Attn}\) in~\eqref{eqn:one_layer_idattn} and the action of \(\msf{Id} + \msf{Ffwd}\) in~\eqref{eqn:one_layer_idffwd}.
We first analyze the \(\msf{Id} + \msf{Attn}\) component.
Let \(N = r + t\) be the sequence length and decompose \(\msf{Attn}(X)\) as follows:
\begin{align} \label{eqn:one_layer_attn_decomp}
    \msf{Attn}(X)
    = \msf{CausalSoftmax}(\lambda X(\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a X^\top) X \mu \Pi_b ^\top \Pi_b
    = \sum_{i = 1}^{N} \mu e_i \sigma_i ^\top X \Pi_b ^\top \Pi_b
\end{align}
where \(e_1, \ldots, e_N \in \mbb{R}^N\) are the basis vectors and \(\sigma_1, \ldots, \sigma_N \in \mbb{R}^{N}\) are the rows of \(\msf{CausalSoftmax}(\ldots)\).
In particular,
\begin{align}
    \sigma_N &= \msf{Softmax}(\lambda x_N ^\top (\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a x_1, \ldots, \lambda x_N ^\top (\Pi_b - \mbf{1}_n \Pi_1)^\top \Pi_a x_N)
    \nonumber \\
    &= \msf{Softmax}(\lambda (s_{t-1} - \mbf{1}_n)^\top \alpha_1, \ldots, \lambda (s_{t-1} - \mbf{1}_n)^\top \alpha_N) \tag{\(\alpha_i = \Pi_i x_i\) with \(\alpha_i = \mbf{0}_n\) for \(i \geq r+1\)} \\
    &= \msf{Softmax}(\lambda z_1, \ldots, \lambda z_N)
    \label{eqn:one_layer_sigmaN_softmax}
\end{align}
where recall that \(s_{t-1} = \Pi_b x_N\),
% \todo{SG: $\Pi_b$ is confusing when you use $\Pi_i$ for multiplication}
and each \(z_1, \ldots, z_N\) is an integer such that:
\begin{align*}
    z_i = (s_{t-1} - \mbf{1}_n) ^\top \alpha_i
    \quad
    \begin{dcases}
        = 0, &\alpha_i \preceq s_{t-1} \\
        < 0, &\text{otherwise}
    \end{dcases}
\end{align*}
Additionally, because \(z_N = 0\) and \(\lambda > 0\), we may then apply Lemma~\ref{lem:one_layer_softmax} on~\eqref{eqn:one_layer_sigmaN_softmax} to yield:
% \todo{This is not easy to follow, might be worthwhile defining the lemma here.}
\begin{align} \label{eqn:one_layer_sigmaN_decomp}
    \sigma_N = \frac{1}{c} \varphi + \varepsilon,
    \quad \varphi = (\alpha_1 \preceq s_{t-1}, \ldots, \alpha_N \preceq s_{t-1}) \in \mbb{B}^N,
    \quad c = \abs{\{i: \alpha_i \preceq s_i\}},
    \quad \norm{\varepsilon}_{\infty} \leq N e^{-\lambda} \leq \mu e^{-\lambda}
\end{align}
% \todo{SG: For $\psi$, use indicators so it is clear what each entry is.}
In particular, observe that:
\begin{align*}
    \varphi^\top X \Pi_b
    = s_{\oplus} ^\top + \beta_{\oplus} ^\top,
    \qquad
    s_{\oplus} ^\top
    = s_0 ^\top + \cdots + s_{t-1} ^\top,
    \qquad
    \beta_{\oplus} ^\top = \sum_{(\alpha, \beta) \in \Gamma : \alpha \preceq s_{t-1}} \beta^\top
\end{align*}
% \todo{SG: Maybe $\Sigma$ instead of $\oplus$}
meaning that we may rewrite~\eqref{eqn:one_layer_attn_decomp} as follows:
\begin{align*}
    \msf{Attn}(X)
    &= \mu e_N \sigma_N ^\top X \Pi_b ^\top \Pi_b + \sum_{i = 1}^{N-1} \mu e_i \sigma_i ^\top X \Pi_b ^\top \Pi_b
    \tag{Pull out \(N\)th term} \\
    &= \frac{\mu}{c} e_N \varphi ^\top X \Pi_b ^\top \Pi_b
        + e_N \underbrace{\mu\varepsilon ^\top X \Pi_b ^\top}_{\zeta^\top} \Pi_b
        + \sum_{i = 1}^{N-1} \mu e_i \sigma_i ^\top X \Pi_b ^\top \Pi_b
    \tag{\(\sigma_N = (\varphi/c) + \varepsilon\)} \\
    &= \frac{\mu}{c} e_N (s_{\oplus} + \beta_{\oplus})^\top \Pi_b
        + e_N \zeta^\top \Pi_b
        + \sum_{i = 1}^{N-1} \mu e_i \sigma_i ^\top X \Pi_b ^\top \Pi_b
\end{align*}
% \todo{Is $\zeta$ being defined here? I would  recommend a table of notations}
and therefore,
\begin{align} \label{eqn:one_layer_idattn}
    X = 
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \beta_r ^\top \\
        1 & \mbf{0}_n ^\top & s_0 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \star \\
        1 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^\top
        & (s_{t-1} + (\mu/c)(s_{\oplus} + \beta_{\oplus}) + \zeta)^\top
    \end{bmatrix}
\end{align}
where \(\star\) denotes miscellaneous entries of the appropriate dimensions.
We next analyze the last row of the~\eqref{eqn:one_layer_idattn} RHS.
To do this, we bound the residual term \(\zeta\) as:
\begin{align*}
    \norm{\zeta}_\infty
    = \norm{\mu \Pi_b X^\top \varepsilon}_\infty
    \leq \mu \norm{\mbf{1}_N \mbf{1}_N ^\top \varepsilon}_\infty
    \leq \mu N \norm{\varepsilon}_\infty
    \leq \mu ^3 e ^{-\lambda}
    < \delta
    \tag{\(\norm{\varepsilon}_\infty \leq \mu e^{-\lambda}\) by~\eqref{eqn:one_layer_sigmaN_decomp}}
\end{align*}
which allows us to derive for the last row of the~\eqref{eqn:one_layer_idattn} RHS that:
\begin{align} \label{eqn:one_layer_idffwd}
    \underbrace{
    \begin{bmatrix}
        1 \\ \mbf{0}_n \\
        s_{t-1} + (\mu/c) (s_{\oplus} + \beta_{\oplus})
    \end{bmatrix}}_{\text{Each entry either \(=0\) or \(\geq 1\) since \(\mu/c \geq 1\)}}
    + \underbrace{\begin{bmatrix} 0 \\ \mbf{0}_n \\ \zeta
    \end{bmatrix}}_{\norm{\cdot}_\infty < \delta}
    \xrightarrow{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        1 \\ \mbf{0}_n \\
        s_{t-1} \lor \bigvee \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s_{t-1}\}
    \end{bmatrix}
    = \begin{bmatrix}
        1 \\ \mbf{0}_n \\ \Gamma(s_{t-1})
    \end{bmatrix}
\end{align}
Specifically, we used the property that sum-then-binarize implements binary disjunctions and the fact that each \(s_{k+1} \succeq s_k\) by definition of \(s_{k+1} = \Gamma(s_k)\).
All together, composing \(\msf{Id} + \msf{Attn}\) with \(\msf{Id} + \msf{Ffwd}\) yields:
\begin{align*}
    X =
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \beta_r ^\top \\
        1 & \mbf{0}_n ^\top & s_0 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^ \top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:one_layer_idattn}]{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_r ^\top & \star \\
        1 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^ \top
        & (s_{t-1}
            + (\mu/c)(s_{\oplus} + \beta_{\oplus}) + \zeta)^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:one_layer_idffwd}]{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_1 ^\top & \star \\
        1 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \mbf{0}_n ^\top & \Gamma(s_{t-1})^\top
    \end{bmatrix}
    = Y
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma} \label{lem:one_layer_softmax}
Consider any \(z \in \mbb{R}^{N}\) where each coordinate is either \(z_i \leq -1\) or \(z_i = 0\), and additionally assume that \(c = \abs{\{i: z_i = 0\}} \geq 1\).
For any \(\lambda > 0\), let \(\varepsilon = \msf{Softmax}(\lambda z) - (\varphi/c)\) where \(\varphi = \mbb{I}[z = 0] \in \mbb{B}^N\), then \(\norm{\varepsilon}_\infty \leq (N-c) e^{-\lambda}\).
\end{lemma}
\begin{proof}
Note that if \(c = N\), then \(\norm{\varepsilon}_\infty = 0\), so we assume \(c < N\).
First consider some \(i\) for which \(z_i < 0\),
\begin{align*}
    \abs{\varepsilon_i}
    = \frac{e^{\lambda z_i}}{c + \sum_{i : z_i < 0} e^{\lambda z_i}}
    \leq \frac{e^{\lambda z_i}}{c}
    \leq e^{\lambda z_i}
    \leq e^{-\lambda}
\end{align*}
because \(\sum_{i: z_i < 0} e^{\lambda z_i} > 0\) and \(c \geq 1\).
Next, consider some \(i\) for which \(z_i = 0\),
\begin{align*}
    \abs{\varepsilon_i}
    = \frac{1}{c} - \frac{1}{c + \sum_{i : z_i < 0} e^{\lambda w_i}}
    \leq \frac{\sum_{i : z_i < 0} e^{\lambda z_i}}{c^2 + c \sum_{i : z_i < 0} e^{\lambda z_i}}
    \leq \frac{1}{c^2} \sum_{i: z_i \leq 0} e^{\lambda z_i}
    \leq \sum_{i : z_i < 0} e^{\lambda z_i}
    \leq (N - c) e^{-\lambda}
\end{align*}
Because \(e^{-\lambda} \leq (N - c) e^{-\lambda}\), the desired inequality follows.
\end{proof}




==> old/old_theory/additional_experiments.tex <==
\section{Additional Experiments}
\label{sec:additional_experiments}


\subsection{Ablations on Model Parameters}
\label{sec:appendix_model_params}

% \input{figures/q5_additional}

\subsection{Additional Plots for the Theoretical Attack Experiments}
\label{sec:appendix_theory_attack}

\input{figures/q2_additional}

\subsection{Additional Plots for the Out-of-Distribution Robustness Experiments}
\label{sec:appendix_ood}

\input{figures/q4_additional}





==> old/old_theory/attack.tex <==
\subsection{Results for Adversarial Attacks}
\label{sec:theory_attack}

We now present our results for adversarial attacks against our theoretical language model construction.

\begin{theorem}[Adversarial Attack]
\label{thm:attack}
Take the definitions as in Theorem~\ref{thm:reasoning} and define \(\msf{Transformer}\) with \(\mu \geq r + t + 2\).
Let \(s_{\msf{tgt}} \in \mbb{B}^n\) be any adversarial target and define \(\beta_{\msf{atk}} = s_{\msf{tgt}} - \kappa (\mbf{1}_n - s_{\msf{tgt}})\) for some \(\kappa \geq \mu\).
Then,
\begin{align*}
    X_{\msf{atk}}
    = \msf{append}(X, (1, \mbf{0}_n, \beta_{\msf{atk}}))
    =
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Transformer}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \star \\
        1 & \mbf{0}_n ^\top & s_{\msf{tgt}} ^\top
    \end{bmatrix}
    = Y_{\msf{atk}}
\end{align*}
\end{theorem}
\begin{proof}
We take a similar approach as in Theorem~\ref{thm:reasoning}, and likewise expand the attention component as follows:
\begin{align*}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \mbf{0}_n ^\top & \beta_{\msf{atk}}^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \frac{\mu}{c} \beta_{\msf{atk}} ^\top
        + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \varepsilon^\top
    \end{bmatrix}
    \tag{Lemma~\ref{lem:reasoning_softmax}}
\end{align*}
where \(\norm{\varepsilon}_\infty < 1/3\)  and \(c = 1 + \abs{\{i: \alpha_i \preceq \beta_{\msf{atk}}\}}\)  for \(i = 1, \ldots, N\).
Except now the above approximates \(s_{\msf{tgt}}\) in that:
\begin{align*}
\begin{split}
    \braces*{j \in \{1, \ldots, n\}:
        \parens*{\frac{c+\mu}{c} \beta_{\msf{atk}}
            + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i
            + \varepsilon
        }_j > 2/3
    }
    &= \braces*{j \in \{1, \ldots, n\}:
        (s_{\msf{tgt}})_j = 1
    } \\
    \braces*{j \in \{1, \ldots, n\}:
        \parens*{\frac{c+\mu}{c} \beta_{\msf{atk}} 
            + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i
            + \varepsilon
        }_j < 1/3
    }
    &= \braces*{j \in \{1, \ldots, n\}:
        (s_{\msf{tgt}})_j = 0}
\end{split}
\tag{Lemma~\ref{lem:attack_approx}}
\end{align*}
Because \(\msf{Id} + \msf{Ffwd}\) implements binarization with \(1/3\) tolerance, we have:
\begin{align*}
    \begin{bmatrix}
        1 \\ \mbf{0}_n \\
        \frac{c+\mu}{c}\beta_{\msf{atk}}
        + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i
        + \varepsilon
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        1 \\ \mbf{0}_n \\ s_{\msf{tgt}}
    \end{bmatrix}
\end{align*}
\end{proof}



%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:attack_softmax}
Take the definitions as in Theorem~\ref{thm:attack} and its proof, then:
\begin{align*}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top \\
        1 & \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Attn}}
    \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \frac{\mu}{c} \beta_{\msf{atk}}^\top + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \star \\
        0 & \mbf{0}_n ^\top & \varepsilon^\top
    \end{bmatrix}
\end{align*}
where \(\norm{\varepsilon}_\infty < 1/3\) and \(c = 1 + \abs{\{i: \alpha_i \preceq s_{\msf{tgt}}\}}\) for \(i = 1, \ldots, N\).
\end{lemma}
\begin{proof}
We proceed similarly to the proof of Lemma~\ref{lem:reasoning_softmax}, where we eventually arrive at:
\begin{align*}
    \msf{CausalSoftmax}(X_{\msf{atk}} W_Q W_K ^\top X_{\msf{atk}}^\top)
    =
    \begin{bmatrix}
        \msf{Softmax}(\lambda (\beta_1 ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), & \ldots, & -\infty, & -\infty) \\
        \vdots & \ddots & \vdots & \vdots \\
        \msf{Softmax}(\lambda (\beta_N ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), & \ldots, & \lambda (\beta_N ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N), & -\infty) \\
        \msf{Softmax}(\lambda (\beta_{\msf{atk}}^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), & \ldots, & \lambda (\beta_{\msf{atk}}^\top \alpha_N - \mbf{1}_n ^\top \alpha_N), & 0)
    \end{bmatrix}
    % \begin{bmatrix}
    %     \star \\ \vdots \\
    %     \msf{Softmax}(\lambda (\beta_N ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), \ldots, \lambda (\beta_N ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N), -\infty) \\
    %     \msf{Softmax}(\lambda (\beta_{\msf{atk}} ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), \ldots, \lambda (\beta_{\msf{atk}}^\top \alpha_N - \mbf{1}_n ^\top \alpha_N), 0)
    % \end{bmatrix}
\end{align*}
For the \(\msf{Softmax}\) arguments \(i = 1, \ldots, N\) in the last row of the above, we have:
\begin{align*}
    \beta_{\msf{atk}} ^\top \alpha_i - \mbf{1}_n ^\top \alpha_i
    &= \parens*{s_{\msf{tgt}} - \kappa(\mbf{1}_n - s_{\msf{tgt}})}^\top \alpha_i - \mbf{1}_n ^\top \alpha_i \\
    &= s_{\msf{tgt}} ^\top \alpha_i
        - \kappa \mbf{1}_n ^\top \alpha_i
        + \kappa s_{\msf{tgt}} ^\top \alpha_i
        - \mbf{1}_n ^\top \alpha_i \\
    &= s_{\msf{tgt}}^\top \alpha_i - \mbf{1}_n ^\top \alpha_i
        + \kappa s_{\msf{tgt}} ^\top \alpha_i - \kappa \mbf{1}_n ^\top \alpha_i \\
    &= (1 + \kappa) (s_{\msf{tgt}}^\top \alpha_i - \mbf{1}_n ^\top \alpha_i)
\end{align*}
and therefore by Lemma~\ref{lem:preceq_insight}:
\begin{align*}
    \lambda (\beta_{\msf{atk}}^\top \alpha_i - \mbf{1}_n ^\top \alpha_i)
    \quad \begin{dcases}
        = 0, & \alpha_i \preceq s_{\msf{tgt}} \\
        \leq - \lambda(1 + \kappa), &\text{otherwise}
    \end{dcases}
\end{align*}
We then apply Lemma~\ref{lem:softmax_approx} to yield:
\begin{align*}
    \msf{Softmax}(\lambda (\beta_{\msf{atk}} ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), \ldots, \lambda (\beta_{\msf{atk}}^\top \alpha_N - \mbf{1}_n ^\top \alpha_N), 0)
    = \frac{1}{c}
    (\alpha_1 \preceq s_{\msf{tgt}}, \ldots, \alpha_N \preceq s_{\msf{tgt}}, 1) + \zeta
\end{align*}
where \(\norm{\zeta}_\infty < (N+1) e^{-\lambda (1 + \kappa)}\) and let \(c = 1 + \abs{\{i: \alpha_i \preceq \beta_{\msf{atk}}\}}\).
Substituting this into \(\msf{Attn}(X_{\msf{atk}})\):
\begin{align*}
    \msf{Attn}(X_{\msf{atk}})
    &= \msf{CausalSoftmax}(X_{\msf{atk}} W_Q W_K ^\top X_{\msf{atk}} ^\top)
    X_{\msf{atk}} \mu \Pi_b ^\top \Pi_b \\
    &= \begin{bmatrix}
        \star & \cdots & \star & \star \\
        \vdots & \ddots & \vdots & \vdots \\
        \frac{1}{c} (\alpha_1 \preceq s_{\msf{tgt}}) & \cdots & \frac{1}{c} (\alpha_N \preceq s_{\msf{tgt}}) & \frac{1}{c}
    \end{bmatrix}
    X_{\msf{atk}} \mu \Pi_b ^\top \Pi_b
    + \begin{bmatrix} \star \\ \vdots \\ \zeta^\top \end{bmatrix}
    X_{\msf{atk}} \mu \Pi_b ^\top \Pi_b \\
    &= \begin{bmatrix}
        \star & \cdots & \star & \star \\
        \vdots & \ddots & \vdots & \vdots \\
        \frac{\mu}{c} (\alpha_1 \preceq s_{\msf{tgt}}) & \cdots & \frac{\mu}{c} (\alpha_N \preceq s_{\msf{tgt}}) & \frac{\mu}{c}
    \end{bmatrix}
    \begin{bmatrix} \beta_1 ^\top \\ \vdots \\ \beta_N ^\top \\ \beta_{\msf{atk}} ^\top
    \end{bmatrix} \Pi_b
        + \begin{bmatrix} \star \\ \vdots \\ \mu \zeta^\top X_{\msf{atk}} \Pi_b ^\top
    \end{bmatrix} \Pi_b \\
    &= \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \frac{\mu}{c} \beta_{\msf{atk}}^\top + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \mu \zeta^\top X_{\msf{atk}} \Pi_b ^\top
    \end{bmatrix}
\end{align*}
Finally, we bound the residual term as:
\begin{align*}
    \norm{\mu \Pi_b X_{\msf{atk}} ^\top \zeta}_\infty
    \leq \mu \norm{\Pi_b X_{\msf{atk}} ^\top \zeta}_\infty
    \leq \mu \norm{\kappa \mbf{1}_n \mbf{1}_{N+1} ^\top \zeta}_\infty
    \leq \kappa \mu (N+1) \norm{\zeta}_\infty
    \leq \kappa \mu^3 e^{-\lambda (1 + \kappa)}
    = \underbrace{\parens*{\kappa \mu^3 e^{-\lambda}}}_{< \kappa / 3}
    \underbrace{\parens*{\kappa \mu^3 e^{-\lambda \kappa}}}_{\leq 1 / \kappa}
\end{align*}
which holds for all \(\kappa \geq 1\) because \(\mu^3 e^{-\lambda} < 1/3\), where recall that each entry of \(\abs{X_{\msf{atk}}}\) is \(\leq \kappa\) and \((N+1) \leq \mu\).
\end{proof}

%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:attack_approx}
Take the definitions as in Theorem~\ref{thm:attack}, then:
\begin{align*}
\begin{split}
    \braces*{j \in \{1, \ldots, n\}:
        \parens*{\frac{c+\mu}{c} \beta_{\msf{atk}}
            + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i
            + \varepsilon
        }_j > 2/3
    }
    &= \braces*{j \in \{1, \ldots, n\}:
        (s_{\msf{tgt}})_j = 1
    } \\
    \braces*{j \in \{1, \ldots, n\}:
        \parens*{\frac{c+\mu}{c} \beta_{\msf{atk}} 
            + \frac{\mu}{c} \sum_{i: \alpha_i \preceq s_{\msf{tgt}}} \beta_i
            + \varepsilon
        }_j < 1/3
    }
    &= \braces*{j \in \{1, \ldots, n\}:
        (s_{\msf{tgt}})_j = 0}
\end{split}
\end{align*}
\end{lemma}
\begin{proof}
By construction, we have:
\begin{align*}
    \braces*{j: (s_{\msf{tgt}})_j = 1}
    &= \braces*{j: (\beta_{\msf{atk}})_j = 1}, \\
    \braces*{j: (s_{\msf{tgt}})_j = 0}
    &= \braces*{j: (\beta_{\msf{atk}})_j = -\kappa},
\end{align*}
Because \(\kappa \geq \mu \geq N\) is quite big and \(\beta_1, \ldots, \beta_N \in \mbb{B}^n\), we have:
\begin{align*}
    \braces*{j: (s_{\msf{tgt}})_j = 1}
    &= \braces*{j:
        \parens*{
        \beta_{\msf{atk}}
        + \sum_{i : \alpha_i \preceq s_{\msf{tgt}}}
            \beta_i
        }_j \geq 1
    }
    = \braces*{j:
        \parens*{
        \frac{c+\mu}{c} \beta_{\msf{atk}}
        + \frac{\mu}{c} \sum_{i : \alpha_i \preceq s_{\msf{tgt}}}
            \beta_i
        }_j \geq 1
    } \\
    \braces*{j: (s_{\msf{tgt}})_j = 0}
    &= \braces*{j:
        \parens*{
        \beta_{\msf{atk}}
        + \sum_{i : \alpha_i \preceq s_{\msf{tgt}}}
            \beta_i
        }_j \leq 0
    }
    = \braces*{j:
        \parens*{
        \frac{c+\mu}{c} \beta_{\msf{atk}}
        + \frac{\mu}{c} \sum_{i : \alpha_i \preceq s_{\msf{tgt}}}
            \beta_i
        }_j \leq 0
    }
\end{align*}
where recall that \((c + \mu)/c \geq (\mu/c) \geq 1\).
Finally, apply \(\norm{\varepsilon}_\infty < 1/3\) to get the desired result.
\end{proof}

==> old/old_theory/construction_1.tex <==
\subsection{A Language Model for One Reasoning Step}
\label{sec:theory_construction}

We now present our theoretical construction for one step of propositional inference.
Recall that our language model consists of the following modules:
\begin{align} \label{eqn:appendix_lm}
    \msf{LM}: U \in \mbb{R}^{N \times d_{\msf{in}}}
    \xrightarrow{\msf{Embed}}
    X \in \mbb{R}^{N \times d}
    \xrightarrow{\msf{Transformer}}
    Y \in \mbb{R}^{N \times d}
    \xrightarrow{\msf{ClsHead}}
    s \in \mbb{R}^{d_{\msf{out}}}
\end{align}
with token dimension \(d_{\msf{in}} = 2n\), embedding dimension \(d = 1 + 2n\), and output label dimension \(d_{\msf{out}} = n\),
where \(n\) is the number of propositions.
We define \(\msf{Embed}\) and \(\msf{ClsHead}\) in~\eqref{eqn:appendix_embed_clshead}, and \(\msf{Transformer}\) in~\eqref{eqn:appendix_tf}.
Now consider some set of rules \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and proof states \(s_0, \ldots, s_{t}\), and let \(N = r + t + 1\) be the input sequence length.
The intermediate stages of \(\msf{LM}\) then take the following forms:
\begin{align*}
    U = \begin{bmatrix}
        \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots \\
        \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \in \mbb{R}^{N \times (n + n)},
    \enskip
    X = \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \in \mbb{R}^{N \times (1 + n + n)},
    \enskip
    Y = \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \Gamma(s_{t})^\top
    \end{bmatrix}
    \in \mbb{R}^{N \times (1 + n + n)}
\end{align*}
where let \(\alpha_{r + k + 1} = \mbf{0}_n\) and \(\beta_{r+k+1} = s_k\) for all \(k = 0, \ldots, t\).
This suggestive naming is used because we treat each proof state \(s_k\) as a rule \((\mbf{0}_n, s_k)\).
Also, recall that \(\msf{Embed}\) and \(\msf{ClsHead}\) are linear projections defined as:
\begin{align} \label{eqn:appendix_embed_clshead}
    \begin{bmatrix} u_a \\ u_b \end{bmatrix} \in \mbb{R}^{n + n}
    \xrightarrow{\msf{Embed}}
    \begin{bmatrix} 1 \\ u_a \\ u_b \end{bmatrix}
    \in \mbb{R}^{1 + n + n},
    \qquad
    \begin{bmatrix} z_1 \\ z_a \\ z_b \end{bmatrix} \in \mbb{R}^{1 + n + n}
    \xrightarrow{\msf{ClsHead}}
    z_b \in \mbb{R}^{n}
\end{align}
for any \(u_a, u_b, z_a, z_b \in \mbb{R}^{n}\).
Moreover, the one-layer \(\msf{Transformer}\) module is defined as follows:
\begin{align} \label{eqn:appendix_tf}
    \msf{Transformer}(X) = 
        ((\msf{Id} + \msf{Ffwd}) \circ (\msf{Id} + \msf{Attn}))(X)
\end{align}
where we define \(\msf{Attn}\) in~\eqref{eqn:appendix_attn} and \(\msf{Ffwd}\) in~\eqref{eqn:appendix_ffwd} (with \(\delta = 1/3)\).


Our main insight is that we can test the \(\preceq\) relation between two binary vectors using a weighted inner product.
This is relevant because the attention mechanism effectively implements a weighted inner product between each row of the embedded inputs.

\begin{lemma}
\label{lem:preceq_insight}
For any \(x, y \in \mbb{B}^n\):
\begin{align*}
    \begin{bmatrix} y \\ 1 \end{bmatrix}^\top
    \begin{bmatrix} I_n & \mbf{0}_n \\ -\mbf{1}_n ^\top & 0 \end{bmatrix}
    \begin{bmatrix} x \\ 1 \end{bmatrix}
    = y^\top x - \mbf{1}_n ^\top x
    \quad
    \begin{dcases}
        = 0, & x \preceq y \\
        \leq -1 & \text{otherwise}
    \end{dcases}
\end{align*}
\end{lemma}
Next, we define the linear projection matrices \(\Pi_1 : \mbb{R}^{1 \times (1 + 2n)}\), \(\Pi_a: \mbb{R}^{n \times (1 + 2n)}\), and \(\Pi_b : \mbb{R}^{n \times (1 + 2n)}\) to act as follows:
\begin{align*}
% \label{eqn:appendix_projections}
    &\begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \Pi_1 ^\top =
    \begin{bmatrix} 1 \\ \vdots \\ 1 \end{bmatrix},
    &&
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \Pi_a ^\top =
    \begin{bmatrix}
        \alpha_1 ^\top \\ \vdots \\ \alpha_N ^\top
    \end{bmatrix},
    &&
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \Pi_b ^\top =
    \begin{bmatrix}
        \beta_1 ^\top \\ \vdots \\ \beta_N ^\top
    \end{bmatrix}
    \\
    &\begin{bmatrix} 1 \\ \vdots \\ 1 \end{bmatrix}
    \Pi_1
    = \begin{bmatrix} 1 & \mbf{0}_n ^\top & \mbf{0}_n ^\top \\
    \vdots & \vdots & \vdots \\
    1 & \mbf{0}_n ^\top & \mbf{0}_n ^\top
    \end{bmatrix},
    &&
    \begin{bmatrix} \alpha_1 ^\top \\ \vdots \\ \alpha_N ^\top \end{bmatrix}
    \Pi_a
    =
    \begin{bmatrix} 0 & \alpha_1 ^\top & \mbf{0}_n ^\top \\
    \vdots & \vdots & \vdots \\
    0 & \alpha_N ^\top & \mbf{0}_n ^\top
    \end{bmatrix},
    &&
    \begin{bmatrix} \beta_1 ^\top \\ \vdots \\ \beta_N ^\top \end{bmatrix}
    \Pi_b
    =
    \begin{bmatrix} 0 & \mbf{0}_n ^\top & \beta_1 ^\top \\
    \vdots & \vdots & \vdots \\
    0 & \mbf{0}_n ^\top & \beta_N ^\top
    \end{bmatrix}
\end{align*}
for any \(\alpha_1, \ldots, \alpha_N \in \mbb{R}^{n}\) and \(\beta_1, \ldots, \beta_N \in \mbb{R}^{n}\).
We then define \(\msf{Attn}\) as follows:
\begin{equation} \label{eqn:appendix_attn}
\begin{gathered}
    \msf{Attn}(X)
    = \msf{CausalSoftmax}\parens*{
        X W_Q W_K^\top X^\top
    }X W_v \\
    W_Q = \lambda I_d,
    \qquad
    W_K ^\top =
    \begin{bmatrix} \Pi_b \\ \Pi_1 \end{bmatrix}^\top
    \begin{bmatrix}
        I_n & \mbf{0}_n \\
        - \mbf{1}_n ^\top & 0
    \end{bmatrix}
    \begin{bmatrix} \Pi_a \\ \Pi_1 \end{bmatrix},
    \qquad W_V = \mu \Pi_b ^\top \Pi_b
\end{gathered}
\end{equation}
for some scaling parameters \(\lambda, \mu > 0\).
Intuitively, \(W_Q W_K ^\top\) will apply a \(\lambda\)-scaled version of the \(\preceq\) test described in Lemma~\ref{lem:preceq_insight}.
Next, observe that a one-layer feedforward neural network to construct a binarization function:
\begin{align}
\label{eqn:appendix_ffwd}
    \msf{Ffwd}(x) = 
    \msf{ReLU}(-x) - \msf{ReLU}(x)
    + \msf{ReLU}((x - 1 + 2 \delta) / \delta)
    - \msf{ReLU}((x - 1 + \delta)/\delta)
\end{align}
where \(\delta\) is called the \emph{tolerance}.
In particular, binarization occurs in the following sense:

\begin{lemma}
For any \(0 < \delta < 1\) and take \(\msf{Ffwd}\) as in~\eqref{eqn:appendix_ffwd}, then:
\begin{align*}
    (\msf{Id} + \msf{Ffwd})(x)
    = \begin{dcases}
        0, & x \leq 1 - 2 \delta \\
        (x - 1 + 2\delta)/\delta, & 1 - 2 \delta < x < 1 - \delta \\
        1, & 1 - \delta \leq x
    \end{dcases}
\end{align*}
If we take \(\delta = 1/3\), then:
\begin{align*}
    (\msf{Id} + \msf{Ffwd})(x)
    = \begin{dcases}
        0, &\quad x \leq 1/3 \\
        3x - 1, &\quad 1/3 < x < 2/3 \\
        1, &\quad 2/3 \leq x
    \end{dcases}
\end{align*}
\end{lemma}

==> old/old_theory/log_depth.tex <==
\subsection{Logarithmic depth}

\begin{definition}[Quasi-composition of rule sets]
For any two rule sets \(\Gamma, \Gamma'\), define:
\begin{align*}
    \Gamma' \triangleleft \Gamma
    = \{(\alpha, \Gamma'(\Gamma(\alpha))): (\alpha, \beta) \in \Gamma\}
\end{align*}
\end{definition}




\begin{lemma}[Rule application is monotone]
\label{lem:rule_app_monotone}
For any \(s, s' \in \mbb{B}^n\) and rule set \(\Gamma\):: \(s \preceq s'\) iff \(\Gamma(s) \preceq \Gamma(s')\).
\end{lemma}


\begin{lemma}[Quasi-composition behaves like composition]
Consider any two rule sets \(\Gamma, \Gamma'\) and suppose that \(\alpha^\star \in \mbb{B}^n\) is the antecedent of some rule in \(\Gamma\),
then \((\Gamma' \triangleleft \Gamma) (\alpha^\star) = \Gamma' (\Gamma(\alpha^\star))\).
\end{lemma}
\begin{proof}
We expand the definition of rule application~\eqref{eqn:one_step_rules} as follows:
\begin{align*}
    (\Gamma' \triangleleft \Gamma)(\alpha^\star)
    &= \alpha^\star \lor \bigvee_{(\alpha, \beta) \in \Gamma, \alpha \preceq \alpha^\star} \Gamma'(\Gamma(\alpha)) \\
    &= \alpha^\star 
        \lor \underbrace{\parens*{\bigvee_{(\alpha, \beta) \in \Gamma, \alpha = \alpha^\star} \Gamma'(\Gamma(\alpha))}
        }_{\text{\(= \Gamma'(\Gamma(\alpha^\star))\) since there exists \(\alpha = \alpha^\star\)}}
        \lor
        \underbrace{\parens*{
        \bigvee_{(\alpha, \beta) \in \Gamma, \alpha \prec \alpha^\star} \Gamma'(\Gamma(\alpha))
        }}_{\text{\(\preceq \Gamma'(\Gamma(\alpha^\star))\) by monotonicity}} \\
    &= \alpha^\star \lor \Gamma'(\Gamma(\alpha^\star))
    = \Gamma'(\Gamma(\alpha^\star))
\end{align*}
\end{proof}



\begin{lemma}[Quasi-composition is weaker than composition]
For any \(s \in \mbb{B}^n\) and rule sets \(\Gamma, \Gamma'\), \((\Gamma' \triangleleft \Gamma)(s) \preceq \Gamma' (\Gamma(s))\).
\end{lemma}
\begin{proof}
Let \((\alpha, \beta)\) denote a rule of \(\Gamma\) and let \((\alpha', \beta')\) denote a rule of \(\Gamma'\), and expand rule application as follows:
\begin{align*}
    (\Gamma' \triangleleft \Gamma) (s)
    &= s \lor \bigvee_{\alpha: \alpha \preceq s} \Gamma' (\Gamma(\alpha)) \\
    &= s \lor \bigvee_{\alpha: \alpha \preceq s} \parens*{
        \Gamma(\alpha) \lor \bigvee_{\alpha': \alpha' \preceq \Gamma(\alpha)} \beta'
    } \\
    &= \underbrace{s \lor
        \parens*{\bigvee_{\alpha: \alpha \preceq s} \Gamma (\alpha)}}_{\text{\(= \Gamma(s)\) since \(\beta \preceq \Gamma(\alpha) \preceq \Gamma(s)\)}}
    \lor \bigvee_{\alpha: \alpha \preceq s}
        \parens*{
        \bigvee_{\alpha': \alpha' \preceq \Gamma(\alpha)} \beta'
    } \\
    &= \Gamma(s) \lor \bigvee_{\alpha: \alpha \preceq s} \parens*{\bigvee_{\alpha': \alpha' \preceq \Gamma(\alpha)} \beta'} \\
    &\preceq \Gamma(s) \lor \bigvee_{\alpha: \alpha \preceq s} \parens*{\bigvee_{\alpha': \alpha' \preceq \Gamma(s)} \beta'} \\
    &\preceq \Gamma(s) \lor \bigvee_{\alpha': \alpha' \preceq \Gamma(s)} \beta'
    = \Gamma'(\Gamma(s))
\end{align*}

\end{proof}



\begin{lemma}[Restricted quasi-composition is associative]
Let \(\Gamma, \Gamma', \Gamma''\) be any rule sets with the same antecedents, i.e.,
\begin{align*}
    \Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\},
    \qquad \Gamma' = \{(\alpha_1, \beta_1 '), \ldots, (\alpha_r, \beta_r ' )\},
    \qquad \Gamma' = \{(\alpha_1, \beta_1 ''), \ldots, (\alpha_r, \beta_r '')\},
\end{align*}
for some \(\alpha_i, \beta_i, \beta_i ', \beta_i '' \in \mbb{B}^n\),
then \((\Gamma'' \triangleleft \Gamma') \triangleleft \Gamma = \Gamma'' \triangleleft (\Gamma' \triangleleft \Gamma)\).
\end{lemma}
\begin{proof}
    \red{AAAAAAAAAA}
\end{proof}



==> old/old_theory/reasoning.tex <==
\subsection{Proofs for One Reasoning Step}

We now formally state and prove our main reasoning result, with a focus on the correctness of a single autoregressive step.

\begin{theorem}[One Reasoning Step]
\label{thm:reasoning}
Define \(\msf{Transformer}\) as in~\eqref{eqn:appendix_tf} by fixing any \(\mu \geq r + t + 1\) and \(\lambda > \log(3 \mu^3)\), where the number of rules \(r\) and the number of previous steps \(t\) are given.
Let \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) be any rule set and \(s_0, \ldots, s_{t} \in \mbb{B}^n\) be any proof states, where each \(s_{k+1} = \Gamma(s_k)\).
Then,

% Then, for any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and proof states \(s_0, \ldots, s_{t} \in \mbb{B}^n\), where each \(s_{k+1} = \Gamma(s_k)\), we have:

% Consider any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and proof states \(s_0, \ldots, s_{t} \in \mbb{B}^n\) where each \(s_{k+1} = \Gamma(s_k)\).
% Define \(\msf{Transformer}\) as in~\eqref{eqn:appendix_tf} for any \(\mu \geq r + t + 1\) and \(\lambda > \log(3 \mu^3)\).
% Then,

% Consider any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and proof states \(s_0, \ldots, s_{t} \in \mbb{B}^n\) where each \(s_{k+1} = \Gamma(s_k)\).
% Define \(\msf{Transformer}\) as in~\eqref{eqn:appendix_tf} 

% Fix any \(\mu \geq r + t + 1\) and \(\lambda > \log(3\mu^3)\), and 
% define \(\msf{Transformer}\) as in~\eqref{eqn:appendix_tf}.
% Then,
\begin{align*}
    X = \begin{bmatrix}
        1 & \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \beta_N ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Transformer}}
    \begin{bmatrix}
        1 & \alpha_1 ^\top & \star \\
        \vdots & \vdots & \vdots \\
        1 & \alpha_N ^\top & \Gamma(s_{t})^\top
    \end{bmatrix}
    = Y,
    \qquad N = r + t + 1,
\end{align*}
where \(\alpha_{r+k+1} = \mbf{0}_n\) and \(\beta_{r+k+1} = s_{k}\) for all \(k = 0, \ldots, t\).
\end{theorem}
\begin{proof}
Recall that \(\msf{Transformer} = (\msf{Id} + \msf{Ffwd}) \circ (\msf{Id} + \msf{Attn})\).
We first expand the attention component as follows:
\begin{align*}
    X = 
    \begin{bmatrix}
            1 & \alpha_1 ^\top & \beta_1 ^\top \\
            \vdots & \vdots & \vdots \\
            1 & \alpha_N ^\top & \beta_N ^\top
        \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
            1 & \alpha_1 ^\top & \beta_1 ^\top \\
            \vdots & \vdots & \vdots \\
            1 & \alpha_N ^\top & \beta_N ^\top
        \end{bmatrix}
        + \begin{bmatrix}
            0 & \mbf{0}_n ^\top & \star \\
            \vdots & \vdots & \vdots \\
            0 & \mbf{0}_n ^\top &
            \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i : \alpha_i \preceq \beta_N} \beta_i ^\top
        \end{bmatrix}
        + \begin{bmatrix}
            0 & \mbf{0}_n ^\top & \star \\
            \vdots & \vdots & \vdots \\
            0 & \mbf{0}_n ^\top & \varepsilon^\top
        \end{bmatrix}
    \tag{Lemma~\ref{lem:reasoning_softmax}}
\end{align*}
where \(\norm{\varepsilon}_\infty < 1/3\).
In particular, the above approximates rule application in the sense that:
\begin{align*}
\begin{split}
    \braces*{j \in \{1, \ldots, n\} :
        \parens*{
            \beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i: \alpha_i \preceq \beta_N} \beta_i
            + \varepsilon
        }_j > 2/3
    }
    &=\braces*{j \in \{1, \ldots, n\} : 
        \Gamma(s_{t})_j = 1
    }
    \\
    \braces*{j \in \{1, \ldots, n\} :
        \parens*{
            \beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i: \alpha_i \preceq \beta_N} \beta_i
            + \varepsilon
        }_j < 1/3
    }
    &=\braces*{j \in \{1, \ldots, n\} : 
        \Gamma(s_{t})_j = 0
    }
\end{split}
\tag{Lemma~\ref{lem:reasoning_approx}}
\end{align*}
Since \(\msf{Id} + \msf{Ffwd}\) implements a binarization function with \(1/3\) tolerance, we thus have:
\begin{align*}
    \begin{bmatrix}
        1 \\ \alpha_N \\
        \beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i : \alpha_i \preceq \beta_N} \beta_i + \varepsilon
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        1 \\ \alpha_N \\ \Gamma(s_{t})
    \end{bmatrix}
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{lemma} \label{lem:reasoning_softmax}
Take the definitions as in Theorem~\ref{thm:reasoning} and its proof, then:
\begin{align*}
    \msf{Attn}(X)
    = \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i : \alpha_i \preceq \beta_N} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top & \varepsilon^\top
    \end{bmatrix},
    \qquad \norm{\varepsilon}_\infty \leq N e ^{-\lambda}
\end{align*}
\end{lemma}
\begin{proof}
Recall that \(\msf{Attn}(X) = \msf{CausalSoftmax}(X W_Q W_K ^\top X^\top) X \mu \Pi_b ^\top \Pi_b\).
We first analyze the \(\msf{CausalSoftmax}(\ldots)\) term:
\begin{align*}
    \msf{CausalSoftmax}(
    X W_Q W_K ^\top X^\top)
    & = \msf{CausalSoftmax}\parens*{\lambda X \begin{bmatrix} \Pi_b \\ \Pi_1 \end{bmatrix} ^\top
    \begin{bmatrix} I_n & \mbf{0}_n \\ -\mbf{1}_n ^\top & 0 \end{bmatrix}
    \begin{bmatrix} \Pi_a \\ \Pi_1 \end{bmatrix}
    X^\top} \\
    & = \msf{CausalSoftmax}\parens*{\lambda
    \begin{bmatrix}
        \beta_1 ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1 & \cdots & \beta_1 ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N \\
        \vdots & \ddots & \vdots \\
        \beta_N ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1 & \cdots & \beta_N ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N
    \end{bmatrix}} \\
    &= 
    \begin{bmatrix}
        \msf{Softmax}(\lambda (\beta_1 ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), & \ldots, & -\infty) \\
        \vdots & \ddots  & \vdots \\
        \msf{Softmax}(\lambda (\beta_N ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), & \ldots, & \lambda (\beta_N ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N)) \\
    \end{bmatrix}
\end{align*}
where observe that for each argument of \(\msf{Softmax}\), we have by Lemma~\ref{lem:preceq_insight}:
\begin{align*}
    \lambda (\beta_N ^\top \alpha_i - \mbf{1}_n ^\top \alpha_i)
    \quad \begin{dcases}
        = 0, &\alpha_i \preceq \beta_N \\
        \leq -\lambda, &\text{otherwise}
    \end{dcases}
\end{align*}
Then, applying Lemma~\ref{lem:softmax_approx}, we get:
\begin{align*}
    \msf{Softmax}(\lambda(\beta_N ^\top \alpha_1 - \mbf{1}_n ^\top \alpha_1), \ldots, \lambda (\beta_N ^\top \alpha_N - \mbf{1}_n ^\top \alpha_N))
    = \frac{1}{c}
    (\alpha_1 \preceq \beta_N, \ldots, \alpha_N \preceq \beta_N) + \zeta
\end{align*}
where \(c = \abs{\{i: \alpha_i \preceq \beta_N\}}\) and \(\norm{\zeta}_\infty \leq N e^{-\lambda}\).
Substituting this into \(\msf{Attn}(X)\) yields the desired form:
\begin{align*}
    \msf{Attn}(X)
    &= \msf{CausalSoftmax}(XW_Q W_K ^\top X^\top) X \mu \Pi_b ^\top \Pi_b \\
    &= \begin{bmatrix}
        \star & \cdots & \star \\
        \vdots & \ddots & \vdots \\
        \frac{1}{c} (\alpha_1 \preceq \beta_N)
        & \cdots & \frac{1}{c} (\alpha_N \preceq \beta_N)
        \end{bmatrix}
        X \mu \Pi_b ^\top \Pi_b
        + \begin{bmatrix} \star \\ \vdots \\ \zeta^\top \end{bmatrix}
        X \mu \Pi_b ^\top \Pi_b
    \\
    &= \begin{bmatrix}
        \star & \cdots & \star \\
        \vdots & \ddots & \vdots \\
        \frac{\mu}{c} (\alpha_1 \preceq \beta_N)
        & \cdots & \frac{\mu}{c} (\alpha_N \preceq \beta_N)
        \end{bmatrix}
    \begin{bmatrix} \beta_1 ^\top \\ \vdots \\ \beta_N ^\top \end{bmatrix}
    \Pi_b
    + \begin{bmatrix} \star \\ \vdots \\ \mu \zeta^\top X \Pi_b ^\top \end{bmatrix} \Pi_b \\
    &= \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \star \\
        \vdots & \vdots & \vdots \\
        0 & \mbf{0}_n ^\top &
        \frac{\mu}{c} \sum_{i: \alpha_i \preceq \beta_i} \beta_i ^\top
    \end{bmatrix}
    + \begin{bmatrix} 0 & \mbf{0}_n ^\top & \star \\ 
    \vdots & \vdots & \vdots \\
    0 & \mbf{0}_n ^\top & 
    \mu \zeta^\top X \Pi_b ^\top \end{bmatrix}
\end{align*}
We conclude by bounding the residual term:
\begin{align*}
    \norm{\mu \Pi_b X ^\top \zeta}_\infty
    = \mu \norm{\Pi_b X ^\top \zeta}_\infty
    \leq \mu \norm{\mbf{1}_n \mbf{1}_N ^\top \zeta}_\infty
    \leq \mu N \norm{\zeta}_\infty
    \leq \mu N^2 e^{-\lambda}
    \leq \mu^3 e^{-\lambda}
    < 1/3
\end{align*}
where recall that \(X\) is a binary-valued matrix and \(N \leq \mu\).
\end{proof}


%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
\label{lem:reasoning_approx}
Take the definitions as in Theorem~\ref{thm:reasoning} and its proof, then:
\begin{align*}
    \braces*{
        j \in \{1, \ldots, n\} :
        \parens*{
            \beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i: \alpha_i \preceq \beta_N} \beta_i
            + \varepsilon
        }_j > 2/3
    }
    &=\big\{
        j \in \{1, \ldots, n\} : 
        \Gamma(s_{t})_j = 1
    \big\}
    \\
    \braces*{
        j \in \{1, \ldots, n\} :
        \parens*{
            \beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i: \alpha_i \preceq \beta_N} \beta_i
            + \varepsilon
        }_j < 1/3
    }
    &=\big\{
        j \in \{1, \ldots, n\} : 
        \Gamma(s_{t})_j = 0
    \big\}
\end{align*}
\end{lemma}
\begin{proof}
We first analyze the coordinates of \(\Gamma(s_{t})\) that are ones:
\begin{align*}
    \braces*{j:
        \Gamma(s_{t})_j = 1}
    &= \braces*{j :
        \parens*{s_{t} + \sum_{(\alpha, \beta) \in \Gamma: \alpha \preceq s_{t}} \beta
        }_j \geq 1
    } \\
    &= \braces*{j:
        \parens*{\beta_N +
        \sum_{(\alpha, \beta) \in \Gamma: \alpha \preceq s_{t}} \beta
        + \sum_{k = 0}^{t} s_k
        }_j \geq 1
    }
    \tag{\(\beta_N = s_{t}\) and \(s_0 \preceq \cdots \preceq s_{t}\)} \\
    &= \braces*{j:
        \parens*{\beta_N + \sum_{i: \alpha_i \preceq \beta_N} \beta_i
        }_j \geq 1
    }
    \tag{\(\alpha_{r + k - 1} = \mbf{0}_n\) and \(\beta_{r + k - 1} = s_k\) for \(k = 0, \ldots, t\)} \\
    &= \braces*{j:
        \parens*{\beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i : \alpha_i \preceq \beta_N} \beta_i
        }_j \geq 1
    }
    \tag{\(\mu \geq N \geq \abs{\{i: \alpha_i \preceq \beta_N\}}\)}
\end{align*}
Similarly, observe that:
\begin{align*}
    \braces*{j: \Gamma(s_{t})_j = 0}
    = \braces*{j:
        \parens*{\beta_N + \frac{\mu}{\abs{\{i: \alpha_i \preceq \beta_N\}}} \sum_{i : \alpha_i \preceq \beta_N} \beta_i}_j = 0
    }
\end{align*}
We then apply \(\norm{\varepsilon}_\infty < 1/3\) to conclude the desired result.
\end{proof}




==> old/old_theory/theory_two_layer/two_layer_attack.tex <==
\subsection{Results for Adversarial Attacks}



\begin{theorem} \label{thm:attack}
Let \(U \in \mbb{R}^{N \times d}\) be the tokenized input of any set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and states \(s_0, \ldots, s_{t-1} \in \mbb{B}^n\) such that each \(s_{k+1} = \Gamma(s_k)\).
For any \(v_{\msf{tgt}} \in \mbb{B}^n\) and any \(\lambda_{\msf{atk}} > \red{XXX}\), define
\begin{align*}
    u_{\msf{atk}} =
    \begin{bmatrix}
        0 & \mbf{0}_n ^\top & \lambda_{\msf{atk}} (2 v_{\msf{tgt}} - \mbf{1}_n)^\top
    \end{bmatrix}
    \in \mbb{R}^{1+2n}
\end{align*}
Let \(N = r + t + 1\) be the length of the adversarial sequence \(\msf{stack}(U, u_{\msf{atk}})\).
Fix any parameters \(\delta, \rho, \lambda\) as in Theorem~\ref{thm:one_step}, where note that \(\rho \geq r + t + 1\).
Then, for \(\msf{LM} : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^{n}\) as defined in \red{(X)}, we have
\(v_{\msf{tgt}} = \msf{LM}(\msf{stack}(U, u_{\msf{atk}}))\).
\end{theorem}
\begin{proof}
The main idea is to treat \(u_{\msf{atk}}\) as the tokenization of the rule \((\mbf{0}_n, \beta_{\msf{atk}})\), where \(\beta_{\msf{atk}} = \lambda_{\msf{atk}} (2 v_{\msf{tgt}} - \mbf{1}_n))\).
Note that \((\mbf{0}_n, \beta_{\msf{atk}})\) is technically not a valid rule since the \(\beta_{\msf{atk}}\) is not binary-valued.
However, we may still feed the sequence \(\msf{stack}(U, u_{\msf{atk}})\) into \(\msf{LM}\),
which recall consists of the following modules:
\begin{align*}
    \msf{LM}
    = \big(\msf{ClsHead} \circ \underbrace{(\msf{Layer}_2 \circ \msf{Layer}_1)}_{\msf{Tf}} \circ \msf{Embed} \big)
    : \mbb{R}^{N \times d_{\msf{in}}} \to \mbb{R}^n
\end{align*}
We therefore begin with the \(\msf{Layer}_1 \circ \msf{Embed}\) part:
\begin{align} \label{eqn:attack_stack}
    \msf{stack}(U, u_{\msf{atk}})
    % = \begin{bmatrix}
    %     \msf{Tokenize}(\gamma_1) \\
    %     \vdots \\
    %     \msf{Tokenize}(\gamma_r) \\
    %     \msf{Tokenize}(s_0) \\
    %     \vdots \\
    %     \msf{Tokenize}(s_{t-1}) \\
    %     u_{\msf{atk}}
    % \end{bmatrix}
    \xrightarrow{\msf{Embed}}
    X =
    \begin{bmatrix}
       0 & \alpha_1 ^\top & \beta_1 ^\top & \mbf{0}_n ^\top \\
       \vdots & \vdots & \vdots & \vdots \\
       0 & \alpha_r ^\top & \beta_r ^\top & \mbf{0}_n ^\top \\
       1 & \mbf{0}_n ^\top & s_0 ^\top & \mbf{0}_n ^\top \\
       \vdots & \vdots & \vdots & \vdots \\
       1 & \mbf{0}_n ^\top & s_{t-1} ^\top & \mbf{0}_n ^\top \\
       0 & \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top & \mbf{0}_n ^\top
    \end{bmatrix}
    \xrightarrow[\text{Lemma~\ref{lem:layer1}}]{\msf{Layer}_1}
    X' =
    \begin{bmatrix}
       0 & \alpha_1 ^\top & \beta_1 ^\top & w_1 ^\top \\
       \vdots & \vdots & \vdots & \vdots \\
       0 & \alpha_r ^\top & \beta_r ^\top & w_r ^\top \\
       1 & \mbf{0}_n ^\top & s_0 ^\top & w_{r+1} ^\top \\
       \vdots & \vdots & \vdots & \vdots \\
       1 & \mbf{0}_n ^\top & s_{t-1} ^\top & w_{N-1} ^\top \\
       0 & \mbf{0}_n ^\top & \beta_{\msf{atk}} ^\top & s_{t-1} ^\top
    \end{bmatrix}
\end{align}
where \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\) are some outputs of \(\msf{Layer}_1\).
The above demonstrates that the \(\msf{Layer}_1\) behaves as expected even with the adversarially suffixed sequence \(\msf{stack}(U, u_{\msf{atk}})\).

Next, we analyze the action of \(\msf{Layer}_2\), for which we adapt the proof of Lemma~\ref{lem:layer2} and inherit all notation for convenience.
For brevity, we skip to the following expression, which resembles that of~\eqref{eqn:atten2_sigmas_subst}:
\begin{align*}
    \msf{Attn}_2 (X')
    = \frac{\rho}{c} e_N h^\top X' \Pi_b ^\top \Pi_c
    + e_N \underbrace{
        \frac{\rho}{c} X' \Pi_b ^\top
    }_{\zeta}
    \Pi_c
    + \sum_{i = 1}^{N-1} e_i \sigma_i ^\top X' \rho \Pi_b ^\top \Pi_c
\end{align*}
with \(\norm{\zeta}_\infty \leq \rho^3 e^{-\lambda}\).
However, the expression \(h^\top X' \Pi_b\) is different from that of~\eqref{eqn:layer2_hXPib}, and instead expands as:
\begin{align} \label{eqn:attack_hXPib}
    h^\top X' \Pi_b
    = s_0 ^ \top + \cdots + s_{t-1} ^\top
    + \beta_+ ^\top
    + \beta_{\msf{atk}},
    \qquad
    \beta_+ ^\top = \sum_{(\alpha, \beta): \alpha \preceq s_{t-1}} \beta ^\top    
\end{align}
because the antecedent of the rule \((\mbf{0}_n, \beta_{\msf{atk}})\) is always subsumed by \(s_{t-1}\).
As a consequence, the action of \(\msf{Id} + \msf{Attn}_2\) on \(X'\) as in~\eqref{eqn:attack_stack} is described as:
\begin{align} \label{eqn:attack_idattn}
    X' = \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}_2}
    \begin{bmatrix}
        z_1 ^\top & \sigma_1 ^\top X' \rho \Pi_b ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \sigma_{N-1} ^\top X' \rho \Pi_b ^\top \\
        z_N ^\top & s_{t-1} ^\top + (\rho/c)(s_0 + \cdots + s_{t-1} + \beta_+ + \beta_{\msf{atk}})^\top + \zeta^\top
    \end{bmatrix}
\end{align}
which is similar to that of~\eqref{eqn:layer2_idattn}, except the \(N\)th row on the RHS has an additional \(\beta_{\msf{atk}}\) term.
Importantly, observe that:
\begin{align*}
    (s_{t-1} + (\rho/c)(s_0 + \cdots + s_{t-1} + \beta_+ + \beta_{\msf{atk}}) + \zeta)_i
    \quad \begin{dcases}
        > 1 - \delta, & v_{\msf{tgt}} = 1 \\
        < \delta, & v_{\msf{tgt}} = 0
    \end{dcases},
    \qquad \text{for all \(i = 1, \ldots, n\).}
\end{align*}
Consequently, the \(N\)th row of the \eqref{eqn:attack_idattn} RHS is mapped as:
\begin{align} \label{eqn:attack_idffwd}
    \begin{bmatrix}
        z_N \\
        s_{t-1} + (\rho/c)(s_0 + \cdots + s_{t-1} + \beta_+ + \beta_{\msf{atk}}) + \zeta
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}_2}
    \begin{bmatrix}
        z_N \\ v_{\msf{tgt}}
    \end{bmatrix}
\end{align}
In summary, the evaluation of \(\msf{LM}(\msf{stack}(U, u_{\msf{atk}}))\) is decomposed as follows:
\begin{align*}
    \msf{stack}(U, u_{\msf{atk}})
    \xrightarrow[\eqref{eqn:attack_stack}]{\msf{Embed}}
    \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \mbf{0}_n ^\top \\
        z_N ^\top & \mbf{0}_n ^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:attack_stack}]{\msf{Layer}_1}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:attack_idattn},\eqref{eqn:attack_idffwd}]{\msf{Layer}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^{\prime\top} \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^{\prime\top} \\
        z_N ^\top & v_{\msf{tgt}} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{ClsHead}}
    v_{\msf{tgt}}
\end{align*}
where \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\) and \(w_1 ', \ldots, w_{N-1} ' \in \mbb{R}^{n}\) are some outputs of \(\msf{Layer}_1\) and \(\msf{Layer}_2\), respectively.
\end{proof}



==> old/old_theory/theory_two_layer/two_layer_constructions.tex <==

\subsection{Transformer Construction}
\label{sec:tf_construction}


\begin{align} \label{eqn:appendix_tf_layer}
    \msf{Layer}_k (X)
        = ((\msf{Id} + \msf{Ffwd}_k) \circ (\msf{Id} + \msf{Attn}_k))(X)
\end{align}
where \(\msf{Id}\) is the identity block that implements a residual connection.
The same feedforward block \(\msf{Ffwd}_k : \mbb{R}^{d} \to \mbb{R}^{d}\) is applied in parallel to each term of the \(N\)-length sequence.
Moreover, the feedforward block of each layer is only 1-hidden unit deep and so takes the form:
\begin{align} \label{eqn:tf_ffwd}
    \msf{Ffwd}_k (x)
    = W_{k2} \sigma (W_{k1} x + b_{k1}) + b_{k2},
\end{align}
with parameters \(W_{k1}, W_{k2}^{\top} \in \mbb{R}^{d_{\msf{ffwd}} \times d}\), \(b_{k1} \in \mbb{R}^{d_{\msf{ffwd}}}\), and \(b_{k2} \in \mbb{R}^{d}\), and \(\sigma\) is some activation function that we assume to be \(\msf{ReLU}\).
Here \(d_{\msf{ffwd}}\) is the feedforward width that is commonly taken to be \(d_{\msf{ffwd}} = 4d\) or some large constant.
An attention block \(\msf{Attn}_k : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) with \(H\) heads with causal attention has form:
\begin{gather*}
    \msf{Attn}_k (X) = \sum_{h = 1}^{H} \msf{CausalSoftmax}(Q_{kh} K_{kh} ^\top) V_{kh} \\
    Q_{kh} = X W_{Qkh},
    \quad K_{kh} ^\top = W_{Kkh} ^\top X^\top,
    \quad V_{kh} = X W_{Vkh}
\end{gather*}
with parameters \(W_{Qkh}, W_{Kkh} ^\top \in \mbb{R}^{d \times d_{\msf{attn}}}\) and \(W_{Vkh} \in \mbb{R}^{d \times d}\) for heads \(h = 1, \ldots, H\).
Note that it suffices to take \(d_{\msf{attn}} \leq d\).
Here, \(\msf{CausalSoftmax}: \mbb{R}^{N \times N} \to \mbb{R}^{N \times N}\) is the causal variant of row-wise softmax defined as follows:
\begin{align*}
    \msf{CausalSoftmax}(Z)
    &= \begin{bmatrix}
        \msf{Softmax}( z_{11}, & -\infty, & \cdots, & -\infty) \\
        \msf{Softmax}( z_{21}, & z_{22}, & \cdots, & -\infty) \\
        \vdots & \vdots & \ddots & \vdots \\
        \msf{Softmax}( z_{N1}, & z_{N2}, & \cdots, & z_{NN})
    \end{bmatrix}
\end{align*}
where \(z_{ij}\) is the \((i,j)\)th entry of the parameter \(Z \in \mbb{R}^{N \times N}\) and \(\msf{Softmax} : \mbb{R}^{N} \to \mbb{R}^{N}\) is given as:
\begin{align*}
    \msf{Softmax}(a_1, \ldots, a_N)
    &= \frac{\parens*{e^{a_1}, \ldots, e^{a_N}}}{e^{a_1} + \cdots + e^{a_N}}
    \in \mbb{R}^{N}
\end{align*}
Observe that \(-\infty\) to an argument of \(\msf{Softmax}\) makes the corresponding position zero.
\(\msf{CausalSoftmax}(Z)\) is thus a lower-triangular matrix with zeros strictly above the diagonal, i.e., \(\msf{CausalSoftmax}(Z)_{ij} = 0\) iff \(j > i\).
Note that our formalism omits the layer normalization, which is typically applied after each attention block and after each feedforward block.
This omission does not change the fundamental expressive power of a transformer~\cite{liu2022transformers} and serves to simplify the theoretical analysis.
Moreover, although the transformer must fix apriori various quantities like \(d, d_{\msf{ffwd}}, d_{\msf{attn}}\), the sequence may be of any length \(N\) --- though in practice there is often an upper bound \(N_{\msf{max}} \geq N\) due to limitations in the choice of positional encoding.


\begin{align} \label{eqn:tf_appendix}
    \msf{Tf}(X) = \big(
        \underbrace{((\msf{Id} + \msf{Ffwd}_2) \circ (\msf{Id} + \msf{Attn}_2))}_{\msf{Layer}_2}
        \circ
        \underbrace{((\msf{Id} + \msf{Ffwd}_1) \circ (\msf{Id} + \msf{Attn}_1))}_{\msf{Layer}_1}
    \big)
    (X)
\end{align}

\begin{align} \label{eqn:attn1}
\begin{split}
    \msf{Attn}_1 (X)
    &= \msf{CausalSoftmax}(\lambda X \Pi_{\msf{hot}} ^\top \Pi_{\msf{s}} X^\top) X \rho \Pi_b ^\top \Pi_c \\
    W_Q &= \lambda \Pi_{\msf{hot}} ^\top,
    \quad W_K = \Pi_{\msf{s}} ^\top,
    \quad W_V = \rho \Pi_b^\top \Pi_c
\end{split}
\end{align}


\begin{align} \label{eqn:attn2}
\begin{split}
    \msf{Attn}_2 (X)
    &= \msf{CausalSoftmax}(\lambda X (\Pi_c - \mbf{1}_n \Pi_{\msf{hot}})^\top \Pi_a X^\top) X \rho \Pi_b ^\top \Pi_c \\
    W_Q &= \lambda (\Pi_c - \mbf{1}_n \Pi_{\msf{hot}})^\top,
    \quad W_K = \Pi_a ^\top,
    \quad W_V = \rho \Pi_b ^\top \Pi_c
\end{split}
\end{align}


==> old/old_theory/theory_two_layer/two_layer_logic.tex <==
\subsection{Results for Autoregressive Propositional Inference}



\begin{theorem} [\(\msf{TF}\)]
\label{thm:one_step}
Consider any set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and states \(s_0, \ldots, s_{t-1} \in \mbb{B}^n\) such that each \(s_{k+1} = \Gamma(s_k)\).
Let \(X \in \mbb{R}^{N \times d}\) be the embedded inputs as in \red{(X)} with sequence length \(N = r + t\) and embedding dimension \(d = 2 + 3n\).
Fix any \(0 \leq \delta < 1/3\), \(\rho \geq N\), and \(\lambda > \log(\rho ^3 / \delta)\).
Then, for \(\msf{Tf} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) as defined in~\eqref{eqn:tf_appendix}, we have:
\begin{align*}
    X = \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \mbf{0}_n ^\top \\
        z_N ^\top & \mbf{0}_n ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_1}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^{\prime \top} \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^{\prime \top} \\
        z_N ^\top & \Gamma(s_{t-1}) ^\top
    \end{bmatrix}
    = Y
\end{align*}
for some \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\) and \(w_1', \ldots, w_{N-1}' \in \mbb{R}^{n}\) that are outputs of \(\msf{Layer}_1\) and \(\msf{Layer}_2\), respectively.


\end{theorem}
\begin{proof}
First apply Lemma~\ref{lem:layer1} for \(\msf{Layer}_1\), then apply Lemma~\ref{lem:layer2} for \(\msf{Layer}_2\). 
\end{proof}

% Let \(n \geq 1\) be the number of atoms, \(r \geq 1\) be the number of rules, and \(t \geq 1\) be the number of states.
% Consider any tolerance \(0 \leq \delta < 1/3\) and scaling factors \(\rho \geq r + t\) and \(\lambda > \log(\rho ^3 / \delta)\).
% Let \(N = r + t\) be the input sequence length, then for \(\msf{Tf} : \mbb{R}^{N \times d} \to \mbb{R}^{N \times d}\) as defined in~\eqref{eqn:tf_appendix} we have:
% where \(X\) is the embedded input of any rule set \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and states \(s_0, \ldots, s_{t-1} \in \mbb{B}^n\) such that \(s_{k+1} = \Gamma(s_k)\),
% and where \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\) and \(w_1 ', \ldots, w_{N-1} ' \in \mbb{R}^{n}\) are some outputs of \(\msf{Layer}_1\) and \(\msf{Layer}_2\), respectively.



\begin{lemma}[\(\msf{Layer}_1\)]
\label{lem:layer1}
Take the definitions as in Theorem~\ref{thm:one_step}.
Then, for some \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\):
\begin{align*}
    \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \mbf{0}_n ^\top \\
        z_N ^\top & \mbf{0}_n ^\top \\
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_1}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top \\
    \end{bmatrix}
\end{align*}
\end{lemma}
\begin{proof}
We expand \(\msf{Attn}_1 (X)\) as follows:
\begin{align} \label{eqn:attn1_sigmas}
    \msf{Attn}_1 (X)
    = \msf{CausalSoftmax}(\lambda X \Pi_{\msf{hot}} ^\top \Pi_{\msf{s}} X^\top) X \rho \Pi_b ^\top \Pi_c
    = \sum_{i = 1}^{N} e_i \sigma_i ^\top X \rho \Pi_b ^\top \Pi_c
\end{align}
where \(e_1, \ldots, e_N \in \mbb{R}^{N}\) are the basis vectors and \(\sigma_1, \ldots, \sigma_N \in \mbb{R}^{N}\) are the rows of \(\msf{CausalSoftmax}(\ldots)\).
We focus on the \(N\)th row, because that is where the \(s_{t-1}\) term will be written, and accordingly analyze the \(\sigma_N\) term:
\begin{align*}
    \sigma_N
    &= \msf{Softmax}(\lambda x_N ^\top \Pi_{\msf{hot}} ^\top \Pi_{\msf{s}} x_1, \ldots, \lambda x_N ^\top \Pi_{\msf{hot}} ^\top \Pi_{\msf{s}} x_N) \\
    &= \msf{Softmax}(\lambda \Pi_{\msf{s}} x_1, \ldots, \lambda \Pi_{\msf{s}} x_N)
        \tag{\(\Pi_{\msf{hot}} x_i = 1\) for all \(i = 1, \ldots, N\)} \\
    &= \frac{1}{\abs{\{i : \Pi_{\msf{s}} x_i = 1\}}}
        \varphi + \varepsilon
    \tag{Lemma~\ref{lem:layer1_softmax} with \(\varphi = X \Pi_{\msf{s}} ^\top \in \mbb{B}^N\)}
\end{align*}
where \(t = \abs{\{i : \Pi_{\msf{s}} x_i = 1\}}\) due to the presence of \(s_0, \ldots, s_{t-1}\) and
\(\norm{\varepsilon}_{\infty} \leq N e^{-\lambda} \leq \rho e^{-\lambda}\) by Lemma~\ref{lem:layer1_softmax}.
We use this to separate out the \(N\)th summation term of~\eqref{eqn:attn1_sigmas} and rewrite:
\begin{align} \label{eqn:attn1_sigmas_subst}
    \msf{Attn}_1 (X)
        &= \frac{\rho}{t} e_N \varphi^\top X \Pi_b ^\top \Pi_c +  e_N \underbrace{\rho\varepsilon^\top X \Pi_b ^\top}_{\zeta} \Pi_c
        + \sum_{i = 1}^{N-1} e_i \sigma_i ^\top X \rho \Pi_b ^\top \Pi_c
\end{align}
where note that \(\varphi^\top X \Pi_b = s_0 ^\top + \cdots + s_{t-1} ^\top\) since \(\varphi_i = 1\) iff row \(i\) of \(X\) encodes a state.
Using~\eqref{eqn:attn1_sigmas_subst}, we may express the action of \(\msf{Id} + \msf{Attn}_1\) as follows:
\begin{align} \label{eqn:layer1_idattn}
    X
    = \begin{bmatrix}
        z_1 & \mbf{0}_n \\
        \vdots & \vdots \\
        z_{N-1} & \mbf{0}_n \\
        z_N & \mbf{0}_n
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}_1}
    \begin{bmatrix}
        z_1 ^\top & \sigma_1 ^\top X \rho \Pi_b ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \sigma_{N-1} ^\top X \rho \Pi_b ^\top \\
        z_{N} ^\top & (\rho/t) (s_0 + \cdots + s_{t-1})^\top + \zeta^\top
    \end{bmatrix}
\end{align}
Next, we bound the residual term \(\zeta\) to analyze the action of \(\msf{Id} + \msf{Ffwd}_1\).
In particular, recall that \(\norm{\varepsilon}_\infty \leq \rho e^{-\lambda}\), so when \(\lambda > \log(\rho^3 / \delta)\) we have:
\begin{align*}
    \norm{\zeta}_{\infty}
    \leq \rho \norm*{\Pi_b X^\top \varepsilon}_{\infty}
    \leq \rho \norm{\mbf{1}_N \mbf{1}_N ^\top \varepsilon}_{\infty}
    \leq \rho N \norm{\varepsilon}_{\infty}
    \leq \rho^3 e^{-\lambda}
    < \delta
\end{align*}
Thus, because \(\rho / t \geq 1\) and \(s_0 + \ldots + s_{t-1} \in \mbb{Z}_{\geq 0} ^n\), we have for the \(N\)th row of the~\eqref{eqn:layer1_idattn} RHS:
\begin{align} \label{eqn:layer1_idffwd}
    \begin{bmatrix}
        z_N \\
        (\rho/t) (s_0 + \cdots + s_{t-1}) + \zeta
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}_1}
    \begin{bmatrix}
        z_N \\
        s_0 \lor \cdots \lor s_{t-1}
    \end{bmatrix}
    = \begin{bmatrix} z_N \\ s_{t-1} \end{bmatrix}
    \in \mbb{B}^d
\end{align}
since the LHS is either \(< \delta\) or \(> 1 - \delta\).
Specifically, we used the property that sum-then-binarize implements binary disjunctions and the fact that each \(s_{k+1} \succeq s_k\) due to \(s_{k+1} = \Gamma(s_k)\).
All together, composing the mappings of \(\msf{Id} + \msf{Attn}_1\) with \(\msf{Id} + \msf{Ffwd}_1\) yields:
\begin{align*}
    X = \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \mbf{0}_n ^\top \\
        z_{N} ^\top & \mbf{0}_n ^\top \\
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:layer1_idattn}]{\msf{Id} + \msf{Attn}_1}
    \begin{bmatrix}
        z_1 ^\top & \sigma_1 ^\top X \rho \Pi_b ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & \sigma_{N-1} ^\top X \rho \Pi_b ^\top \\
        z_{N} ^\top & (\rho/t) (s_0 + \cdots + s_{t-1})^\top + \zeta^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:layer1_idffwd}]{\msf{Id} + \msf{Ffwd}_1}
    \begin{bmatrix}
        z_1 ^\top & w_1^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_{N} ^\top & s_{t-1} ^\top
    \end{bmatrix}
\end{align*}
for some \(w_1, \ldots, w_{N-1} \in \mbb{R}^{n}\).
\end{proof}



\begin{lemma} \label{lem:layer1_softmax}
Consider any \(\varphi \in \mbb{B}^N\) where \(t = \abs{\{i : \varphi_i = 1\}} \geq 1\).
For any \(\lambda > 0\), let \(\varepsilon = \msf{Softmax}(\lambda \varphi) - (\varphi/t)\), then \(\norm{\varepsilon}_\infty \leq (N - t) e^{-\lambda}\).
\end{lemma}
\begin{proof}
Note that if \(t = N\), then \(\norm{\varepsilon}_\infty = 0\), so we assume \(t < N\).
We first consider some \(i\) for which \(\varphi_i = 0\),
\begin{align*}
    \abs{\varepsilon_i} = \frac{1}{t e^{\lambda} + N - t}
    \leq \frac{1}{t e^{-\lambda}}
    \leq e^{-\lambda}
\end{align*}
Next, consider some \(i\) for which \(\varphi_i = 1\),
\begin{align*}
    \abs{\varepsilon_i} = \frac{1}{t} - \frac{e^{\lambda}}{t e^{\lambda} + N - t}
    \leq \frac{N - t}{t^2 e^\lambda + t (N-t)}
    \leq \frac{N - t}{t^2 e^\lambda}
    \leq (N - t) e^{-\lambda}
\end{align*}
Since \(e ^{-\lambda} \leq (N - t) e^{-\lambda}\), our desired inequality follows.
\end{proof}



\begin{lemma}[\(\msf{Layer}_2\)]
\label{lem:layer2}
Take the definitions as in Theorem~\ref{thm:one_step}.
Then, for some \(w_1 ', \ldots, w_{N-1} ' \in \mbb{R}^{n}\):
\begin{align*}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^{\prime\top} \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^{\prime\top} \\
        z_N ^\top & \Gamma(s_{t-1}) ^\top
    \end{bmatrix}
\end{align*}
\end{lemma}
\begin{proof}
The proof is similar to that of Lemma~\ref{lem:layer1}.
Let \(X' = \msf{Layer}_1 (X)\), and expand \(\msf{Attn}_2 (X')\) as follows:
\begin{align} \label{eqn:attn2_sigmas}
    \msf{Attn}_2 (X')
    = \msf{CausalSoftmax}(\lambda X' (\Pi_c - \mbf{1}_n \Pi_{\msf{hot}})^\top \Pi_a X^{\prime\top}) X' \rho \Pi_b ^\top \Pi_c
    = \sum_{i = 1}^{N} e_i \sigma_i ^\top X' \rho \Pi_b ^\top \Pi_c
\end{align}
where \(e_1, \ldots, e_N \in \mbb{R}^{N}\) are the basis vectors and \(\sigma_1, \ldots, \sigma_N \in \mbb{R}^{N}\) are the rows of \(\msf{CausalSoftmax}(\ldots)\).
Again, we will focus on the \(\sigma_N\) term, which we rewrite as:
\begin{align*}
    \sigma_N &= \msf{Softmax}(\lambda x_N ^{\prime\top} (\Pi_c - \mbf{1}_n \Pi_{\msf{hot}})^\top \Pi_a x_1 ',
    \ldots,
    \lambda x_N ^{\prime\top} (\Pi_c - \mbf{1}_n \Pi_{\msf{hot}})^\top \Pi_a x_N ') \\
    &= \msf{Softmax}(\lambda (s_{t-1} - \mbf{1}_n)^\top \alpha_1,
    \ldots,
    \lambda(s_{t-1} - \mbf{1}_n)^\top \alpha_N)
    \tag{\(\alpha_i = \Pi_a x_i '\) for all \(i = 1, \ldots, N\)}
\end{align*}
where recall that \(s_{t-1} = \Pi_c x_N '\).
In an abuse of notation, we write \(\alpha_1, \ldots, \alpha_N\) to mean the antecedents of rows \(i = 1, \ldots, N\) because our tokenization and embedding scheme treats proof states as rules with empty antecedents, i.e., if \(x_i\) embeds a proof state, then \(\alpha_i = \mbf{0}_n\).
In particular, \((s_{t-1} - \mbf{1}_n)^\top \alpha_i \in \mbb{Z}_{\leq 0}\) is such that:
\begin{align*}
    (s_{t-1} - \mbf{1}_n)^\top \alpha_i
    \quad
    \begin{dcases}
        = 0, & \alpha_i \preceq s_{t-1} \\
        < 0, & \text{otherwise}
    \end{dcases},
    \qquad \text{for all \(i = 1, \ldots, N\).}
\end{align*}
We then apply Lemma~\ref{lem:layer2_softmax} to rewrite \(\sigma_N\) as follows:
\begin{align*}
\sigma_N = \frac{1}{c}
    \varphi + \varepsilon,
    \qquad
    \varphi = (\alpha_1 \preceq s_{t-1}, \ldots, \alpha_N \preceq s_{t-1}) \in \mbb{B}^N,
    \qquad
    c = \abs{\{i : \alpha_i \preceq s_i\}}
\end{align*}
where \(\norm{\varepsilon}_{\infty} \leq N e^{-\lambda} \leq \rho e^{-\lambda}\).
Substituting this expression of \(\sigma_N\) into~\eqref{eqn:attn2_sigmas} yields:
\begin{align} \label{eqn:atten2_sigmas_subst}
    \msf{Attn}_2 (X')
    = \frac{\rho}{c} e_N \varphi^\top X' \Pi_b ^\top \Pi_c
    + e_N \underbrace{
        \rho \varepsilon^\top X' \Pi_b ^\top
    }_{\zeta}
    \Pi_c
    + \sum_{i = 1}^{N-1} e_i \sigma_i ^\top X' \rho \Pi_b ^\top \Pi_c
\end{align}
Importantly, \(\varphi_i = 1\) iff the row \(x_i\) embeds either a proof state or a rule \((\alpha, \beta)\) with \(\alpha \preceq s_{t-1}\), which implies that:
\begin{align} \label{eqn:layer2_hXPib}
    \varphi^\top X' \Pi_b
    = s_0 ^ \top + \cdots + s_{t-1} ^\top
    + \beta_+ ^\top,
    \qquad
    \beta_+ ^\top = \sum_{(\alpha, \beta): \alpha \preceq s_{t-1}} \beta ^\top
\end{align}
Similar to Lemma~\ref{lem:layer1}, we use~\eqref{eqn:atten2_sigmas_subst} and~\eqref{eqn:layer2_hXPib} to summarize the action of \(\msf{Id} + \msf{Attn}_2\) as follows:
\begin{align} \label{eqn:layer2_idattn}
    X' = \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top + \sigma_1^\top X' \rho \Pi_b ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top + \sigma_{N-1}^\top X' \rho \Pi_b ^\top \\
        z_N ^\top & s_{t-1} ^\top + (\rho/c)(s_0 + \cdots + s_{t-1} + \beta_+)^\top + \zeta^\top
    \end{bmatrix}
\end{align}
Next, we bound the residual term \(\zeta\) in order to analyze \(\msf{Id} + \msf{Ffwd}_2\).
Recall from above that \(\norm{\varepsilon}_\infty \leq \rho e^{-\lambda}\), so when \(\lambda > \log(\rho^3 / \delta)\) we have:
\begin{align*}
    \norm{\zeta}_{\infty}
    \leq \rho \norm*{\Pi_b X^{\prime\top} \varepsilon}_\infty
    \leq \rho \norm{\mbf{1}_N \mbf{1}_N ^\top \varepsilon}_\infty
    \leq \rho N \norm{\varepsilon}_\infty
    \leq \rho^3 e^{-\lambda}
    < \delta
\end{align*}
Thus, because \(\rho / c \geq 1\) and \(s_0 + \cdots + s_{t-1} + \beta_+ \in \mbb{Z}_{\geq 0}^n\), we have for the \(N\)th row of the \eqref{eqn:layer2_idattn} RHS:
\begin{align} \label{eqn:layer2_idffwd}
    \begin{bmatrix}
        z_N \\
        s_{t-1} + (\rho/c) (s_0 + \cdots + s_{t-1} + \beta_+) + \zeta
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}_2}
    \begin{bmatrix}
        z_N \\
        s_{t-1} \lor \bigvee\{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s_{t-1}\}
    \end{bmatrix}
    = \begin{bmatrix} z_N \\ \Gamma(s_{t-1}) \end{bmatrix}
    \in \mbb{B}^{d}
\end{align}
since each term of the LHS is either \(< \delta\) or \(> 1 - \delta\), and also because \(s_{t-1} = s_0 \lor \cdots \lor s_{t-1}\).
Like in Lemma~\ref{lem:layer1}, we used the property that sum-then-binarize implements binary disjunctions and the fact that \(s_{k+1} \succeq s_k\) by \(s_{k+1} = \Gamma(s_k)\).
In summary, composing the mappings of \(\msf{Id} + \msf{Attn}_2\) with \(\msf{Id} + \msf{Ffwd}_2\) yields:
\begin{align*}
    X' =
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:layer2_idattn}]{\msf{Id} + \msf{Attn}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^\top + \sigma_1^\top X' \rho \Pi_b ^\top \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^\top + \sigma_{N-1}^\top X' \rho \Pi_b ^\top \\
        z_N ^\top & s_{t-1} ^\top + (\rho/c)(s_0 + \cdots + s_{t-1} + \beta_+)^\top + \zeta^\top
    \end{bmatrix}
    \xrightarrow[\eqref{eqn:layer2_idffwd}]{\msf{Id} + \msf{Ffwd}_2}
    \begin{bmatrix}
        z_1 ^\top & w_1 ^{\prime\top} \\
        \vdots & \vdots \\
        z_{N-1} ^\top & w_{N-1} ^{\prime\top} \\
        z_N ^\top & s_t ^\top
    \end{bmatrix}
\end{align*}
for some \(w_1', \ldots, w_{N-1} ' \in \mbb{R}^{n}\), where \(s_t = \Gamma(s_{t-1})\).
\end{proof}





\begin{lemma} \label{lem:layer2_softmax}
Consider any \(w \in \mbb{Z}_{\leq 0} ^N\) where \(c = \abs{\{i : w_i = 0\}} \geq 1\).
For any \(\lambda > 0\), let \(\varepsilon = \msf{Softmax}(\lambda w) - (\varphi/c)\) where \(\varphi = \mbb{I}[w = 0] \in \mbb{B}^N\), then \(\norm{\varepsilon}_\infty \leq (N-c) e^{-\lambda}\).
\end{lemma}
\begin{proof}
Note that if \(c = N\), then \(\norm{\varepsilon}_\infty = 0\), so we assume \(c < N\).
First consider some \(i\) for which \(w_i < 0\),
\begin{align*}
    \abs{\varepsilon_i}
    = \frac{e^{\lambda w_i}}{c + \sum_{i : w_i < 0} e^{\lambda g_i}}
    \leq e^{\lambda w_i}
    \leq e^{-\lambda}
\end{align*}
Next, consider some \(i\) for which \(w_i = 0\),
\begin{align*}
    \abs{\varepsilon_i}
    = \frac{1}{c} - \frac{1}{c + \sum_{i : w_i < 0} e^{\lambda w_i}}
    \leq \frac{\sum_{i : w_i < 0} e^{\lambda w_i}}{c^2 + c \sum_{i : w_i < 0} e^{\lambda w_i}}
    \leq \sum_{i : w_i < 0} e^{\lambda w_i}
    \leq (N - c) e^{-\lambda}
\end{align*}
Because \(e^{-\lambda} \leq (N - c) e^{-\lambda}\), the desired inequality follows.
\end{proof}




==> old/q1.tex <==
\begin{figure}[ht]
\centering



\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns1.png}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns2.png}
\end{minipage}%
\begin{minipage}{0.32\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{images/exp_plots/exp1/grid_ns3.png}
\end{minipage}%



% % \includegraphics[width=0.95\linewidth]{images/exp_plots/exp1_seed101_plot.png}
% \includegraphics[width=0.95\linewidth]{images/exp_plots/exp1/exp1_l1_plot.png}


\caption{
A reasoner needs embedding dimension linear in the problem size.
We fix \(L=1\) layers and \(H=1\) heads according to our theory and vary the embedding dimension \(d\) and the number of propositions \(n\).
Near-perfect accuracy (\(\geq 0.99\)) is attained when \(d \geq 4n\). The accuracies are rounded up to two decimal places.
% The mean accuracy across three runs is reported.
% The embedding dimension \(d\) and the number of propositions \(n\) demonstrate a linear trend with respect to the mean validation accuracy as suggested by Theorem~\ref{thm:main_result_sketch}. 
% An \((n, d)\) entry here represents the validation accuracy of a transformer with embedding dimension \(d\), \(L = 1\) layers and \(H = 1\) heads on reasoning with \(n\) propositions. The mean accuracy across three runs is reported.
}
\label{fig:q1}
\end{figure}


==> old/robustness_1.tex <==


\section{Language Models Fail to Reason Robustly}
\label{sec:robustness}

In this Section, we study the extent to which models fail to reason.
In particular, we study how to elicit some desired response (\emph{adversarial target}) from a reasoner model by appending some malicious \emph{attack tokens} to its input sequence.
We illustrate this mechanism in Figure~\ref{fig:attack}.

\input{figures/attack}

Although various forms of attacks exist~\cite{huang2023catastrophic}, we focus on suffix-based attacks~\cite{zou2023universal} due to their simplicity.
The subject of our attacks is a language model~\eqref{eqn:lm} trained for reasoning, which we call \(\msf{Reasoner}\).
Given some adversarial target \(s_{\msf{tgt}} \in \mbb{B}^n\), token sequence \(U \in \mbb{R}^{N \times d_{\msf{in}}}\), and \emph{attack budget} \(N_{\msf{atk}} > 0\), our attack problem is then expressed as the following search problem:
\begin{align} \label{eqn:attack_problem}
\begin{split}
    \text{find} \enskip U_{\msf{atk}} \in \mbb{R}^{N_{\msf{atk}} \times d_{\msf{in}}},
    \qquad 
    \text{subject to}
        &\enskip s_{\msf{tgt}} = \msf{Reasoner}(\msf{append}(U, U_{\msf{atk}}))
\end{split}
\end{align}
We first consider attacks against our theoretical construction of a perfect \(\msf{Reasoner}\) in Section~\ref{sec:theory_attacks}.
Then, in Section~\ref{sec:learned_attacks}, we consider the problem of training a language model to attack a learned \(\msf{Reasoner}\).


\subsection{Perfect Reasoners are Easily Attacked}
\label{sec:theory_attacks}

We first consider attacks against our theoretical construction of \(\msf{Reasoner}\) as in Section~\ref{sec:theory_overview}.
In particular, we find that \emph{a single suffix token suffices} to attack a perfect reasoner.
Moreover, we sketch this result below.

\begin{theorem}[Sketch of Attack Result]
\label{thm:attack_result_sketch}
Consider any \(\msf{Reasoner}\) language model as given in Section~\ref{sec:theory_overview}, token sequence \(U\), and adversarial target label \(s_{\msf{tgt}} \in \mbb{B}^n\), then for sufficiently large \(\kappa > 0\) we have:
\begin{align*}
    s_{\msf{tgt}} = \msf{Reasoner}(\msf{append}(U, u_{\msf{atk}}))
\end{align*}
with attack token \(u_{\msf{atk}} = (\mbf{0}_n, s_{\msf{tgt}} - \kappa (\mbf{1}_n - s_{\msf{tgt}}))
    \in \mbb{R}^{2n}\).
\end{theorem}

We present a proof in Appendix~\ref{sec:theory_attack}.
This result implies that our theoretical construction is still susceptible to attacks despite being a perfect reasoner.
In particular, the attack token is independent of the input \(U\) but is dependent on constants used in the theoretical constructions in Appendix~\ref{sec:theory_construction}.
Intuitively, this attack over-saturates the softmax attention mechanism with a large input.


\subsection{Training a Language Model for Attack}
\label{sec:learned_attacks}

We now show how a language model can be trained to attack \(\msf{Reasoner}\).
This attacking model, which we call \(\msf{Attacker}\), is to behave similarly to Figure~\ref{fig:attack} and has the same language model architecture as described in~\eqref{eqn:lm}.
For consistency, we remark that one must appropriately tokenize and append the adversarial target label \(s_{\msf{tgt}}\) with the token sequence \(U\).
Let \(\theta\) be the parameters of \(\msf{Attacker}\) and suppose that \(\mcal{D}\) is the training distribution of \(\msf{Reasoner}\).
We then express the \(\msf{Attacker}\) training as the following optimization problem:

\begin{align} \label{eqn:attacker_training_problem}
\begin{split}
    \underset{\theta}{\text{minimize}}
        &\quad \expval{U \sim \mcal{D}}\, \mcal{L}(\hat{s}, s_{\msf{tgt}}; \theta) \\
    \text{where}
        &\quad u_{\msf{atk}} = \msf{Attacker}(s_{\msf{tgt}}, U; \theta) \\
        &\quad \hat{s} = \msf{Reasoner}(\msf{append}(U, u_{\msf{atk}}))
    \end{split}
\end{align}
We emphasize that we are training only \(\msf{Attacker}\) and that \(\msf{Reasoner}\) is fixed.
We have left the loss function \(\mcal{L}\) under-specified for flexibility, but in our experiments of Section~\ref{sec:experiments_learned_attackers}, we use binary cross-entropy loss, which is the same objective used to train \(\msf{Reasoner}\).





==> old/theory_1.tex <==
\input{figures/modules}

\section{CoT Reasoning with Language Models}
\label{sec:theory}

In Section~\ref{sec:theory_autoregressive}, we first give an overview of autoregressive propositional inference, the main computational mechanism of CoT reasoning in propositional Horn logic.
Then, in Section~\ref{sec:theory_overview}, we give a technical overview of our construction of a language model capable of autoregressive propositional inference.
Notably, this model has two layers, one attention head, and an embedding dimension linear in the number of propositions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Autoregressive Propositional Inference}
\label{sec:theory_autoregressive}


The main idea of CoT reasoning with language models is to iteratively generate the intermediate \emph{proof states} until the target query is either proven or we exhaust our step budget.
A basic polynomial-time algorithm for Problem~\ref{prob:logical_reasoning} in propositional Horn logic is as follows: given a set of rules \(\Gamma\) and some query \(\tau \in \mbb{B}^n\), we begin at some initial proof state \(s_0 = \mbf{0}_n\) and iteratively generate a sequence of proof states \(s_0, s_1, s_2, \ldots\)
where each subsequent state is given by a one-step rule application \(s_{k+1} = \Gamma(s_{k})\), defined as:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where \(\alpha \preceq s\) iff each \(\alpha_i \leq s_i\).
Therefore, we will simultaneously view \(\Gamma\) as a set of rules and as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
In the functional view, one-step rule application involves identifying which rules \((\alpha, \beta) \in \Gamma\) are applicable with respect to the current proof state \(s_k\), i.e., whether \(\alpha \preceq s_k\).
If so, we include \(\beta\) into the next state \(s_{k+1}\).
Observe that each \(s_{k} \preceq s_{k+1}\) by definition of \(\Gamma\), meaning that one needs at most \(n\) steps of rule application to prove \(\tau\).
To check whether \(\Gamma \vDash \tau\), it therefore suffices to check whether \(\tau \preceq s_n\).
We may stop the loop before the full \(n\) steps if some \(\tau \preceq s_{k}\), i.e., we have deduced the propositional query \(\tau\) before exhausting our \(n\)-step budget.

The act of generating new proof states via \(s_{k+1} = \Gamma(s_k)\) is also known as \emph{propositional inference} because we are deriving new propositions from existing ones.
Our goal with encoding language model-based CoT reasoning is to autoregressively execute propositional inference as described in~\eqref{eqn:one_step_rules}.
Given a set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and initial proof state \(s_0\), we adapt the autoregressive loop from~\eqref{eqn:autoreg} as follows:
\begin{align} \label{eqn:autoreg_propositional_inference}
\begin{gathered}
    U_0 = \msf{Tokenizer}(\gamma_1, \ldots, \gamma_r, s_0),
    \quad s_t = \msf{LM}(U_{t-1}) \\
    U_t = \msf{Stack}(U_{t-1}, \msf{Tokenizer}(s_t))
\end{gathered}
\end{align}
As with the classical algorithm, this process continues until either all \(s_0, s_1, \ldots, s_n\) are generated, or if at some \(s_k\) we have \(\tau \preceq s_k\).
Our theoretical analysis will focus on the internals of \(\msf{LM}\), in particular, the \(\msf{TF}\) module.
The sketch of our main theoretical CoT reasoning result is as follows.

\begin{theorem}[Sketch of CoT Logical Reasoning Result]
\label{thm:main_result_sketch}
Let \(\Gamma\) be any set of \(r\) rules over \(n\) propositions and \(\tau \in \mbb{B}^n\) a query.
There exists an \(\msf{LM}\) with autoregressive evaluation that decides Problem~\ref{prob:logical_reasoning} using \(L=2\) layers, \(H = 1\) attention heads, embedding dimension \(d = \mcal{O}(n)\), feedforward width \(d_{\msf{ffwd}} = 4d\), and \(\mcal{O}(n)\) autoregressive iterations.
\end{theorem}

The implication of this result is that the embedding dimension is the only parameter size that matters for handling instances with more propositions.
In our experiments of Section~\ref{sec:experiments}, we empirically demonstrate the importance of the embedding dimension.
Interestingly, we also found that increasing the number of layers improves scaling to instances with more propositions.



\subsection{Technical Overview of Constructions}
\label{sec:theory_overview}

We now give an overview of our theoretical construction of a transformer-based \(\msf{LM}\) capable of autoregressive propositional inference.
Consider a set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and proof states \(s_0, \ldots, s_{t-1}\) wherein each \(s_{k+1} = \Gamma(s_{k})\) by one-step rule application~\eqref{eqn:one_step_rules} and \(s_{t-1}\) is the most recent state.
The goal for a single autoregressive evaluation iteration is to output a label corresponding to \(s_{t}\).
Our high-level execution is described as follows:
\begin{align} \label{eqn:high_level_seqcls}
    (\gamma_1, \ldots, \gamma_r, s_0, \ldots, s_{t-1})
    \xrightarrow{\msf{Tokenizer}}
    U_{t-1}
    \xrightarrow{\msf{LM}}
    s_t
\end{align}
where the sequence length is \(N = r + t\) and \(U \in \mbb{R}^{N \times d_{\msf{in}}}\).
We will use an input token dimension of \(d_{\msf{in}} = 1 + 2n\), an embedding dimension of \(d = 2 + 3n\), and an output label dimension of \(d_{\msf{out}} = n\).
In the following, we first give an overview of the tokenization procedure.
We then give a summary of each of the three modules of an \(\msf{LM}\) as described in~\eqref{eqn:lm}, namely the embedding function \(\msf{Embed}\), the core transformer module \(\msf{Tf}\), and the classification head \(\msf{ClsHead}\).
A more detailed expansion of the pipeline~\eqref{eqn:lm} is shown in~\eqref{eqn:lm_pipeline}.


\paragraph{Tokenization}

Our tokenization scheme leverages our earlier simplifications in that facts are equivalent to rules with antecedents of \(\mbf{0}_n\).
Similarly, the proof states \(s_0, \ldots, s_{t-1}\) may also be thought of as facts.
For a rule \(\gamma = (\alpha_i, \beta_i) \in \mbb{B}^n \times \mbb{B}^n\) and a state \(s_k \in \mbb{B}^n\), the action of tokenization is respectively:
\begin{align} \label{eqn:tokenize}
\begin{split}
    \gamma_i &\xrightarrow{\msf{Tokenizer}}
    \begin{bmatrix} 0 & \alpha_i ^\top & \beta_i ^\top \end{bmatrix} \\
    s_k &\xrightarrow{\msf{Tokenizer}}
    \begin{bmatrix} 1 & \mbf{0}_n ^\top & s_k ^\top \end{bmatrix}
\end{split}
\end{align}
meaning that the input token dimension is \(d_{\msf{in}} = 1 + 2n\).
The leftmost bit of the vector indicates whether the token encodes a rule or a proof state.
We aim to be flexible between row and column representation of vectors, but we will interpret vectors to be in column form by default.


\paragraph{Embedding Function}
We next describe the embedding function \(\msf{Embed}: \mbb{B}^{N \times d_{\msf{in}}} \to \mbb{B}^{N \times d}\), which is an affine function that maps the token sequence to an embedded input sequence.
Our embedding function behaves as follows:
\begin{align} \label{eqn:embed_fn}
\begin{split}
    \begin{bmatrix} 0 & \alpha_i ^\top & \beta_i ^\top \end{bmatrix}
    &\xrightarrow{\msf{Embed}}
    \begin{bmatrix} 1 & 0 & \alpha_i ^\top & \beta_i ^\top & \mbf{0}_n ^\top \end{bmatrix} \\
    \begin{bmatrix} 1 & \mbf{0}_n ^\top & s_k ^\top \end{bmatrix}
    &\xrightarrow{\msf{Embed}}
    \begin{bmatrix} 1 & 1 & \mbf{0}_n ^\top & s_k ^\top & \mbf{0}_n ^\top \end{bmatrix}
\end{split}
\end{align}
wherein the embedding dimension is \(d = 2 + 3n\).
The leftmost bit is \(1\) for both the rule and state embedding.
This hot bit will be used to generate constants in our proof construction.
We call the rightmost \(n\) bits the \emph{workspace slot}, which is initially set to \(\mbf{0}_n\) and will be used for intermediate transformer layer computations.
Note that our construction does not require positional encodings because we only need information on whether each row encodes a rule or a state.



\paragraph{Transformer Layers}
We construct a shallow transformer with only two layers, denoted as \(\msf{Tf} = \msf{Layer}_2 \circ \msf{Layer}_1\).
The overall action of each layer is described as follows:
\begin{align} \label{eqn:layers}
\begin{split}
    X =
    \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        % z_{N-1} & \mbf{0}_n \\
        z_N ^\top & \mbf{0}_n ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_1}
    \begin{bmatrix}
        z_1 ^\top & \star \\
        \vdots & \vdots \\
        % z_{N-1} & w_{N-1} \\
        z_N ^\top & s_{t-1} ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Layer}_2}
    \begin{bmatrix}
        z_1 ^\top & \star \\
        \vdots & \vdots \\
        % z_{N-1} & w_{N-1} ' \\
        z_N ^\top & s_t ^\top
    \end{bmatrix}
\end{split}
\end{align}
where \(z_k \in \mbb{B}^{2 + 2n}\) denotes the first \(2 + 2n\) bits of each row, which recall has size \(d = 2 + 3n\).
First, \(\msf{Layer}_1\) writes some entries, which we express as \((\star) \in \mbb{R}^{n}\), to the first \(N-1\) rows and \(s_{t-1}\) to the \(N\)th row.
Next, \(\msf{Layer}_2\) writes some entries to the first \(N-1\) rows and \(s_t = \Gamma(s_{t-1})\) to the \(N\)th row.
The given construction of \(\msf{Tf}\) will not change the \(z_1, \ldots, z_N\) bits of each row; only the contents of the workspace slot are altered, and we pay special attention to the last row.

We defer a detailed exposition to Appendix~\ref{sec:tf_theory} and instead provide some intuition for now.
Our encoding employs two key ideas.
First, with appropriate scaling of the weights, we may use the attention block's inner product mechanism to perform conditional testing and parallel writes to the workspace slot of each row.
Second, we may use the feedforward block with a \(\msf{ReLU}\) activation to encode a thresholding function that binarizes the output of each layer to be \(\{0,1\}\).
Importantly, this allows us to implement binary disjunctions using sum-then-binarize operations.
For an input token sequence constructed from well-formed rules and proof states, the \(\msf{Tf}\) module will produce a binary-valued output at the \(N\)th row.


\paragraph{Classification Head}
Finally, the role of the classification head is to act as a linear projection on the workspace slot in order to extract the \(s_t\) bits.
In particular, we project out the last row.
Altogether, we expand the mappings of~\eqref{eqn:lm} in more detail and describe the three principal modules of \(\msf{LM}\) below:
\begin{align} \label{eqn:lm_pipeline}
    \begin{bmatrix}
        u_1 ^\top \\ \vdots \\ u_N ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Embed}}
    \begin{bmatrix}
        z_1 ^\top & \mbf{0}_n ^\top \\
        \vdots & \vdots \\
        z_N ^\top & \mbf{0}_n ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Tf}}
    \begin{bmatrix}
        z_1 ^\top & \star \\
        \vdots & \vdots \\
        z_N ^\top & s_t ^\top
    \end{bmatrix}
    \xrightarrow{\msf{ClsHead}}
    s_t
\end{align}
where \(u_1, \ldots, u_N \in \mbb{R}^{d_{\msf{in}}}\) are the input tokens as before, \(z_1, \ldots, z_N \in \mbb{B}^{2+2n}\) are the first \(2+2n\) non-workspace bits of the embedded input that are unchanged by \(\msf{Tf}\).



\paragraph{Checking the Query}
Finally, to check whether the query is proven at some step \(t\), it suffices to check whether \(\tau \preceq s_t\).
Observe that by definition of one-step rule application in~\eqref{eqn:one_step_rules}, we have \(s_0 \preceq s_1 \preceq \cdots \preceq s_t\).
Moreover, we need at most \(n\) iterations because there are only \(n\) propositions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Other Remarks}

% \red{AAAAAAAAAAAAAAAAAAAAAAAA}

% \red{AAAAAAAAAAAAAAAAAAAAAAAA}


==> old/theory_2.tex <==

\input{figures/layers_math}

\section{Reasoning with Language Models}
\label{sec:theory}

The main idea of CoT reasoning is to iteratively generate proof states until the target query is either proven or some budget is exhausted.
Given a set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and previously derived proof states \(s_0, \ldots, s_{t-1}\), the objective of a single reasoning step is to derive the next state \(s_t\).
This is repeated until the query \(\tau\) is derived.
We illustrate this in Figure~\ref{fig:autoreg} and present its main computational mechanism, autoregressive propositional inference, in Section~\ref{sec:theory_autoregressive}.
Then, in Section~\ref{sec:theory_overview}, we give a construction of an exact reasoning language model for propositional Horn logic.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Autoregressive Propositional Inference}
\label{sec:theory_autoregressive}

Our main challenge is to encode a language model that can perfectly perform one step of reasoning.
To approach this, we first study a simple and well-known algorithm for reasoning in propositional Horn logic.
Given a set of rules \(\Gamma\) and query \(\tau \in \mbb{B}^n\), we begin at the initial proof state \(s_0 = \mbf{0}_n\) and iteratively generate new states \(s_1, s_2, \ldots\) via one-step rule application \(s_{k+1} = \Gamma (s_k)\), defined as:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where \(\alpha \preceq s\) iff each \(\alpha_i \leq s_i\).
This one-step inference is also known as \emph{propositional inference} because we are deriving new propositions from existing ones.

Under this notation, we simultaneously view \(\Gamma\) as a rule set and as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
In the functional view, one-step rule application involves identifying which rules \((\alpha, \beta) \in \Gamma\) are applicable with respect to the current proof state \(s_k\), i.e., whether \(\alpha \preceq s_k\).
If a rule \((\alpha, \beta)\) is applicable, we include the propositions of \(\beta\) into the next state \(s_{k+1}\), i.e., \(\beta \preceq s_{k+1}\).
Observe that each \(s_{k} \preceq s_{k+1}\) by definition of \(\Gamma\), meaning that one needs at most \(n\) steps to prove \(\tau\).
To check whether \(\Gamma\) entails \(\tau\), it therefore suffices to check whether \(\tau \preceq s_n\).
% We may also stop the loop early if some \(\tau \preceq s_k\), i.e., we have deduced the query \(\tau\) before exhausting our \(n\)-step budget.


Having defined a single step of propositional inference, we now consider the autoregressive case, as described in Figure~\ref{fig:autoreg}.
In particular, such a loop can be expressed as the following set of recursive equations:

\begin{align} \label{eqn:autoreg_propositional_inference}
\begin{gathered}
    U_0 = \msf{Tokenizer}(\gamma_1, \ldots, \gamma_r, s_0),
    \quad s_t = \msf{LM}(U_{t-1}) \\
    U_t = \msf{Stack}(U_{t-1}, \msf{Tokenizer}(s_t))
\end{gathered}
\end{align}


\red{AAAAAA}



A basic polynomial-time algorithm for Problem~\ref{prob:logical_reasoning} in propositional Horn logic is as follows: given a set of rules \(\Gamma\) and some query \(\tau \in \mbb{B}^n\), we begin at some initial proof state \(s_0 = \mbf{0}_n\) and iteratively generate a sequence of proof states \(s_0, s_1, s_2, \ldots\)
where each subsequent state is given by a one-step rule application \(s_{k+1} = \Gamma(s_{k})\), defined as:
% \begin{align} \label{eqn:one_step_rules}
%     \Gamma(s)
%     = s \lor \bigvee
%         \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
% \end{align}
% where \(\alpha \preceq s\) iff each \(\alpha_i \leq s_i\).
Therefore, we will simultaneously view \(\Gamma\) as a set of rules and as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
In the functional view, one-step rule application involves identifying which rules \((\alpha, \beta) \in \Gamma\) are applicable with respect to the current proof state \(s_k\), i.e., whether \(\alpha \preceq s_k\).
If so, we include \(\beta\) into the next state \(s_{k+1}\).
Observe that each \(s_{k} \preceq s_{k+1}\) by definition of \(\Gamma\), meaning that one needs at most \(n\) steps of rule application to prove \(\tau\).
To check whether \(\Gamma\) entails \(\tau\), it therefore suffices to check whether \(\tau \preceq s_n\).
We may stop the loop before the full \(n\) steps if some \(\tau \preceq s_{k}\), i.e., we have deduced the propositional query \(\tau\) before exhausting our \(n\)-step budget.

The act of generating new proof states via \(s_{k+1} = \Gamma(s_k)\) is also known as \emph{propositional inference} because we are deriving new propositions from existing ones.
Given a set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and initial proof state \(s_0\), our strategy is to perform propositional inference in an autoregressive manner, as described in Figure~\ref{fig:autoreg}.
This procedure can also be expressed as the following set of recursive equations:
% \begin{align} \label{eqn:autoreg_propositional_inference}
% \begin{gathered}
%     U_0 = \msf{Tokenizer}(\gamma_1, \ldots, \gamma_r, s_0),
%     \quad s_t = \msf{LM}(U_{t-1}) \\
%     U_t = \msf{Stack}(U_{t-1}, \msf{Tokenizer}(s_t))
% \end{gathered}
% \end{align}
As with the classical algorithm, this process continues until either all \(s_0, s_1, \ldots, s_n\) are generated, or if at some \(s_k\) we have \(\tau \preceq s_k\).
Our theoretical analysis will focus on the internals of \(\msf{LM}\), in particular, the \(\msf{TF}\) module.
The sketch of our main reasoning result is as follows.

\begin{theorem}[Sketch of Reasoning Result]
\label{thm:main_result_sketch}
Let \(\Gamma\) be any set of \(r\) rules over \(n\) propositions and \(\tau \in \mbb{B}^n\) a query.
There exists an \(\msf{LM}\) with autoregressive evaluation that decides Problem~\ref{prob:logical_reasoning} using \(L=2\) layers, \(H = 1\) attention heads, embedding dimension \(d = \mcal{O}(n)\), feedforward width \(d_{\msf{ffwd}} = 4d\), and \(\mcal{O}(n)\) autoregressive iterations.
\end{theorem}

The implication of this result is that the embedding dimension is the only parameter size that matters for handling instances with more propositions.
In our experiments of Section~\ref{sec:experiments}, we empirically demonstrate the importance of the embedding dimension.
Interestingly, we also found that increasing the number of layers improves scaling to instances with more propositions.



\subsection{Technical Overview of Constructions}
\label{sec:theory_overview}

We now give an overview of our theoretical construction of a transformer-based \(\msf{LM}\) capable of autoregressive propositional inference.
Consider a set of rules \(\Gamma = \{\gamma_1, \ldots, \gamma_r\}\) and proof states \(s_0, \ldots, s_{t-1}\) wherein each \(s_{k+1} = \Gamma(s_{k})\) by one-step rule application~\eqref{eqn:one_step_rules} and \(s_{t-1}\) is the most recent state.
The goal for a single autoregressive evaluation iteration is to output a label corresponding to \(s_{t}\).
Our high-level execution is described as follows:
\begin{align} \label{eqn:high_level_seqcls}
    (\gamma_1, \ldots, \gamma_r, s_0, \ldots, s_{t-1})
    \xrightarrow{\msf{Tokenizer}}
    U_{t-1}
    \xrightarrow{\msf{LM}}
    s_t
\end{align}
where the sequence length is \(N = r + t\) and \(U_{t-1} \in \mbb{R}^{N \times d_{\msf{in}}}\).
We describe the behavior of each module of \(\msf{LM}\) is described in Figure~\ref{fig:layers_math}, where we use an input token dimension of \(d_{\msf{in}} = 1 + 2n\), an embedding dimension of \(d = 2 + 3n\), and an output dimension of \(d_{\msf{out}} = n\).
In the following, we first give an overview of \(\msf{Tokenizer}\) and then give a summary for each module of \(\msf{LM}\), those being \(\msf{Embed}\), \(\msf{Tf}\), and \(\msf{ClsHead}\).



\paragraph{Tokenization}

Our tokenization scheme leverages the insight that the proof states \(s_0, \ldots, s_{t-1}\) may be thought of as facts.
By the convention of empty conjunctions, we may therefore think of each state \(s_k\) as a rule \((\mbf{0}_n, s_k)\).
For a rule \(\gamma_i = (\alpha_i, \beta_i) \in \mbb{B}^n \times \mbb{B}^n\) and a state \(s_k \in \mbb{B}^n\), the action of tokenization is respectively:
\begin{align} \label{eqn:tokenize}
\begin{split}
    \gamma_i &\xrightarrow{\msf{Tokenizer}}
    \begin{bmatrix} 0 & \alpha_i ^\top & \beta_i ^\top \end{bmatrix} \\
    s_k &\xrightarrow{\msf{Tokenizer}}
    \begin{bmatrix} 1 & \mbf{0}_n ^\top & s_k ^\top \end{bmatrix}
\end{split}
\end{align}
meaning that the input token dimension is \(d_{\msf{in}} = 1 + 2n\).
The leftmost bit of the vector indicates whether the token encodes a rule or a proof state.
% We aim to be flexible between row and column representation of vectors, but we will interpret vectors to be in column form by default.


\paragraph{Embedding Function}
We next describe the embedding function \(\msf{Embed}: \mbb{B}^{N \times d_{\msf{in}}} \to \mbb{B}^{N \times d}\), which is an affine function that maps the token sequence to an embedded input sequence.
Our embedding function behaves as follows:
\begin{align} \label{eqn:embed_fn}
\begin{split}
    \begin{bmatrix} 0 & \alpha_i ^\top & \beta_i ^\top \end{bmatrix}
    &\xrightarrow{\msf{Embed}}
    \begin{bmatrix} 1 & 0 & \alpha_i ^\top & \beta_i ^\top & \mbf{0}_n ^\top \end{bmatrix} \\
    \begin{bmatrix} 1 & \mbf{0}_n ^\top & s_k ^\top \end{bmatrix}
    &\xrightarrow{\msf{Embed}}
    \begin{bmatrix} 1 & 1 & \mbf{0}_n ^\top & s_k ^\top & \mbf{0}_n ^\top \end{bmatrix}
\end{split}
\end{align}
wherein the embedding dimension is \(d = 2 + 3n\).
The leftmost bit is \(1\) for both the rule and state embedding.
This hot bit will be used to generate constants in our proof construction.
Note that in Figure~\ref{fig:layers_math}, we have replaced the two leftmost bits with \(\star\).
We call the rightmost \(n\) bits the \emph{workspace slot}, which is initially set to \(\mbf{0}_n\) and will be used by \(\msf{Layer}_1\), \(\msf{Layer}_2\), and \(\msf{ClsHead}\).
Note that our construction does not require positional encodings because we only need information on whether each row encodes a rule or a state.



\paragraph{Transformer Layers}
We construct a shallow transformer with only two layers, denoted as \(\msf{Tf} = \msf{Layer}_2 \circ \msf{Layer}_1\).
As described in Figure~\ref{fig:layers_math}, the action of \(\msf{Layer}_1\) is to perform state aggregation in order to write \(s_{t-1}\) to the workspace slot of the \(N\)th row.
Next, the role of \(\msf{Layer}_2\) is to select this \(s_{t-1}\) and perform rule application to derive \(s_t = \Gamma (s_{t-1})\), which then overwrites the \(N\)th row's workspace slot.

We defer a detailed exposition to Appendix~\ref{sec:tf_construction} and instead provide some intuition for now.
Our encoding employs two key ideas.
First, with appropriate scaling of the weights, we may use the attention block's inner product mechanism to perform conditional testing and parallel writes to the workspace slot of each row.
Second, we may use the feedforward block with a \(\msf{ReLU}\) activation to encode a thresholding function that binarizes the output of each layer to be \(\{0,1\}\).
Importantly, this allows us to implement binary disjunctions using sum-then-binarize operations.
For \(U_{t-1}\) tokenized from well-formed rules and states, the output sequence \(Y_{t-1} = (\msf{Tf} \circ \msf{Embed})(U_{t-1})\) contains exactly the binary vector \(s_t\) in its \(N\)th row's workspace slot.


\paragraph{Classification Head and Query Checking}
Finally, the classification head linearly projects out the \(n\) workspace slot bits from the last row.
Altogether, we have \(s_t = \msf{LM}(U_{t-1})\).
To check whether the state \(s_t\) proves the query \(\tau\), it suffices to check whether \(\tau \preceq s_{t}\).
Observe that by definition of one-step rule application~\eqref{eqn:one_step_rules}, we have \(s_0 \preceq s_1 \preceq \cdots \preceq s_t\).
Moreover, we need at most \(n\) iterations because there are only \(n\) propositions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Other Remarks}

% \red{AAAAAAAAAAAAAAAAAAAAAAAA}

% \red{AAAAAAAAAAAAAAAAAAAAAAAA}


==> old/theory_3.tex <==

\input{figures/layers_math}

\section{CoT reasoning with language models}
\label{sec:theory}

The main idea of CoT reasoning is to iteratively derive proof states until the target goal is either proven or some other stopping condition (e.g., maximum iterations) is met.
Given a set of rules \(\Gamma\) and previously derived proof states \(s_0, \ldots, s_{t-1}\), the objective of a single reasoning step is to derive the next state \(s_t\).
We show one step of reasoning in Figure~\ref{fig:autoreg} and give more details in Section~\ref{sec:theory_autoregressive}.
Then, in Section~\ref{sec:theory_overview}, we present a language model for perfect reasoning in propositional Horn logic.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{What does one step of reasoning look like?}
\label{sec:theory_autoregressive}

Our main challenge is to encode a language model that can perform one step of reasoning.
To approach this, we first consider rule application.
Given some proof state \(s \in \mbb{B}^n\) and rule \((\alpha, \beta) \in \Gamma\): if \(s\) subsumes \(\alpha\), then we may conclude that \((s \lor \beta) \in \mbb{B}^n\), where disjunction is defined coordinate-wise for binary vectors.
We may then view a single reasoning step with respect to \(\Gamma\) as the simultaneous application of all rules, for which we overload notation to express as follows:
\begin{align} \label{eqn:one_step_rules}
    \Gamma(s)
    = s \lor \bigvee
        \{\beta : (\alpha, \beta) \in \Gamma, \, \alpha \preceq s\}
\end{align}
where for two vectors, \(x \preceq y\) iff each \(x_i \leq y_i\).
Under this notation, we view \(\Gamma\) as a set \(\Gamma \subseteq \mbb{B}^{2n}\) and also as a function \(\Gamma: \mbb{B}^n \to \mbb{B}^n\).
Here, \(\Gamma(s)\) represents the aggregate result of all rule applications: if a rule \((\alpha, \beta) \in \Gamma\) satisfies the subsumption \(\alpha \preceq s\), then we include the propositions of \(\beta\) using a disjunction.
Starting at some initial proof state \(s_0 \in \mbb{B}^n\), we may repeatedly apply \(\Gamma: \mbb{B}^n \to \mbb{B}^n\) to generate a sequence of proof states:
\begin{align} \label{eqn:state_seq}
    s_0 \xrightarrow{\Gamma}
    s_1 \xrightarrow{\Gamma}
    s_2 \xrightarrow{\Gamma}
    \cdots
\end{align}
Observe that \(s_0 \preceq s_1 \preceq s_2 \preceq \ldots\) by definition of \(\Gamma\).
Moreover, because there are \(n\) propositions: to check whether \(\Gamma\) entails the goal \(\tau\), it suffices to check whether \(\tau \preceq s_n\).


Our main theoretical contribution is to encode a language model \(\msf{LM}\) with a one-layer transformer that can exactly simulate the sequence~\eqref{eqn:state_seq} using an autoregressive evaluation strategy.
An overview of this is given in Figure~\ref{fig:autoreg} (more details in Section~\ref{sec:theory_overview} and Figure~\ref{fig:layers_math}), where the autoregressive loop is expressed as the following set of recursive equations:
\begin{align}
\label{eqn:autoreg_loop}
\begin{split}
    U_0 &= ((\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r), (\mbf{0}_n, s_0)) \\
    U_{t} &= \msf{append}(U_{t-1}, (\mbf{0}_n, \hat{s}_t)),
    \quad 
    \hat{s}_{t} = \msf{LM}(U_{t-1})
\end{split}
\end{align}
where we tokenized proof states by padding a \(\mbf{0}_n\) at the start.
Starting at some shared \(s_0 \in \mbb{B}^n\), our encoding guarantees an exact simulation trajectory between~\eqref{eqn:state_seq} and~\eqref{eqn:autoreg_loop} in the sense that \(s_t = \hat{s}_t\) for all \(t\).
We sketch this statement in relation to the broader reasoning problem below.




\begin{theorem}[Sketch of Reasoning Result]
\label{thm:main_result_sketch}
We can solve Problem~\ref{prob:logical_reasoning} in \(\mcal{O}(n)\) autoregressive iterations using an \(\msf{LM}\) of size:
\(L=1\) layers, \(H = 1\) attention heads, embedding dimension \(d = 1 + 2n\), and feedforward width \(d_{\msf{ffwd}} = 4d\).
\end{theorem}

Our result shows that transformers can efficiently encode one step of propositional inference as defined in~\eqref{eqn:one_step_rules}.
The algorithm described in~\eqref{eqn:state_seq} is also known as \emph{SLD resolution with forward chaining}~\cite{levesque1986knowledge}, and we give further discussion in Section~\ref{sec:discussion_logic}.



% This mechanism is broadly called \emph{propositional inference} because new propositions are derived from existing ones through a set of inference rules.


\subsection{Transformers can encode one step of reasoning}
\label{sec:theory_overview}

We now present a language model that executes one step of reasoning.
Given any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and sequence of states \(s_0, \ldots, s_{t-1}\) derived as in~\eqref{eqn:state_seq}, we illustrate how to derive the next proof state \(s_t\) in Figure~\ref{fig:layers_math}.
In particular, we use input token dimension \(d_{\msf{in}} = 2n\), embedding dimension \(d = 1 + 2n\), and output label dimension \(d_{\msf{out}} = n\).
We next describe the actions of each language model component: \(\msf{Embed}\), \(\msf{Transformer}\), and \(\msf{ClsHead}\).


\paragraph{Embedding function}
For any token \(u \in \mbb{R}^{2n}\), we define \(\msf{Embed}(u) = (1, u)\).
This prepending is applied row-wise to each of the \(N = r + t\) tokens in \(U_{t-1} \in \mbb{R}^{N \times 2n}\) to form the embedded inputs \(X_{t-1} = \msf{Embed}(U_{t-1})\).



\paragraph{Transformer}
Our result in Theorem~\ref{thm:main_result_sketch} states that \(L = 1\) layers suffice for propositional inference.
Therefore, we represent our transformer as follows:
\begin{align*}
    \msf{Transformer} = (\msf{Id} + \msf{Ffwd}) \circ (\msf{Id} + \msf{Attn})
\end{align*}
Given \(X_{t-1} = \msf{Embed}(U_{t-1})\), we first approximate rule application using \(\msf{Id} + \msf{Attn}\), and then adjust this approximation into a binary vector via \(\msf{Id} + \msf{Ffwd}\).
Taken together:
\begin{align*}
    X_{t-1} \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        \star & \star \\
        \star & (\Gamma(s_{t-1}) + \varepsilon)^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        \star & \star \\
        \star & s_t ^\top
    \end{bmatrix}
\end{align*}
where let \(\star\) denote miscellaneous entries of the appropriate dimensions, let \(\varepsilon \in \mbb{R}^n\) denote the approximation error, and recall that \(s_t = \Gamma(s_{t-1}) \in \mbb{B}^n\).


Our encoding employs two key ideas.
First, we observe that the attention block's inner product mechanism can check whether a rule is applicable with respect to a proof state.
Second, we may use the \(\msf{Id} + \msf{Ffwd}\) block to implement a piecewise linear function that approximates indicator functions, which lets us binarize the outputs of \(\msf{Id} + \msf{Ffwd}\) when they fall within some prescribed range.
We compose these two ideas to implement binary disjunctions using a single layer, thereby encoding one step of propositional inference as defined in~\eqref{eqn:one_step_rules}.
We provide additional details in Appendix~\ref{sec:theory_construction}.


\paragraph{Classification head}
We define \(\msf{ClsHead}\) as a linear projection on the last term of the embedded output sequence \(Y_{t-1} = \msf{Transformer}(X_{t-1})\).
In particular, the last row of \(Y_{t-1}\) has form \((1, \mbf{0}_n, s_t) \in \mbb{B}^{1 + 2n}\), with projection on \(s_t\) accordingly defined.
We operate only on the last row (i.e., the last sequence term) because we use causal self-attention, which we elaborate on in Appendix~\ref{sec:theory_construction}.

\paragraph{Proving the goal}
Altogether, we have the relation \(s_t = \Gamma(s_{t-1}) = \msf{LM}(U_{t-1})\) for any \(t\) and initial state \(s_0\) as given in the autoregressive loop~\eqref{eqn:autoreg_loop}.
To check whether the state \(s_t\) entails the goal \(\tau\), it suffices to check whether \(\tau \preceq s_t\).
Because there are \(n\) prepositions, we need to run the loop for at most \(n\) iterations.




==> old/theory_4.tex <==



\input{figures/layers_math}

\section{CoT Reasoning with Language Models}
\label{sec:theory}

The main idea of CoT reasoning is to iteratively derive proof states until the target goal is either proven or some other stopping condition (e.g., maximum iterations) is met.
Given a set of rules \(\Gamma\) and previously derived proof states \(s_0, \ldots, s_{t}\), the objective of a single reasoning step is to derive the next state \(s_{t+1}\).
We show one reasoning step in Figure~\ref{fig:autoreg} and give more details in Section~\ref{sec:theory_autoregressive}.
Then, in Section~\ref{sec:theory_overview}, we present a language model for perfect reasoning in propositional Horn logic.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{What Does One Step of Reasoning Look Like?}
\label{sec:theory_autoregressive}



Our main theoretical contribution is to encode a language model \(\msf{LM}\) with a one-layer transformer that can exactly simulate the sequence~\eqref{eqn:state_seq} using an autoregressive evaluation strategy.
An overview of this is given in Figure~\ref{fig:autoreg} (more details in Section~\ref{sec:theory_overview} and Figure~\ref{fig:layers_math}), where the autoregressive loop is expressed as the following set of inductive equations:
\begin{align}
\label{eqn:autoreg_loop}
\begin{split}
    U_0 = ((\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r), (\mbf{0}_n, s_0)),
    \enskip
    U_{t+1} = \msf{append}(U_{t}, (\mbf{0}_n, \hat{s}_{t+1})),
    \enskip 
    \hat{s}_{t+1} = \msf{LM}(U_{t})
\end{split}
\end{align}
where proof states are tokenized by padding a \(\mbf{0}_n\) at the start.
Beginning at some shared \(s_0 \in \mbb{B}^n\), our encoding guarantees an exact match between the \(\hat{s}_1, \hat{s}_2, \hat{s}_3, \ldots\) generated by~\eqref{eqn:autoreg_loop}, and the \(s_1, s_2, s_3, \ldots\) generated by repeated application of \(\Gamma\) as in~\eqref{eqn:state_seq}.
That is, \(\hat{s}_t = s_t\) for all \(t \geq 1\).
This is sketched in relation to the broader reasoning problem below.




\begin{theorem}[Sketch of Reasoning Result]
\label{thm:main_result_sketch}
Problem~\ref{prob:propositional_entailment} is solvable in \(\mcal{O}(n)\) autoregressive iterations using an \(\msf{LM}\) of size:
\(L=1\) layers, \(H = 1\) attention heads, embedding dimension \(d = 1 + 2n\), and feedforward width \(d_{\msf{ffwd}} = 4d\).
\end{theorem}

Our result shows that transformers can efficiently encode one step of propositional inference as defined in~\eqref{eqn:one_step_rules}.
The strategy described in~\eqref{eqn:state_seq} and~\eqref{eqn:autoreg_loop} is effectively \emph{forward chaining}~\cite{levesque1986knowledge}, a classic algorithm for propositional inference in Horn logic.



% This mechanism is broadly called \emph{propositional inference} because new propositions are derived from existing ones through a set of inference rules.


\subsection{Transformers Can Encode One Step of Reasoning}
\label{sec:theory_overview}

We now present a language model that executes one step of reasoning.
Given any rule set \(\Gamma = \{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r)\}\) and sequence of states \(s_0, \ldots, s_{t}\) by \(t\) previous applications of \(\Gamma\), we illustrate how to derive the next proof state \(s_{t+1}\) in Figure~\ref{fig:layers_math}.
In particular, we use input token dimension \(d_{\msf{in}} = 2n\), embedding dimension \(d = 1 + 2n\), and output label dimension \(d_{\msf{out}} = n\).
We next describe the actions of each language model component: \(\msf{Embed}\), \(\msf{Transformer}\), and \(\msf{ClsHead}\).


\paragraph{Embedding Function}
For any token \(u \in \mbb{R}^{2n}\), we define \(\msf{Embed}(u) = (1, u)\).
This prepending is applied row-wise to each of the \(N = r + t + 1\) tokens in \(U_{t} \in \mbb{R}^{N \times 2n}\) to form the embedded inputs \(X_{t} = \msf{Embed}(U_{t})\).



\paragraph{Transformer}
Our result in Theorem~\ref{thm:main_result_sketch} states that \(L = 1\) layers suffice for propositional inference.
Therefore, we represent our transformer as follows:
\begin{align*}
    \msf{Transformer} = (\msf{Id} + \msf{Ffwd}) \circ (\msf{Id} + \msf{Attn})
\end{align*}
Given \(X_{t} = \msf{Embed}(U_{t})\), we first approximate rule application using \(\msf{Id} + \msf{Attn}\), and then adjust this approximation into a binary vector via \(\msf{Id} + \msf{Ffwd}\).
Taken together:
\begin{align*}
    X_{t} \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        \star & \star \\
        \star & (\Gamma(s_{t}) + \varepsilon)^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Ffwd}}
    \begin{bmatrix}
        \star & \star \\
        \star & s_{t+1} ^\top
    \end{bmatrix}
\end{align*}
where let \(\star\) denote miscellaneous entries of the appropriate dimensions, let \(\varepsilon \in \mbb{R}^n\) denote the approximation error, and recall that \(s_{t+1} = \Gamma(s_{t}) \in \mbb{B}^n\).


Our main insight is that \(\msf{Attn}\)'s inner product mechanism can check whether a rule is applicable with respect to a proof state, which we use to select and aggregate the consequent of applicable rules.
Moreover, we may use the \(\msf{Id} + \msf{Ffwd}\) block to implement a piecewise linear approximation of indicator functions, which we use to binarize the outputs of \(\msf{Id} + \msf{Attn}\) when they fall within some prescribed range.
In summary, we implement binary disjunctions using a single layer, thereby encoding one step of propositional inference as defined in~\eqref{eqn:one_step_rules}.
We provide additional construction details in Appendix~\ref{sec:theory_construction}.


% Our encoding employs two key ideas.
% First, we observe that the attention block's inner product mechanism can check whether a rule is applicable with respect to a proof state.
% Second, we may use the \(\msf{Id} + \msf{Ffwd}\) block to implement a piecewise linear function that approximates indicator functions, which lets us binarize the outputs of \(\msf{Id} + \msf{Ffwd}\) when they fall within some prescribed range.
% We compose these two ideas to implement binary disjunctions using a single layer, thereby encoding one step of propositional inference as defined in~\eqref{eqn:one_step_rules}.
% We provide additional details in Appendix~\ref{sec:theory_construction}.


\paragraph{Classification Head}
We define \(\msf{ClsHead}\) as a linear projection on the last term of the embedded output sequence \(Y_{t} = \msf{Transformer}(X_{t})\).
In particular, the last row of \(Y_{t}\) has form \((1, \mbf{0}_n, s_{t+1}) \in \mbb{B}^{1 + 2n}\), with projection on \(s_{t+1}\) accordingly defined.
We operate only on the last row (i.e., the last sequence term) because we use causal self-attention, which we elaborate on in Appendix~\ref{sec:theory_construction}.

\paragraph{Proving the Goal}
Altogether, we have the relation \(s_{t+1} = \Gamma(s_{t}) = \msf{LM}(U_{t})\) for any \(t\) and initial state \(s_0\) as given in the autoregressive loop~\eqref{eqn:autoreg_loop}.
To check whether the state \(s_{t+1}\) entails the goal \(\tau\), it suffices to check whether \(\tau \preceq s_{t+1}\).
Because there are \(n\) propositions, we need to run the loop for at most \(n\) iterations.




==> old/theory_5.tex <==

\input{figures/layers_math}

\section{CoT Reasoning with Language Models}
\label{sec:theory}

The main idea of CoT reasoning is to iteratively derive proof states until the target goal is either proven or some other stopping condition (e.g., maximum iterations) is met.
Given a set of rules \(\Gamma\) and previously derived proof states \(s_0, \ldots, s_{t}\), the objective of a single reasoning step is to derive the next state \(s_{t+1}\).
In Section~\ref{sec:theory_overview}, we first give a high-level overview of how this is done and state our theoretical result.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{What Does One Step of Reasoning Look Like?}
\label{sec:theory_overview}

We showcase one autoregressive iteration of CoT reasoning in Figure~\ref{fig:layers_math}.
Principally, this autoregressive loop is governed by the following set of inductive equations:
\begin{align} \label{eqn:autoreg_loop}
    X_{t+1} = \msf{append}(X_t, (\mbf{0}_n, \hat{s}_{t+1})),
    \quad \hat{s}_{t+1} \leftarrow \msf{TF}(X_t),
    \quad
    X_0 = \parens*{(\alpha_1, \beta_1), \ldots, (\alpha_r, \beta_r), (\mbf{0}_n, s_0)}
\end{align}
where \(\hat{s}_{t+1}\) is extracted out from the last row of \(\msf{TF}(X_t)\) via a linear projection.
The goal is to learn weights for \(\msf{TF}\) such that we can simulate applications of \(\Gamma\) in the following sense:
\begin{align*}
    s_0 \xrightarrow{\Gamma}
        s_1 \xrightarrow{\Gamma}
        s_2 \xrightarrow{\Gamma}
        \cdots
    \quad \approx \quad
    s_0 \xrightarrow{\msf{TF}}
    \hat{s}_1 \xrightarrow{\msf{TF}}
    \hat{s}_2 \xrightarrow{\msf{TF}}
    \cdots
\end{align*}

Our main theoretical contribution is to show that, under some assumptions, there exist weights for \(\msf{TF}\) such that \(s_t = \hat{s}_t\) for all steps \(t\).
We formalize this as follows:
\begin{theorem}[Encoding Result] \label{thm:encoding}
Problem~\ref{prob:propositional_entailment} is solvable in \(n\) autoregressive iterations using \(\msf{TF}\) with embedding dimension \(d = 2n\) and feedforward width \(d_{\msf{ffwd}} = 4d\).
\red{(FIX)}
\end{theorem}
\begin{proof}(Sketch)
With an appropriate choice of weights for the self-attention block:
\begin{align*}
    X = \begin{bmatrix}
        \alpha_1 ^\top & \beta_1 ^\top \\
        \vdots & \vdots \\
        \mbf{0}_n ^\top & s_t ^\top
    \end{bmatrix}
    \xrightarrow{\msf{Id} + \msf{Attn}}
    \begin{bmatrix}
        \star & \star \\
        \vdots & \vdots \\
        \star & \parens*{s_t + \sum_{i: \alpha_i \preceq s_t} \beta_i + \varepsilon}^\top
    \end{bmatrix}
    \in \mbb{R}^{N \times 2n},
\end{align*}
where \(\varepsilon\) is a small residual term.
This approximates rule application in the sense that
\begin{align*}
    \parens*{s_t + \sum_{i: \alpha_i \preceq s_t} \beta_i + \varepsilon}_j
    \begin{dcases}
        \leq 1/3 & \text{iff \(\Gamma(s_t)_{j} = 0\)} \\
        \geq 2/3 & \text{iff \(\Gamma(s_t)_{j} = 1\)}
    \end{dcases},
    \qquad \text{for all coordinates \(j = 1, \ldots, n\)},
\end{align*}
where the disjunctions in rule application (see~\eqref{eqn:one_step_rules}) are implemented with scaled summation of binary values.
Then, \(\msf{Id} + \msf{Ffwd}\) approximates an indicator function on values \(\geq 2/3\).
\end{proof}


%%%%%



\subsection{(Q1) How Good are Learned Reasoners?}
We have shown that shallow transformers can theoretically encode one step of propositional reasoning, but how do they fare in practice?
We now show that learned models can indeed attain high accuracies across different values of \(n\) (number of propositions) and \(d\) (embedding dimension).


\paragraph{Model Setup}
We use GPT-2~\citep{radford2019language} as our base transformer model initialized with one layer, one self-attention head, and different values of embedding dimension \(d\).
By default, GPT-2 uses feedforward width \(d_{\msf{ffwd}} = 4d\) with GeLU activation and layer norms.


\paragraph{Dataset Setup}
Although we use randomized datasets for this experiment, we must be careful in their generation.
We first generate an initial random set of rules as follows:
\begin{align*}
    \Gamma_{\msf{init}} = \{
        (\alpha_1, \beta_1),
        \ldots,
        (\alpha_r, \beta_r)
    \},
    \quad \alpha_i, \beta_i \sim \mcal{B}^n(p),
    \quad p \sim \msf{Unif}(0.2, 0.3),
    \quad r \sim \msf{Unif}(32, 64),
\end{align*}
where \(\mcal{B}^n (p)\) is the \(n\)-dimensional coordinate-wise iid Bernoulli distribution with hot probability \(p\), and \(\msf{Unif}\) is the uniform distribution that may be continuous or discrete depending on context.
However, observe that \(\Gamma_{\msf{init}} (\mbf{0}_n) = \mbf{0}_n\) with high probability if \(n\) is sufficiently large, meaning that each rule is hard to trigger.
Therefore, we modify \(\Gamma_{\msf{init}}\) to have enough structure to prevent the model from learning a trivial (all zeros) solution.
For some \(k \sim \msf{Unif}(4, 7)\), we generate \(\Gamma = \msf{InjectStructure}(\Gamma_{\msf{init}}, k)\) to ensure a non-trivial sequence of proof states \(\mbf{0}_n = s_0 \prec \cdots \prec s_k\).
Using this, we return the input sequence:
\begin{align*}
    X = \msf{append}(\Gamma, (\mbf{0}_n, s_0), \ldots, (\mbf{0}_n, s_t))
    \in \mbb{R}^{(r+t+1) \times 2n},
    \quad s_{t+1} = \Gamma(s_t),
    \quad s_{0} = \mbf{0}_n,
    % \quad t \sim \msf{Unif}(1, 4).
\end{align*}
where \(t \sim \msf{Unif}(1,4)\) is the number of previous steps.
The model's goal is to predict \(s_{t+1}\).


\paragraph{Training Setup}
We train each model for a total of 4096 steps with a batch size of 1024.
We use AdamW~\cite{Loshchilov2017DecoupledWD} as our optimizer with a \(5e^{-4}\) learning rate, \(10\%\) warmup, and linear decay schedule.
We use binary cross entropy with logit loss.
% By default, each experiment is run with three random seeds, and we report the mean validation accuracy of correctly predicting all \(n\) bits of the final state.


\input{figures/gpt2_grid}


We present our results in Figure~\ref{fig:gpt2_grid} for different \(n \in \{16, 32, \ldots, 128\}\), \(d \in \{32, 64, \ldots, 256\}\), and autoregressive steps \(k \in \{1,2,3\}\).
We observe that learning becomes harder as the number of steps increases, likely because the model must make the correct prediction on all \(k\) steps.
Notably, for \(d = 2n\) in the \(k=1\) case, the model consistently attains high accuracy \(99\%+\).
When \(d < 2n\), however, the accuracy quickly decays.
This suggests that, empirically for setup, our proposed encoding in Theorem~\ref{thm:encoding} is fairly tight.
Moreover, for all the plots, the trend in models that can attain \(99\%\) accuracy appears to be linear.




